Backpressure Flow Control

Effective congestion control for data center networks is becoming increasingly challenging with a growing amount of latency sensitive traffic, much fatter links, and extremely bursty traffic. Widely deployed algorithms, such as DCTCP and DCQCN, are still far from optimal in many plausible scenarios, particularly for tail latency. Many operators compensate by running their networks at low average utilization, dramatically increasing costs. In this paper, we argue that we have reached the practical limits of end-to-end congestion control. Instead, we propose, implement, and evaluate a new congestion control architecture called Backpressure Flow Control (BFC). BFC provides per-hop per-flow flow control, but with bounded state, constant-time switch operations, and careful use of buffers. We demonstrate BFC's feasibility by implementing it on Tofino2, a state-of-the-art P4-based programmable hardware switch. In simulation, we show that BFC achieves near optimal throughput and tail latency behavior even under challenging conditions such as high network load and incast cross traffic. Compared to existing end-to-end schemes, BFC achieves 2.3 - 60 X lower tail latency for short flows and 1.6 - 5 X better average completion time for long flows.

==> abstract.tex <==
Effective congestion control for data center networks is becoming
increasingly challenging with a growing amount of latency-sensitive
traffic, much fatter links, and extremely bursty traffic.
% rapidly increasing workload demand, ever
% faster links, small average transfer sizes, extremely bursty traffic, 
% limited switch buffer capacity, and latency-sensitive applications.
Widely deployed algorithms, such as DCTCP and DCQCN, are still far from optimal
in many plausible scenarios, particularly for tail latency. Many operators
compensate by running their networks at low average utilization, dramatically
increasing costs.

In this paper, we argue that we have reached the practical limits
of end-to-end congestion control. Instead, we propose, implement, and evaluate a new
congestion control architecture called \emph{Backpressure Flow Control} (BFC).
BFC provides per-hop per-flow flow control, but with bounded state, constant-time
switch operations, and careful use of buffers.
% based on hop-by-hop per-flow flow control . In contrast to prior hop-by-hop schemes, 
% BFC requires only limited metadata and packet buffering. 
% BFC involves using only simple per-packet operations supported by commodity switches. 
We demonstrate BFC's feasibility by implementing it on a state-of-the-art P4-based programmable 
hardware switch. In simulation, we show that BFC achieves near 
optimal throughput and tail latency behavior even under challenging conditions such as 
high network load and incast cross traffic. Compared to existing end-to-end schemes, 
BFC achieves 2.3\,-\,60$\times$ lower tail latency for short flows and 1.6\,-\,5$\times$ better
average completion time for long flows.

\if 0
In this paper, we argue that we have reached the practical limits
of end-to-end congestion control. \pg{Instead, we propose a new clean slate design 
based on hop-by-hop per-flow flow control called \emph{Backpressure Flow Control} (BFC). In contrast to prior hop-by-hop schemes, 
BFC requires only limited metadata, and simple per-packet operations supported by commodity switches. We demonstrate feasibility of our design by implementing and evaluating BFC on a P4-based programmable hardware switch. Using large-scale simulations, we show that BFC achieves near optimal tail latency behavior even under challenging conditions such as high network load and in-cast cross traffic. Compared to existing schemes, BFC achieves 2-60$\times$ lower tail latency for short flows. The average throughput for long flows is 1.5-5$\times$ better.}
\fi


==> background.tex <==
\section{Background}
\label{s:background}
Remote Direct Memory Access (RDMA) has become an increasingly popular paradigm for data center network communication.
For applications, RDMA offers extremely low overhead and high bandwidth, with message handling implemented
in hardware without OS kernel mediation.  And with RDMA over Converged Ethernet (RoCEv2)~\cite{infiniband2014rocev2}, RDMA can run on
any switched Ethernet physical layer.  

Because server network interface cards (NICs) have long been designed to provide high bandwidth
for large TCP transfers, the primary benefit of RDMA has been for applications with 
fine-grained sharing between nodes. These applications are often latency sensitive~\cite{logp}, and when work
is farmed out in parallel, tail-latency sensitive~\cite{dean2013tail} -- application performance often 
depends on the worst case communication time, rather than the average case. 

An ongoing challenge for RDMA networks is how best to handle congestion.
Because message handling is implemented in hardware, RDMA systems typically use simple error handling, 
such as Go-Back-N, that make performance highly vulnerable to packet loss. 
To address this, most RDMA-enabled data centers deploy a hop-by-hop flow control mechanism called 
PFC (Priority-based Flow Control). (For simplicity, we will focus on the case where there is
congestion among the traffic at a particular priority level.) With PFC, if the packets from
a particular input port start building up at a congested switch (past a configurable threshold),
the switch sends a pause frame upstream stopping that input from sending more traffic until the
switch has a chance to drain.  This prevents the switch buffers from being overrun and needing to drop packets.

Unfortunately, PFC has a side effect: head-of-line (HoL) blocking~\cite{dcqcn}. For example, suppose a congested
switch is receiving an incast of packets from several of its input ports; the incast will arrive more quickly
than it can drain, building up buffers, and causing PFC pause frames to be sent upstream on those input ports.
This will prevent packet loss, but only at the cost of pausing unrelated traffic that traverses the
paused link but is destined for other
uncongested output ports. These flows will be delayed 
until the incast packets can be drained. Worse, as packets queue up behind
a PFC, additional upstream PFCs can be triggered, widening the scope of HoL-blocking. 
Even without incast, random fluctuations
in load can cause short-term congestion and PFC pauses, leading to HoL-blocking of unrelated traffic.  
HoL-blocking is particularly problematic for tail-latency performance, as short flows can be
queued behind much longer flows. Any congestion hurts tail latency, 
but HoL-blocking delays are often a large multiple of the delays a packet would experience in an 
idealized non-HoL blocking network at the same load level.

To reduce HoL-blocking, researchers and data center operators have proposed several end-to-end
congestion avoidance systems that aim to reduce buffer occupancy and thus the need for 
PFC pause frames. Timely~\cite{timely}, DCQCN~\cite{dcqcn}, and HPCC~\cite{hpcc} monitor
gather information from the network in response to packet transmissions to gate how quickly
to send additional packets.  Because earlier results have shown that DCQCN outperforms Timely~\cite{ecnordelay,hpcc},
we focus our comparison on the later two. DCQCN and HPCC can be effective when congestion is due to
so-called elephant flows: large, many-round trip transfers that can be throttled up or down
based on network conditions to avoid HoL-blocking for short, latency sensitive flows. 
However, measurements of data center network workloads suggest that most traffic completes within 
at most a few round trips; simply prioritizing short flows over long flows is insufficient
when the network is overwhelmed with short to moderate flows.

We next argue that these trends are getting worse over time.


\if 0
Software networking stacks are finding it increasingly difficult to handle the low tail latency and high bandwidth requirements of the modern data centers. Increasingly, data centers are offloading their networking stacks into the hardware and are adopting remote direct memory access (RDMA) over Converged Ethernet Versions 2 (RoCEv2). While RDMA offers performance, it lacks flexibility. Running intricate network stack algorithms is challenging. A consequence is that for drops, current RDMA deployments do not support efficient packet retransmission algorithms such as Selective Acknowledgement (SACK). RDMA instead relies on primitive retransmission algorithms such as Go-Back-N or Go-Back-0 that are easier to implement in the hardware. These algorithms respond poorly to drop events, retransmitting multiple packets in response to a single packet drop. Moreover, data centers frequently have incast episodes (multiple senders sending to a single receiver). These traffic from incast flows can increase buffer build up at the bottleneck switch, increasing drops.  As a result, to avoid performance degradation due to drops, congestion control algorithms for RDMA strive to minimize drops and realize a ``lossless'' network.

\textbf{Priority-based Flow Control (PFC):} PFC is link level congestion control algorithm aimed at limiting the buffer occupancy and ensuring zero drops. In PFC, switches estimate the amount of buffer occupied by traffic from each incoming link (ingress port) at each priority level. If the buffer occupied by flows from a particular ingress port (I) at a given priority level (P) exceeds a certain threshold, then the switch sends a pause frame to the upstream switch corresponding to the ingress port I. On receiving the pause frame, the upstream switch pauses all the flows at priority level P destined to the downstream switch. Since PFC, signals pauses to the immediate upstream switch, it's reaction time is only 1 Hop-RTT (RTT between two directly connected switches). Thus, PFC is more reactive than congestion control protocols that adjust their rates at the NIC (e.g., DCQCN, HPCC, etc.) and react on the scale of end-to-end RTTs. Moreover, PFC is simple and doesn't have complicated control loops for adjusting rates. As a result, PFC is widely deployed in data centers for limiting drops in the network.

While PFC pauses reduce drops, they can cause serious head-of-line blocking problems. The problem is that PFC pauses all the flows on a port (for a particular priority), instead of just pausing the flow causing the congestion. This implies that a ``victim flow'' that was not causing congestion at the downstream switch, can still get paused in response to congestion caused by other flows. Moreover, pause frames can cascade across the data center, pausing multiple links. This problem is referred to as head-of-line blocking (HoL). HoL hurts both throughput and latency for flows. 

\textbf{CC protocols at the NIC:} To limit HoL, recently, many congestion control protocols (e.g., DCQCN, TIMELY, HPCC, etc.) have been proposed. These protocols adjust the rate of flows based on congestion signals from the switches, to reduce buffer occupancy and avoid HoL due to PFC or deep packet buffer build up. Because the congestion feedback from switch is delayed by an end-to-end RTT, these protocols are inherently slower in reacting to congestion compared to PFC (end-to-end RTT vs 1 Hop-RTT). By the time these protocols adjust their rates congestion state at the switches might have changed already. If the congestion at the bottleneck switch dropped within a RTT, then the feedback delay might cause flows to underutilize the network. Alternatively, if the congestion at the bottleneck switch increased, then the feedback delay might cause flows to increase the buffering triggering PFC or creating deep packet buffers.  Slower reaction times can thus lead to both under-utilization and higher latencies. Another problem with these protocols protocols have a large number of parameters governing the trade-off between utilization and latency. The parameters for a given protocol doesn't generalize across network conditions and workloads, and, need to be tuned manually given the environment.  

% this point doesn't really fit here, but might later
A potential solution to reduce head-of-line blocking is to supplement these congestion protocols with scheduling algorithms at the switches (e.g, SFQ, AFQ, etc.). While such policies can reduce head-of-line blocking due to large buffer build ups, the fail to reduce head-of-line blocking due to PFC pauses. The problem is that scheduling in itself doesn't reduce the buffering. During congestion episodes, the PFC pauses will thus be triggered at the same rate with and without scheduling. 

\textbf{Consequences of contemporary data center trends:} The slow reaction time of these congestion protocols can hurt performance significantly. PFC reacts faster, but it's inability to pause individual flows causes head-of-line blocking. The shortcomings of the schemes discussed so far are further aggravated by the following trends.
\fi 

\smallskip
\noindent\textbf{Trend 1: Rapidly increasing link speed}
\Fig{broadcom} shows the switch capacity of top of the line data center switches manufactured by Broadcom~\cite{broadcom,switchtrend}.  
Switch capacity and link speeds have increased by a factor of 10 over the past six years with no signs
of stopping. As a result, much more data can be transmitted within a single round trip; 
for example, with a 100\,Gbps network link and 12\,us round trip delay, there can be 150\,KB in flight
before {\em any} feedback is received at the endpoint.

Larger bandwidth-delay makes it harder for end-to-end congestion control to manage network buffers.
\Fig{dcqcnbuf} shows the cumulative distribution function (CDF) of buffer occupancy with DCQCN across 
different link speeds, using the T2 topology (from \S\ref{s:eval}) and the Google workload from Section~\ref{s:eval} set to 75\% load plus 5\% incast, 
but without PFC enabled. DCQCN fails to limit buffer occupancy at higher link speeds, if utilization is kept constant.

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/buffersize_linkspeed.pdf}
    \vspace{-4mm}
    \caption{\small Hardware trends for top of the line data center switches manufactured by Broadcom. Buffer size is not keeping up with increases in switch capacity.}
    \label{fig:broadcom}
    \vspace{-4.5mm}
 \end{figure}
 
 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/motivation_linkspeed2.pdf}
    \vspace{-4mm}
    \caption{\small CDF of switch buffer occupancy for DCQCN (without PFC). The workload is scaled
    for equal utilization at various link speeds. Higher speed switches reduce DCQCN's ability to control buffer occupancy.}
    \label{fig:dcqcnbuf}
    \vspace{-4.5mm}
 \end{figure}

\smallskip
\noindent\textbf{Trend 2: Buffer size is not scaling with switch capacity}
 \Fig{broadcom} shows that the switch buffer size relative to its capacity has decreased by a factor of 2 (from 80 us to 40 us) over the past six years. With smaller buffers relative to link speed, buffers now fill up more quickly, making it more difficult for end-to-end congestion control to manage those buffers. Using 100\,Gbps links and the same topology and workload as \Fig{dcqcnbuf}, \Fig{buffersizedelta} shows the effect on flow completion tail latency (99$^{th}$ percentile) as a function of the buffer space ratio. 
 If the buffer space ratio continues to go down due to chip design constraints, the ability of DCQCN to manage tail latency is likely to worsen.

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/motivation_buffer3.pdf}
    \vspace{-4mm}
    \caption{\small The effect of the switch buffer capacity ratio on the 99$^{th}$ percentile flow completion times (FCT) with DCQCN. Reducing buffer size hurts tail latency.}
    \label{fig:buffersizedelta}
    \vspace{-5.5mm}
 \end{figure}

\smallskip
\noindent\textbf{Trend 3: Flow sizes remain small}
\Fig{flowsize} shows the cumulative bytes contributed by flows with different sizes in three industry data center workloads: 1) All applications in a Google datacenter, 2) Hadoop cluster in a Facebook center, and 3) WebSearch workload from DCTCP~\cite{homa}. Note that these were not gathered on an RDMA network; they define a flow to be any
message with a large delay between subsequent transmissions. 
For each of these workloads, the majority of flows are smaller than the bandwidth-delay product.
Instead, the graph shows the byte-weighted cumulative distribution. For example,
the large majority of bytes in the Google workload are in flows that fit 
inside a single round trip. Although data processing jobs are typically considered to have large flows, 
almost all Facebook Hadoop traffic is likely to fit within a single round trip within the next few years,
with websearch graph analysis to follow shortly thereafter.

There are several consequences. Even if we develop protocols to gather precise information
about the state of the bottleneck switch and return it to the sender, that information could well be
out of date by the time the sender could act on it.  Even if congestion is stable, 
end-to-end adaptation is inherently iterative. The rate for any particular flow depends
on secondary bottlenecks encountered by other flows as they simultaneously change their rate. 
Equilibrium sharing is reached with DCQCN only after many round trips.
Flows could be intentionally slowed down to provide more consistency over time, but this would come at a cost 
in substantial added latency (and tail latency).

While some have argued 
that data center flows are (or should be) increasing in size~\cite{atulhotos}, widespread use of RDMA is likely to be
pushing in the opposite direction, as it supports fine-grained memory access as a programming model. 

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/flowsize_cdf_contribution.pdf}
    \vspace{-4mm}
    \caption{\small Cumulative bytes contributed by different flow sizes for three different industry workloads.}
    \label{fig:flowsize}
    \vspace{-5.5mm}
 \end{figure}

\smallskip
\noindent\textbf{Trend 4: Multi-data center communication}
Fault tolerance concerns are leading many data center applications to be spread over clusters
of nearby data centers.  Protocols for homogeneous environments, similar link speed and latencies,
need to be generalized to these emerging workloads. With high bandwidth connectivity between
data centers and much longer round trip times, as well as the greater operating costs of
long haul fiber encouraging higher utilization, 
these settings are likely to put even greater pressure on end to end congestion control.



\if 0 
% maybe a good idea but we probably don't have space to really make the argument stick
\textbf{The CUT theorem:} We summarize these trends with what we call the CUT theorem of data center network operations.
Ideally, we want high capacity (C) links, moderate to high utilization of those links (U),
and low tail latency (T). However, typical data center workloads have transfer sizes that are much
smaller than the end to end bandwidth-delay product. The CUT theorem states that for typical
workloads and switch buffer sizes for a large-scale data center network,
end-to-end congestion control can at most provide two of the three desired properties.
The operator can choose which two, but not all three.  For example, we can support
moderate utilization and high capacity, as long as we take multiple round trips to probe the network,
but these extra probes result in higher latency.  
Or we can run the network at low utilization so that congestion is a non-issue,
allowing us to have high capacity and low tail latency.  Or with low capacity links,
most traffic will take multiple round trips, enabling end-to-end congestion control
to be effective.

\fi

\if 0
 \begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/buffersize_linkspeed.pdf}
    \vspace{-7mm}
    \subcaption{Switch capacity and buffer size trends}
    \label{fig:hardware_trends:data}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/motivation_linkspeed2.pdf}
    \vspace{-7mm}
    \subcaption{Consequences of increasing link speed}
    \label{fig:hardware_trends:effect}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Increasing link speed ---} The top figure shows hardware trends for top of the line data center switches manufactured by Broadcom. Both switch capacity and buffer size are increasing, but the buffer size is not keeping up with the switch capacity. The lower figure shows the CDF of buffer occupancy at the ToR switches for DCQCN (without PFC). With higher link speed DCQCN's ability to control the buffer occupancy reduces.}
    \label{fig:hardware_trends}
    \vspace{-4mm}
 \end{figure}
 
 \begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/flowsize_cdf_contribution.pdf}
    \vspace{-7mm}
    \subcaption{Bytes contributed}
    \label{fig:flow_size:data}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/motivation_distribution.pdf}
    \vspace{-7mm}
    \subcaption{Consequences of shorter flow sizes}
    \label{fig:flow_size:effect}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Flow size distribution ---} The top figure shows cumulative bytes contributed by different flow sizes for three different industry workloads. The lower figure shows 95$^{th}$ percentile FCTs for these workloads with DCQCN. Workloads with smaller flows experience higher FCTs. The offered load and the data center topology is same as \Fig{hardware_trends:effect}. }
    \label{fig:flow_size}
    \vspace{-4mm}
 \end{figure}
 
The data center topology in the experiment consists of 64 leaf, 4 top of the rack (ToR) and 8 spine nodes. The flow size distribution was derived from a google datacenter trace (see \Fig{flow_size:data}). The offered load was 75\%, with 5\% additional load from 20 to 1 incast of 10MB. For DCQCN, the threshold for marking ECN (i.e. the desired limit on buffering) was set to K$_{min}$ = 100KB and K$_{max}$ = 400KB in each case. DCQCN fails to limit the buffer occupancy to the desired level on higher speed links. Increasing link speed, increases the buffer occupancy.


The latter workloads (Facebook and WebSearch) are running a single application that usually transfers large amounts of data. As a result in these workloads, majority of the traffic is contributed by long flows. To increase resource utilization, modern data centers instead run a variety of applications, many of which use small request-response style messages. As a result, in these datacenters a significant fraction of the traffic is from short flows. In the Google workload, more than 50\% of the traffic is contributed by flows with size smaller than the 1 BDP (assuming 100 Gbps links and 12 us end-to-end RTT). This implies that majority of the traffic is contributed by flows which finish before undergoing rate adjustments by the congestion control protocol. Without rate adjustments, this traffic can build up buffers causing head-of-line blocking.

Data center applications are increasingly using request-response style messages (e.g., remote procedure calls or RPCs). The data associated with these messages/flows is usually small (less than few 100 kilobytes). 

\Fig{flowsizefct} shows the impact of flow size distribution of these workloads on the tail FCT slowdowns with DCQCN. The topology and the offered load is same as \Fig{hardware_trends:effect}. Workload with longer flows have better FCTs. With longer flows, the congestion control protocol can exert control over a higher fraction of the traffic, limiting buffers and decreasing head-of-line blocking.

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/motivation_distribution.pdf}
    \vspace{-3mm}
    \caption{\small Tail latency (95$^{th}$ percentile) flow completion times for three workloads using DCQCN. Workloads with smaller flows have worse tail latency.}
    \label{fig:flowsizefct}
    \vspace{-4mm}
 \end{figure}
 
 Existing congestion control protocols have been designed for homogeneous environments, i.e. similar link speed and latencies across the data center. These protocols are not well suited for emerging heterogeneous environments. An example is networks with inter-connected data centers in the same metropolitan area, with intra and inter-data center traffic. In such a network, the inter-data centers flows will have much higher RTTs compared to the intra-data center flows. With existing protocols, the inter-data center flows will react much slower compared to the intra-data center flows. These slower reaction times can cause inter-data center flows to overflow the buffers or underutilize the network.

\fi

==> concl.tex <==
\section{Conclusion}
\label{s:concl}
%\vspace{-1mm}
In this paper, we present Backpressure Flow Control (BFC), a practical congestion control architecture for datacenter networks. BFC provides per-hop per-flow flow control, but with bounded state, constant-time switch operations, and careful use of buffers. 
Switches dynamically assign flows to physical queues, allowing fair scheduling among competing flows and use selective backpressure to reduce buffering with minimal head of line blocking. 
Relative to existing end-to-end congestion control schemes, BFC improves
short flow tail latency and long flow utilization for networks with high bandwidth links and bursty traffic. 
We demonstrate BFC’s feasibility by implementing it on a state-of-art P4-based programmable hardware switch. In simulation, compared to existing end-to-end schemes, 
BFC achieves 2.3\,-\,60$\times$ lower tail latency for short flows and 1.6\,-\,5$\times$ better
average completion time for long flows.

\if 0
\pg{Change}
In this paper, we present Backpressure Flow Control (BFC), a new architecture for per-flow per-hop flow control in datacenter networks. Relative to existing end-to-end congestion control schemes, BFC improves
short flow tail latency and long flow utilization for networks with high bandwidth links and bursty traffic.
Switches dynamically assign flows to physical queues, allowing fair scheduling among
competing flows and selective backpressure on a per-flow basis.  On synthetic workloads derived from measurements
of data centers, BFC outperforms existing end-to-end congestion control mechanisms, both with
and without the presence of competing incast traffic.
\fi
%\textbf{Acknowledgements.} We thank Anirudh Sivaraman, Ahmed Saeed, and Srinivas Narayana for useful discussions. This work was supported in part by DARPA under Contract No. HR001117C0048, a gift from the Cisco Research Center, a Google Faculty Research Award, and NSF grants CNS-1407470, CNS-1751009, and CNS-1617702.
%\begin{equation}
%    er(t + RTT) =
%\end{equation}
%\textbf{This work does not raise any ethical issues.}


==> design.tex <==
\section{BFC Design}
\label{s:design}
Our approach is to design a practical system for per-hop, per-flow flow control.
We first describe the goals and constraints on our design,
we then sketch a plausible straw proposal that surprisingly turns out to
not work well at all, and we use that as motivation for our design, which
we evaluate in the following section.

\subsection{A Practical Solution to Network CUT}
\label{s:design_goals}

Our primary goal is to solve what we call the data center network CUT problem:
for a high capacity (C) network where most flows, and most bytes in flows,
fit inside the end-to-end bandwidth-delay product of the network, we want both
(i) efficient network utilization (U), that is, low network operating cost, and 
(ii) low tail latency (T) for flow completion, that is, better application performance.
Obviously, U and T are in conflict -- if the workload can be modeled as Poisson or more heavy-tailed
arrivals, then any increase in utilization will hurt flow completion times and
tail latency to an even greater degree.  Our goal is not to force the network operator to choose
how best to trade off application performance against system cost, but simply to
make efficient that tradeoff.

Our work is largely orthogonal to switch scheduling policy, but
for concreteness, we will constrain our discussion to fair queueing.
(One could equally combine our approach with hierarchical round robin,
priority scheduling, and so forth. These would have different scheduling metrics.)
We can then use an idealized fair queued switch with infinite buffering
as a benchmark.  Ignoring hardware constraints that would make such a switch
impractical to build, it would do well at CUT: flows could be safely sent into the
network at line rate, be queued at any bottleneck, and complete in a manner
that (roughly speaking) would minimize both average and tail completion time
by ensuring that every flow gets an equal share of the bottleneck link capacity.

We observe that for typical FIFO switches with limited buffering,
and typical data center workloads,
end-to-end congestion control {\em cannot} provide all three CUT properties.
At best, we must choose two out of the three. We can support moderate utilization (U) 
and high capacity links (C), as long as we spread transmissions over multiple round trips 
so that network probes measure a stable property.  These extra round trips result in higher latency.
Or we can over-provision the network, so that congestion is a non-issue,
allowing us to have high capacity links (C) with low tail latency (T).  Or with a low capacity network,
most flows will take many round trips, enabling end-to-end congestion control to be effective.

We want our approach to be practical, so we add three design constraints:

\begin{itemize}
\item{In-order packet delivery:} Packets from the same flow should be scheduled out the egress
port in the same order that they arrived at the switch ingress, to simplify packet handling at the
destination server.

\item{Zero configuration:} Our solution should require minimal configuration.
While it is possible to auto-tune parameters, a system with simpler and more intuitive configuration will be more likely to work robustly across rapidly evolving workloads and topologies.

\item{Hardware plausibility:} We assume hardware design constraints typical of modern switches.  For example,
we assume that there are a limited number (32 in our simulations) of FIFO 
queues per output port, that are scheduled in deficit round-robin or priority order. We can independently pause
and unpause each queue without preventing or slowing down forwarding from other FIFO queues.  However, if we pause a flow, we must pause
{\em all} of the packets that share the same FIFO queue.  In other words, head-of-line blocking is an inherent
challenge caused by hardware design constraints; we cannot assume that the switch scheduler can pick arbitrarily from any
of a large number of queued flows, in constant time.  Similarly, any metadata should be small, relative to
the space required for switch packet buffers.
\end{itemize}

\input{table.tex}

\subsection{Straw Proposal}
\label{s:straw}

We originally thought the following design would meet our goals. Following stochastic fair queueing~\cite{sfq},
compute the egress port for every arriving packet. Use a hash function on the flow header to consistently 
assign the packets of each flow to the same randomly-chosen FIFO queue at the egress.
We selectively pause a flow (at the upstream switch) if its queue depth becomes too large, 
e.g., one per-hop bandwidth-delay product. Above this point,
we would (likely) have time to signal the upstream switch to resume sending before the queue completely drained.
Of course, there could be contention at the upstream switch that would prevent the flow from refilling quickly enough,
but let us leave that aside for the moment. 

When we need to pause a flow, we need to pause all flows sharing the same FIFO queue at the upstream switch.  
To simplify matters, for the straw proposal, let's assume that we use the {\em same} hash function at each switch;
that way, {\em all} flows from the same ingress port to the same egress port, and assigned to the same FIFO queue,
will be paused together.  Unlike PFC, pauses in the straw proposal only affect individual flows; 
flows in other queues can continue to be forwarded downstream and scheduled out of the switch.

It seems like we should be done, and this paper could be short.  However, the straw proposal does not work
well, for three reasons.  First, the birthday paradox causes worse tail latency at the congested
switch than you might think.  With even a modest number of flows,
there is a significant chance that any specific flow will land in an already busy FIFO queue.
For example, with 10 flows assigned to 32 FIFO queues, it is highly likely that two flows will be randomly assigned
to the same queue, causing HoL-blocking and hurting tail latency.  Second, if we need to pause
a flow because a FIFO queue becomes too full, any flow at any upstream switch that hashes to the same queue
will potentially be affected by the pause. In other words, the per-flow pauses will propagate upstream
to affect other flows with the same hash value, even if they have different downstream routes.

These problems occur because flows experience hash collisions, even when we have enough physical resources
to give each flow its own dedicated FIFO queue.
We should expect this to be the common case.  With Poisson flow arrivals and where every flow
sends as fast as possible until it is done (as in RDMA), queueing theory~\cite{queueing} states
that the expected number of queued flows at a link is $1/(1-U)$ where $U$ is the utilization of the link,
and the variance in the queued flows is $1/(1-U)^2$. A link with 75\% utilization (that is, moderately congested)
will have an average of 4 queued flows, and a variance of 16, well under the typical
number of physical queues, but enough to make the birthday paradox matter.

The third problem is buffer management. Recall that the buffering in switches is trending 
downward relative to switch capacity, to a small multiple of the end-to-end bandwidth delay product. 
The straw proposal attempts to keep one hop of bandwidth delay per flow at the bottleneck switch.
In reality, however, this is overkill, as flows can only make use of one hop of bandwidth delay
{\em in aggregate}. Suppose we have an incast of flows at a congested switch. With enough incoming flows,
where each flow stores a bandwidth-delay at each hop, we could completely run out of buffer space 
and be forced into PFC-style blanket pauses. These in turn would
cause cascading upstream HoL-blocking.  Even without incast, moderate to severe congestion 
among a few hundred moderate-length flows
could lead to periods of buffer space exhaustion, with no compensating benefit in system performance.
% \tom{yes sorry about that but i think its ok}
% \pg{I am not sure if this problem occurs with the strawman in the eval as it uses \bfc{}'s threshold. I think it's fine.}
To address these issues, we add two more design constraints:

\begin{itemize}
\item{No needless HoL-blocking:} If the number of queued flows at an egress is less than the
number of FIFO queues, the design should have no HoL-blocking.  This applies recursively, so if a flow
is paused, but its upstream has fewer queued flows than the number of FIFO queues, it should also have no HoL-blocking.

\item{Stable buffer occupancy:} We should aim to store the minimum number of packets needed
to keep downstream links busy, consistent with scheduling objectives. In particular, 
buffer occupancy should not scale to a large multiple of the number of queued flows.
\end{itemize}

Providing a design that achieves these constraints, along with an evaluation of how this general approach
affects performance, are the principal contributions of this work.

\subsection{BFC Overview}
\label{s:bfc_overview}


Table~\ref{tab:functionality} outlines the main components of our solution, called Backpressure Flow Control (BFC).

To fix the problems with the straw proposal, 
we need to dynamically assign flows to unallocated physical queues, respecting packet order
so that subsequent packets for that flow will be placed into the same FIFO queue. Likewise, when we transmit the
last packet of a flow, we need to reclaim the physical queue and return it to the unallocated set.
Each flow has a unique 5-tuple of the source and destination address and port numbers; we can call this the
virtual flow ID (VFID). Our implementation needs to do a lookup on the VFID on every arriving packet,
and so we actually store the VFID as a hash of the 5-tuple.  
We also use this hash to signal per-flow pauses between switches, and so we configure all 
switches in the network to compute the VFID in the same way. We also need to be careful to handle
collisions in the VFID space correctly.  For simplicity, it is easiest to think of the VFID as
the 5-tuple. 

We have state per VFID: which physical queue it has been assigned, whether it has been paused, and how many packets are
queued. Unlike ATM switches that implement credit-based per-flow flow control~\cite{kung1995credit}, 
BFC only has state for a flow while the VFID has a queued packet; the state is reclaimed when the last packet
of the flow leaves the switch.
During normal operation, even a heavily used switch will only have a few hundred active VFIDs, that is,
flows with queued packets. A switch under incast can have more, and in the limit we could have as many
active VFIDs as buffer slots. We discuss the VFID storage and lookup problem in more detail later in this section (\Sec{bookkeeping}).

Since there are a limited number of physical queues, it is possible that all physical queues have
been allocated at a particular egress when a new flow arrives.  In that case, HoL-blocking is unavoidable.
In our implementation, we assign the flow to a random physical queue, but we could also be more sophisticated,
for example, by assigning the flow to the shortest queue or by avoiding those physical queues that have 
already been paused. Note that once a flow has been assigned to a queue, all packets from that flow
must be assigned to the same physical queue until all of the packets from that flow have left the switch.

In BFC, pauses are sent on each ingress link as a multistage bloom filter~\cite{multistagebloom} representing
all paused (and implicitly all unpaused) flows on a particular ingress link. The bloom filter is sent periodically,
at a rate of one every half (per-hop) round trip delay. These pauses do not need to be synchronized across inputs.
If a pause packet is dropped due to link corruption, the subsequent retransmission, half a round
trip delay later, is idempotent. We remove pauses by keeping an internal counting bloom filter at the downstream
switch, with a small integer per bit in the bloom filter.
If two paused VFIDs map to the same bloom filter bit position, the count will be two, so that when the time comes
to unpause one of the VFIDs, the bit transmitted upstream will still reflect the other VFID. A VFID 
% \pg{add "is considered paused at the upstream"?} 
is paused at the upstream if and only if the bloom filter matches on all four hash bit positions.

Note that BFC is {\em not} a per-hop credit-based flow control 
scheme~\cite{kung1995credit}. Flows start in the unpaused state, and can send at full line
rate until a pause is received; in practice, of course, the flow's packets may be interleaved
with other traffic traversing the same link, and so will generally send less quickly.
When a resume is received (because the VFID no longer matches in the bloom filter), 
the upstream can again send at the full line rate until another pause is received.

Unlike PFC where a pause blocks all traffic on a link, in normal operation a pause only affects a single flow. 
Thus, instead of delaying pauses as long as possible hoping to avoid them, we pause aggressively 
to preserve space in the congested switch 
for other flows to transit the switch unaffected. We pause whenever a packet arrives that, in expectation,
will not exit the switch before we can unpause and send the next packet -- taking into 
account the delay to the next pause frame,
its arrival at the upstream switch, and the transmission time for the subsequent packets from that flow 
to arrive at the downstream
switch.  

With deficit round robin, how long a queued packet will take to drain depends on a number of factors, 
including potentially the future arrival of packets for other flows. 
We estimate this as the number of active (unpaused) physical queues
at the egress port times the queue depth of the physical queue (including packets from other VFIDs assigned
to the same physical queue). As an estimate, it could be wrong. We compute whether a flow should remain
paused each time we dequeue one of its packets at the downstream switch.  We describe the pause/unpause
computation more precisely below.

Note that when we pause a flow at the upstream switch, it blocks all flows sharing the same queue from 
proceeding (HoL-blocking). Likewise, at the downstream switch, a physical queue can be shared by a mixture
of paused and unpaused VFIDs. Pausing one VFID does not prevent other flows from continuing to fill the downstream
buffer, although generally those flows will also be paused when their packets are added if the queue is 
sufficiently large.

% If flows are not paused, and \pg{Can we start the sentence from here instead ->} there are more FIFO queues than flows for a particular egress port, then
The packet scheduler uses deficit round robin to implement fair queueing, among the physical queues that
are not paused. Of course, when multiple VFIDs are assigned to a physical queue, we do not guarantee 
fair queueing among flows.


\subsection{Pause Threshold}
The goal for pausing in \bfc{} is to maintain the minimum amount of buffering without physical queues running out of packets due to pausing. We first describe the simpler case of how \bfc{} computes the pause/resume threshold when each flow queued at the egress port has its own physical queue.  We then describe the more general case in the next subsection.

%\noindent\textbf{Case 1: Active virtual flows < physical queues:} 
Because of communication delay, any pause/resume for a virtual flow will take $HRTT$, the round trip delay for
a pause message to reach the upstream and for its effect to return downstream. Moreover, since the pause/resume are 
only sent periodically (every $\tau$ s), the pause/resume can take an additional 
time $\tau$ to take effect. To account for this feedback delay, physical queues in \bfc{} need some amount 
of buffering before pausing so that they do not run out of packets. 
More formally, a physical queue builds ($HRTT + \tau$) of buffering (at the rate the physical queue is being dequeued) 
before pausing the virtual flow associated with the physical queue. $N_{active}$ is the 
number of active physical queues (that is, unpaused, with data to transmit). Then, the pause 
threshold $Th$ (for a particular physical queue) is $(HRTT + \tau) \cdot (\mu / N_{active})$,
where $\mu$ is the capacity of the link. This assumes the scheduling policy is deficit round robin;
a different calculation would be needed for other scheduling policies. Of course, this is just an
estimate, as the actual delay depends on future packet arrivals and the depth of the other queues.

Because the pause takes $HRTT + \tau$ to take effect, one might think we should pause
earlier than $Th$, to account for packets in flight or those that will be sent
before the pause can take effect. If switch buffering was
highly constrained, for example, we could monitor the rate at which data is arriving 
for a particular flow to estimate the precise moment that we should pause. 
Or, instead of a blanket unpause, we could give the upstream switch a specific number of credits
to use for filling the downstream buffer. Instead, we simply acknowledge that pauses take
some time to take effect, and therefore the amount of buffering consumed can exceed $Th$,
in the worst case, by $(HRTT + \tau) \cdot \mu$.

When a physical queue receives a pause from a downstream switch, it immediately pauses,
but it does not necessarily transmit the pause
to its upstream in turn.
Instead, it uses its local value of $N_{active}$ to compute the desired buffer length it would need if it were
{\em not} paused, and forwards a pause upstream when (or if) a packet is received that exceeds that threshold.
This way, when the queue is eventually resumed, there is sufficient buffering in place to
keep the link busy until its upstream can be resumed in turn.  
Note that we compute a flow's pauses/resumes only on packet arrival/departure for that flow.
We do not recalculate
the set of paused flows every time $N_{active}$ changes.


\if 0
\noindent\textit{Calculating $\mu_{pq}$:} The value of $\mu_{pq}$ depends on the scheduling policy. Moreover, it is also dependent on the number of physical queues that can be scheduled (i.e. have packets in them and are not paused because of the pauses from downstream). For fair queueing this value is simply given by:
\begin{align}
\mu_{PQ} = \frac{\mu}{N_{active}}
\end{align}
where $\mu$ is the link rate of the entire link, and $N_{active}$ is the number of physical queue at the link with packets in them that are not paused by the downstream. The rational is that the link is equally by the unpaused physical queues. The calculation for $\mu_{PQ}$ can be simply implemented as a match-action look up table on the current switches, with $N_{active}$ as the key. Note that if a given physical queue $PQ$ is paused (by the downstream), then it is not dequeuing any packets but we still use $\mu_{PQ}$ as it's rate for pausing/resuming. This is because immediatelt after sending a pause to the upstream, the physical queue might get resumed by the downstream. In this case, the physical queue will star dequeuing packets at $\mu_{PQ}$, therefore to avoid running out of packets the physical queue should pause only after accumulating $HRTT + \tau$  buffering at $\mu_{PQ}$.

\bfc{} decouples pauses and scheduling, the primary function of the physical queues is for selective pushback. This implies that \bfc{} can support a plethora of scheduling policies with the only constraint that the packets for an active virtual flow are enqueued in the same physical queue. This constraint ensures that pausing physical queues doesn't cause reordering.  For other scheduling policies, $\mu_{PQ}$ can also be calculated along similar lines. Moreover, one could simply use $\mu$ as an upper bound for $\mu_{PQ}$ for calculating the pause threshold. This might lead to some extra buffering though.
\fi

\subsection{Resuming Multiple Flows} 
\label{s:resuming_multiple}
We next discuss how pausing and resuming works when multiple flows
are assigned to the same physical queue. It is important to keep
in mind that while the different flows sharing a physical
queue use the same egress port, they may come from different ingress ports.

A strawman approach would be to pause as before, whenever a flow's packet
arrives if the physical queue is too large. When resuming, we could unpause
all $n$ flows associated with the physical queue if the queue length
drops below the threshold.  The problem is that each of the $n$ newly unpaused
flows could potentially send at line rate (if they originated on different
ingress ports). This could easily exhaust the downstream switch buffers
if applied across every congested egress queue, requiring a blanket pause
to avoid packet loss.

Since this extra buffering is unneeded, we adopt the heuristic that we
resume at most two flows per round trip (per physical queue). 
When a flow is to be resumed, we temporarily put it on a ``toberesumed'' list.  
Every bloom filter interval (half of $HRTT$), we take one flow off the ``toberesumed'' list
and clear its information from the bloom filter.
The choice to resume two flows per round trip helps in the 
scenario where a resumed virtual flow does not have packets at the upstream.

\if 0

when it exceeds the threshold and resume all the $n$ virtual flows when it drops below the threshold. Such an approach might build too much buffering, the problem is resuming all virtual flows when the physical queue goes below the pause threshold. After a resume event, each of the $n$ resumed virtual flows might send data at the line rate for $HRTT + \tau$ before being paused again. So after a resume event the physical queue can build $n \times (HRTT + \tau)$ of buffering. But recall that only $(HRTT + \tau)$ buffering is necessary for keeping the physical queue occupied. The extra buffering doesn't help the throughput of the virtual flows but can fill up buffers.

To avoid this extra buffering, in \bfc{} a physical queue doesn't instantaneously resume all flows when it goes below the pause threshold. Instead, when the physical queues exceeds the pause threshold it records all the associated virtual flows in a ``paused\_list'' (1 per physical queue). When a physical queue goes below the threshold, it resumes virtual flows periodically in the sequence they were paused. Specifically, it resumes 1 virtual flow per 0.5 $HRTT$. By doing so a physical queue limits the number of resumed virtual flows sending traffic to 2 (oversubscription). Consequently, this limits the buffering at the physical queue. The oversubscription helps in the scenario when a resumed virtual flow doesn't have packets at the upstream. By resuming multiple virtual flows, oversubscription avoids underutilization originating from virtual flows running out of packets.  Our evaluation (see \Fig{buffersize}) shows that the buffer optimization enables \bfc{} to limit buffering per physical queue.

Pausing all virtual flows when the physical queue exceeds the pause threshold might be infeasible on the datapath. For practical feasibility, switches pause a virtual flow (and add it to the paused\_list) only when a packet for the virtual flow is enqueued/dequeued. Checking whether the virtual flow should be paused only requires a look up operation (for calculating $(\mu_{pq})$ and a comparison operation to check if the physical queue size is greater than the threshold. For resuming virtual flows, the switch runs a dedicated thread that goes over all the physical queues every 0.5 $HRTT$ ($1$ us in typical datacenter setting), resuming 1 virtual flow for every physical queue with size lesser than the pause threshold.
\fi

\subsection{Communicating Pauses}
We next turn to the mechanics of communicating and implementing pauses. Instead of a bloom
filter, we could explicitly send each VFID to signal the pause/resume to the upstream switch. 
Since we only pause (and therefore resume) a flow at most once per packet
arrival, with batching this would bound the link overhead to a reasonable level.
We did not take this approach, however, as it would require 
communicating the pauses {\em reliably},
e.g., with a mechanism to detect and retransmit the pause packet if it was corrupted by
the transmission link.

Instead, we communicate pauses periodically using a small, idempotent multistage bloom filter~\cite{multistagebloom}.
Multistage bloom filters are ideal for communicating sparse bit maps and are convenient for processing updates
in parallel. In our evaluation we use 4 hash functions for the bloom filter, and 
a bloom filter size of 128 bytes. The contents of the bloom filter are specific to a given ingress.
For a 100\,Gbps link and a frequency of half of one hop round trip, this
implies a signalling overhead of about 1\%.
We note that this overhead will decrease with future increases in link speed.

Of course, a bloom filter can have false positives; in our setting, this can mean needlessly pausing a virtual flow
even though the downstream switch would permit it to send. With no HoL-blocking,
there are at most 32 queued flows to be paused per ingress. 
With 4 hash functions, the likelihood of a false positive is then 1 in 5 million. 
The false positive rate goes up with incast workloads and high levels of congestion; however,
in these settings, there is likely to be other flows with packets to transmit in its place.

When the upstream switch receives a bloom filter, it cannot easily invert it into
a set of paused VFIDs. Instead, we take the set of physical queues and check the first packet
against the bloom filter; if there is a match, we pause the physical queue. This implicitly
pauses all other packets in the same physical queue. Equally, if the first packet is not paused,
the second packet might be if it is for a different VFID. Thus, we recompute the match 
against the bloom filter after every packet send.

A detail is that the host network interface card (NIC) must be engineered to accept
bloom filter pause frames, to avoid potentially overfilling the
first level switch. 
We assume the NIC has sufficient hardware to maintain a physical queue per VFID, simplifying the logic.

\if 0
Recall that since an upstream switch doesn't know the VFID at the downstream, in \bfc{} switches communicate pauses on the virtual queue corresponding to the virtual flows to paused. Additionally to ensure that a virtual flow is paused at the upstream, the switch pauses a virtual queue if any virtual flow corresponding to the upstream (identified by the ingress port of the virtual flow) is paused. On receiving a pause for a virtual queue $VQ$, the upstream switch pauses all the physical queues where the virtual queue of the packet at the head is $VQ$. This pauses all the flows with the virtual queue $VQ$.

One way for communicating pauses to the upstream would be to send a pause/resume packet every time switch decides to pause/unpause the virtual queue at the port. A problem with such an approach is that if the link drops a pause/unpause packet then the upstream switch will not pause/resume the virtual queue until the downstream switch sends it a pause/resume again. To solve this in \bfc{} switches send a multistage bloom filter ~\cite{multistagebloom} periodically (every $\tau$ s) to communicate the set of paused virtual queues. Multistage bloom filters are ideal for communicating sparse bit maps, and allow updates to different stages in parallel (important for running at line rate). Since the fraction of paused virtual queues is small the false positive rate in the bloom filter is small. The switch maintains a bloom filter for every upstream switch, whenever a virtual queue is paused or resumed, the bloom filter is updated. Since the resume operation is equivalent of deleting entries, switches also maintain a counting bloom filter for all upstream switches.

The frequency for communicating pauses ($\frac{1}{\tau}$) via bloom filter presents a trade-off. If the frequency is small (i.e. $\tau$) is high) then the pause threshold will be high (Eq. ~\ref{eq:pause_threshold}), increasing buffering. If the frequency is high, then the bandwidth consumed by the bloom filter will be high. Increasing frequency has diminishing returns for reducing the pause threshold. We advocate using a $\tau$ value of the order of $HRTT$. In our experiments we use $\tau = 0.5 \times HRTT$. For the bloom filter, increasing the number of hash functions/stages reduces false positives but increases the computational complexity in updating it. In our evaluation we used 4 hash functions (or 4 parallel operations) for the bloom filter, this is supported by existing switches. Similarly, increasing the size of the bloom filter reduces the false positive rate but increases the bandwidth consumed by the bloom filter. We advocate using a bloom filter that consumes $\sim$ 1\% of the link capacity. For 100 Gbps links, with 2us 1 Hop RTT, this implies that the size of the bloom filter will be 128 bytes. The false positive rate for communicating a set of 32 paused virtual queues (the number of physical queues per port in our evaluation) is 1 in 5 million. Our evaluation (~\Fig{bloom}) shows that the performance of our system is not sensitive to the size of the bloom filter.

\noindent\textit{Implementation:} A switch runs a separate thread to pause/resume physical queues based on the received bloom filter. The thread goes over all the physical queues every $\tau$ duration, pausing/resuming the physical queues based on the bloom filter and the virtual queue of the packet at the head. Additionally, on dequeuing a packet from the physical queue, the switch checks whether the physical queue should be paused or not based on the virtual queue of the next packet in the physical queue. 

\noindent\textbf{\bfc{} NIC:} The NIC in \bfc{} is fairly simple. Unlike switches, the existing NIC's are capable of maintaining per flow queue. This implies that the NIC doesn't need the virtual space indirection or smart physical queue assignment. The \bfc{} NIC's don't enforce any rate limits on flows, instead they just schedule the per flow queues at line rate. On receiving a bloom filter, the NIC simply pauses flows if their corresponding virtual queue is present in the bloom filter.
\fi

\subsection{Reducing HoL Blocking for Short Flows}
Most traces of data center communication have found that a majority 
of flows are a single packet or less.  
If we assign the packets for these singleton packets
to an already occupied physical queue, they will experience HoL-blocking and poor tail
latency behavior.  Instead, we observe that singleton packets can be directly scheduled.
We maintain a special FIFO queue per egress port to hold the first packet from each flow.
One can think of this as pre-scheduling this packet, in priority ahead of the other 
physical queues for that egress.  We call this the ``high priority queue.'' 
We only put a packet into the high priority queue if its VFID is not paused
and there are no other packets queued for that flow. 
We never pause the high priority queue.  This means that a downstream switch may receive
one additional packet for a given newly paused flow than it would otherwise.
Additional packets that arrive for a flow are assigned to a regular physical queue, and scheduled normally.

In our prototype, we implement a simplification of this idea. The sender NIC marks
the first packet of every flow, and this signals the switch to put that packet into
the high-priority queue.  Unmarked packets are assigned as usual.

\if 0
This optimization is based on two observations. First, most of the flows in the current data center workloads are 1 packet or smaller, e.g., more than 60\% of the flows in the Google and FB\_Hadoop distribution are lesser than 1KB. Second, since these very short flows only have 1 packet, the scheduling decision for when to send the very short flow (or the corresponding packet) out only requires one scheduling decision per flow; as a result, these flows need not be scheduled out of separate physical queues. To save physical queues consumed by very short flows, we schedule them out of a single high priority physical queue. The \bfc{} switch identifies the first packet of any flow using it's sequence number in the packet header (required for Go-back-N at the NIC), and enqueues it in the high priority physical queue. Thus, the high priority queue contains all the flows with size < 1 packet. The high priority queue is scheduled ahead of all other physical queues, and reduces the number of physical queues used at an egress port, improving FCTs. Moreover, the high priority queue also reduce FCTs for these very short RPC style flows, benefitting applications. Our evaluation (\Fig{hpq}) shows that using a high priority queue saves physical queues and improves FCTs across all flow sizes. 
\fi

\subsection{Bookkeeping}
\label{s:bookkeeping}
When a packet arrives at a switch, we need to look up its VFID to locate
its state: whether the flow has any packets queued, which physical queue
is has been assigned, and whether it has been paused. Since it happens
on every packet, this lookup needs to be fast.  An array might work,
but a switch is unlikely to have more than a few hundred active flows
at any one time, while the VFID space is much larger to avoid collisions.
Thus, a linear array would be sparse and inefficient.

Instead, we use a hash table with a bucket size of four; we avoid needing
to store the VFID key by setting the number of buckets equal to the number
of VFIDs.  In addition to the VFID state, an entry in the hash table also stores 
the ingress and egress for the flow.
This means that we can disambiguate VFID collisions that have different
inputs and outputs; two 5-tuples that hash to the same VFID and 
that share the same input and output 
are treated (by that switch) as if they are the same flow.  We choose the VFID space to
be large enough that these collisions are rare. In our simulations,
the hash table took 256\,KB, or 2\% of the simulated packet buffer space available
in the switch.

A consequence of using a hash table with buckets is that the buckets
may fill from time to time. We maintain a small (100 entry) associative cache
for these overflow VFIDs.  If the overflow cache overflows, we put the
packets for these flows into a special per-egress overflow queue which is scheduled
along with the other queues in the normal manner. This is not perfectly order
preserving within a flow, as the hash table bucket may become free at some point
in the future, (rarely) leading to packets in both the overflow queue and a regular physical
queue.

\if 0

Since the VFID space is large, 
Till now, we assumed that the state for virtual flows is maintained as an array indexed by the VFID. Recall, that we want the space for virtual flows (and the virtual queues) to be very large to avoid Head-of-Line blocking. Storing this information as an array can be inefficient. Majority of the entries in the array will be for inactive virtual flows (virtual flows without any packets in the buffer), the space used by such inactive flows is unnecessary. We will now present an efficient way of storing the entries for virtual flows that still allows fast look ups.

Hash tables have proven to be effective to store such sparse entries in a space efficient way. We use a per switch hash table to keep track of state associated with virtual flows with packets in the buffer. The VFID and the state is stored as a <key, value> pair. To allow fast lookups at line rate, we limit the depth of the hash table to 4. This is because, finding an entry corresponding to a virtual flow requires $O(depth)$ operations. With an increased depth the switch might not be able to operate at line rate. 

Furthermore, to reduce the space required for storing the key for each entry. The length of the hash table is set to the number of virtual queues. This implies that the hash table need not store the virtual queue number in the key. To look an entry for a given VFID $X$, the switch matches the ingress and the egress port of $X$ against the entries in the hash table bucket corresponding to the virtual queue of $X$. Each entry in the hash table thus uses the <ingress port, egress port> pair as the key. Each key takes up 2 bytes of memory for a 256 port switch. The value (or the state) uses $~\sim$ 2 Bytes of memory; 1 Byte for the number of packets, 1 byte for the physical queue, 1 bit for tracking whether the virtual flow is paused or not. Thus each <key, value> pair consumes 4 Bytes, and each bucket in the hash table requires 16 Bytes of memory. The length of the hash table (or the number of virtual queues) depends on the size of the switch buffer. In our evaluation, we set the number of virtual queues to 16K, this consumes 256 KB of memory (only 2\% for our 12MB switch buffers). Without our optimization, the memory required for bookkeeping is 32 MB (for a 32 port switch).

\noindent\textit{Overflows:} An inadvertent consequence of using a hash table with limited depth is ``overflows''. When a packet for a new virtual flow (virtual without an entry in the hash table) arrives, there might not be enough space in the hash table bucket corresponding to the virtual flow. In such a case, the switch enqueues the overflow packet in an overflow queue (1 per egress port). For scheduling purposes, the overflow queue is treated as any other physical queue. 

The overflow packets can cause reordering for a virtual flow. E.g., consider a situation when the initial packets of a virtual flow $X$ were enqueued in the overflow queue because there was no space in the bucket ($VQ$) corresponding to $X$ in the hash table. Now, if the bucket $VQ$ freed an entry (i.e., a virtual flow in the bucket ran out of packets), then, a new packet arrival from $X$ will create an entry in the hash table; therefore, the subsequent packet from $X$ will be enqueued in a regular physical queue. Since packets of $X$ can are in different physical queues, it might experience reordering.

\pg{I chose to skip pauses/resume for overflows. I am wondering if we should just say we limit the size of the overflow queue to 1-HopBDP instead.}

Note that we used a single hash table for the switch, instead of keeping multiple hash tables (e.g., 1 per egress port). This is because, splitting the space among different hash tables increases the number of overflows. Our evaluation shows that with our design overflows and the associates reordering are very rare.

\item \emph{Low tail FCTs for short flows:} In RDMA, data center applications send frequent short request-response style messages. Many applications create multiple short flows simultaneously (e.g, map-reduce), the performance of the application is thus tied to the tail FCT of these short flows ~\cite{dean2013tail}.
\item \emph{High Utilization:} Data centers also run applications that initiate big data transfers (e.g., distributed machine learning). For such large transfers, the throughput and hence the utilization of the network is important. Moreover, current data center operators overprovision their networks to avoid congestion, wasting expensive resources. With improved CC, data center operators can run their network at higher loads, increasing resource utilization.

it would be infeasible to keep and reference per-flow state for the hundreds of thousands of flows that traverse
a switch each second. The new CC schemes should be deployable on existing hardware (NIC and switches) without requiring intrusive modifications. In particular, the overhead of the CC on the network capacity in communicating feedback, computational complexity to calculate the feedback and the switch/NIC's memory for bookkeeping should be minimal and realizable in practice.

We now walk through various design principles that enable \bfc{} to achieve our design goals given the current data center trends.

\noindent\textbf{The need for scheduling at the switches:}
Data center switches can build up significant buffering during heavy congestion (e.g., a high degree incast event). In case the switch is using a single FIFO queue per port, a short flow will have to wait for the packets ahead of it in the queue to be transmitted. This head-of-line blocking can hurt tail FCTs for short flows significantly. Existing switches allready support multiple (24-32) physical FIFO queues per egress port~\cite{portlimit}. By assigning flows to these physical queues and scheduling the queues (e.g., using fair queuing), switches can reduce the FCT for short flows. The choice of the scheduling  policy depends on the requirements of the data center operators, e.g., in multi-tenant environment operators might want to use hierarchical fair queuing to ensure fairness among different tenants, while also doing fair queuing for flows from the same tenant to improve FCT for short flows of the tenant. Alternatively, if a data center operator only cares about reducing FCTs in aggregate, they might use shortest flow first (or it's practical approximation ~\cite{homa,pfabric}). \bfc{} supports arbitrary scheduling policies with the constraint that, at any given time, all the packets in the buffer from a flow are in the same FIFO queue and are in order. This implies that \bfc{} can support fair queuing, hierarchical fair queuing and priorities but cannot support approximate fair queuing (AFQ ~\cite{afq}) where packets from a flow can be in multiple queues. In our implementation of \bfc{}, we used fair queuing.

\noindent\textbf{The need for selective pushback:}
Existing CC algorithms adjust the rate of a flow based on the congestion feedback from the switches. The delayed feedback from switches implies that existing schemes react on an end-to-end RTT scale and might be too slow on high speeds links or for workloads with smaller flows. The flows might overflow the switch buffer during congestion episodes, potentially causing excessive packet drops. Existing CC schemes either use pushback mechanisms like PFC to reduce such drops and/or use smart retransmission strategies like Improved ROCE NIC (IRN ~\cite{irn}) to reduce the overhead of retransmissions. 

Compared to Go-Back-N, IRN's improved retransmission reduces performance degradation during drops but doesn't alleviate it entirely. The retransmissions in IRN will still consume bandwidth decreasing overall utilization. On the other hand, since PFC's push back mechanism works on a hop-by-hop RTT scale, it can control buffer sizes better compared to the CC mechanisms at the NIC, reducing drops significantly. Having said that, PFC pauses all the flows from an incoming link (at a given priority) even if most of them are not causing congestion at the downstream switch. By pausing flows not causing congestion, PFC increases their FCTs. Moreover, PFC pauses can stop all the traffic on a link, causing underutilization.

Therefore, to limit the buffer occupancy without incurring HoL blocking or underutilization, we need a fast pushback mechanism at the switches that only ``selectively'' pauses incoming flows causing congestion.


\noindent\textbf{Using the physical queues efficiently:}
Ideally, per flow pausing could limit buffer occupancy without introducing HoL blocking. One way to achieve this would be to assign each flow to a separate physical queue at all the egress ports along the path. With per flow queues, if a particular flow starts to build excessive buffering, the switch can signal the upstream to pause only the particular flow without causing HoL blocking for other flows. While in theory, such a solution could work, in practice it's not realizable. First, existing switches only support a limited number of physical queues per port, this is because scheduling across a larger number of queues at line rate is challenging ~\cite{pifo}. Second, such a solution requires per-flow state, updating per-flow state at line rate on high capacity switches is also not realizable on existing hardware. The problem is that looking up state of a flow requires $O(log(n))$ operations, where n is the number of active flows at the switch. Modern switches have a strict time budget of only 10s of ns to process a packet. If the look up for a flow takes longer than that, then, it might slow down the switch's pipeline reducing utilization. 

Alternatively, consider the following strawman proposal for selective pushback that only uses a limited number of physical queues and doesn't require per flow state. The switches do consistent SFQ at the egress ports, i.e a flow gets mapped to the same physical queue ID across all egress ports on the path. For each physical queue ID, switches maintain the amount of buffering from each upstream switch. In case the flows from a particular upstream switch (U) at a given physicalID (pid) are building excessive buffering, the switch signals U to pause pid. While at a first glance such a solution might seem reasonable, it can introduce significant HoL blocking. In this proposal, two flows might get mapped to the same physical queue even if there are unused physical queues in the system. E.g., consider an egress port with 32 physical queues and 10 active flows, the expected fraction of flows sharing the same physical queue at the port is given by $\frac{^{10}C_2}{32 \cdot 10}$ = 0.14!. So even if the number of active flows is only one-third the number of physical queues, a significant fraction of the flow end up sharing the same physical queue.  Such collisions, can pause flows unnecessarily, increasing tail latencies. Moreover, in addition to HoL blocking from pauses, collisions in the physical queue can also degrade benefits from scheduling, hurting FCTs. E.g., if a short flow gets mapped to a physical queue already containing packets from other flows, then the short flow's throughput will be below it's fair share, increasing the FCT. In our evaluation, we compare the straw proposal against \bfc{} (see \Fig{indirection}). The strawman proposal doesn't use physical queues efficiently and has frequent collisions, resulting in 15 $\times$ higher FCTs for short flows.


In \bfc{}, switches track a limited number of flows with packets in the buffer. To enable fast look ups for state corresponding to a flow ($O(1)$), switches maps each flow to a <virtual queue, ingress port, egress port>  tuple, the ``VFID'' (virtual flow ID). Switches communicate pauses for virtual flows on the virtual queue space. The virtual queue for a flow is same across all the switches and is computed using the hash of the flow's 5 tuple. At a given switch, flows mapped to the same VFID are treated as if they were a single flow. Since, the only limit on the number of virtual queues in the space required to store the state, the number of virtual queues can be very large, as a result the fraction of flows sharing the same virtual queue are very small, reducing HoL blocking due to pauses. 

For each virtual flow, the switch records the number of packets in the buffer. When an empty virtual flow (VFID without any packets in the buffer) receives a packet, the switch maps it to an unused physical queue at the corresponding egress port, if there is one. Otherwise, the virtua flow is mapped to a random physical queue at the egress port.  When a packet arrives, the switch looks up the physical queue associated with the packet's VFID, and enqueues the packet in the corresponding physical queue. The physical queue assignment in \bfc{} ensures that two virtual flows will never share the same physical queue at an egress port, if the number of active virtual flows (VFIDs with packets in the buffer) are lesser than the number of physical queues. By doing so, \bfc{} reduces collisions significantly. Our evaluation shows that in \bfc{} the collisions in the physical queue are rare.

In \bfc{}, switches pause virtual flows and communicate pauses on the virtual queue space. If a given virtual flow at a switch builds up enough buffering, then the switch sends a pause on the it's virtual queue at the upstream switch (identified by the ingress port) associated with the VFID. At each egress port, the switch keeps track of the virtual queue of the packet at the head of each physical queue. On receiving a pause for a virtual queue from a downstream switch, the switch pauses all such physical queues at the egress port it received the pause from. The pause and the resume threshold is same for a given virtual flow and is set to a small value for which the associated physical queue doesn't run out of packets due to pauses. Switches communicate the set of paused virtual queues periodically using a bloom filter. 

The net effect is reduced tail buffering and low HoL blocking due to pauses. The design of \bfc{} enables it to achieve better FCTs compared to the existing schemes. We now present the design of \bfc{} in detail.


\subsection{Virtual space indirection} 
To assign physical queues to flows efficiently and to generate pauses selectively, \bfc{} maintains an approximation of per-flow state to keep track of: 1) the physical queue assigned to the flow; 2) the number of packets in the buffer; 3) whether the flow is paused at the upstream or not. Moreover, state lookups should be fast ($O(1)$), so that the switch can operate at line rate. To achieve this, \bfc{} maps flows to a virtual flow ID (VFID). The rational is if the virtual flow ID space is big enough then the fraction of active flows (flows with packets in the buffer) sharing the same VFID will be small, this way \bfc{} can approximately keep track of the state associated with each active flow. Flows mapped to the same VFID are treated as a single flow and referred as virtual flow from hereon.

Side note: For now we will assume that state associated with each virtual flow is stored in an array (indexed by the VFID), allowing fast look ups at line rate. Later we will show that using an array is space inefficient as most of the VFIDs would be empty (i.e., won't have packets in the buffer). Then, we will present a way of storing the virtual flow entries using a hash table, that is both space efficient and allows fast lookups (still $O(1)$).

An important thing to note while mapping flows to VFIDs at a switch: two flows going through different egress ports should have different physical queue assignments based on their egress ports. This implies that at a switch, two flows going through different egress ports shouldn't map to the same VFID. Similarly, two flows coming from different ingress ports shouldn't have the same VFID. This is because, to pause a given virtual flow, \bfc{} sends a directed pause to the corresponding upstream switch of the flow (identified by ingress port of the VFID). Sending the pause to all the upstreams can pause flows unnecessarily. As a result, the VFID for a flow is given by the following tuple <virtual queue, ingress port, egress port>. This implies flows with different ingress or egress port will have different VFIDs. The virtual queue corresponding to a flow is same across all the switches on the path and is calculated by taking a hash of the flow's 5-tuple. This consistency is important for pausing as we will see shortly.

A flow can have different VFIDs at different switches along it's path, as the ingress and egress port at each switch can be different. To pause flows mapped to a virtual flow $X$ at the upstream, a switch $S$ communicates only the virtual queue $VQ$ of the virtual flow $X$ to the upstream. This is done as the upstream switch doesn't know the egress port of a flow at switch $S$, hence it cannot identify flows with VFID $X$ at switch $S$. So the switches, instead communicates pauses/resumes on the virtual queue $VQ$ associated with the virtual flow $X$. A caveat is that to ensure that a paused virtual flow doesn't receive further packets, a switch sends resume on a virtual queue $VQ$ at upstream switch $US$, only if all virtual flows with the virtual queue $VQ$ coming from the upstream stream switch $US$ are unpaused.

On receiving a pause for a particular virtual queue $VQ$, the upstream switch (at the egress port where it received the pause from) pauses all the physical queue where the virtual queue of the packet at the head is $VQ$. The consistency in mapping to virtual queue ensures that the upstream switch pauses all flows mapped to the VFID $X$ at switch $S$. Having said that, the flows at a given egress port can incur HoL blocking due to pauses from a downstream if they share the same virtual queue. Since the virtual queue space is large, the probability of collisions is low, hence, such HoL blocking is minimal. Pauses in \bfc{} can also cause HoL blocking when the different virtual flows share the same physical queue, pausing flows unnecessarily. We now describe \bfc{}'s physical queue assignment to reduce collisions in the physical queue. 

\subsection{Assigning physical queues}

When an empty virtual flow (i.e. virtual flow without packets in the buffer) gets a packet, the switch assigns it a physical queue at the corresponding egress port. The switch keeps track of empty physical queues at each port. If the egress port contains empty physical queues, the switch assigns an empty physical queue. Otherwise, the switch assigns a physical queue at the egress port randomly. The first packet and the subsequent incoming packets for the virtual flow are then enqueued in the corresponding physical queue. This implies that, in \bfc{} the packets from two virtual flows will not share the same physical queue if the number of active virtual flows at an egress port is less than the number of physical queues at that port. Note that if a virtual flow runs out of packets and becomes inactive, then it's mapping to the physical queue is destroyed, freeing up the physical queue to be used by other virtual flows. This also implies that when the virtual flow becomes active again the switch can assign it some other empty physical queue if possible. 

Moreover, since physical queues are FIFO in nature, and all the packets for an active virtual flow are enqueued in the same physical queue, the packets for a given virtual flow (and the corresponding physical flows) are always dequeued in order. This is important as reordering can trigger retransmissions. Next we describe, how does a switch decide when to pauses/resume a virtual flow.

\fi

==> design_sigcomm.tex <==
\section{Design}
\label{s:design}
Our goal is to design a practical system for per-hop, per-flow flow control for data center networks. We first describe the constraints on our design (\S\ref{s:design_goals}). We then sketch a plausible strawman proposal  that surprisingly turns out to not work well at all (\S\ref{s:strawman}), and we use that as motivation for our design (\S\ref{s:bfc_overview}).


\begin{figure}[t]
    \vspace{-5.5mm}
     \centering
    \includegraphics[trim= 0.25cm 0.5cm 0.25cm 1.5cm, clip, width=\columnwidth]{images_nsdi21/bfc_design.pdf}
    \vspace{-13mm}
    \caption{\small Logical switch components in per-hop, per-flow flow control.}
    \label{fig:design_diagram}
    \vspace{-6mm}
 \end{figure}
 
\subsection{Design Constraints}
\label{s:design_goals}


\Fig{design_diagram} shows the basic components of a per-hop, per-flow flow control scheme (per port). (1) {\em Mapping to physical queues:} When a packet arrives at the switch, the switch routes the packet to an egress port and maps it to a FIFO queue at that port. This assignment of flows to queues must be consistent, that is, respect packet ordering. (2) {\em Backpressure module:} Based on queue occupancy, the switch generates backpressure feedback for some flows and sends it upstream. (3) {\em Scheduler:} The scheduler at each egress port forwards packets from queues while respecting backpressure feedback from the downstream switch. 

ATM per-hop per-flow flow control systems~\cite{anderson1993high,kung1995credit} roughly followed this architecture, but they would be impractical for modern data centers. 
First, they assumed per-flow queues and per-flow state, but modern switches have a 
limited number of queues per egress port~\cite{afq,bosshart2014p4} 
and modest amounts of table memory~\cite{bosshart13, chole2017drmt}. 
In particular, it is not possible to maintain switch state for all live connections.
% , which can easily be in the millions. 
Second, earlier schemes did not attempt to minimize buffer occupancy. 
Instead, they sent backpressure feedback only when the switch was about to run out of buffers. 
On a buffer-constrained switch, this can result in buffer exhaustion\,---\,buffers held by straggler
flows can prevent other flows from using those buffers at a later time.
% hurting performance at a later time.



%Existing per-hop per-flow flow control systems built for ATM~\cite{anderson1993high,kung1995credit} roughly follow this architecture, but they are impractical for modern data centers for several reasons. First, they assume per-flow queues and per-flow state, but modern switches have only a limited number of queues per port (e.g., up to 32 per port~\cite{afq,bosshart2014p4}) 
%and modest amounts of table memory (e.g., a few MBytes~\cite{bosshart13, chole2017drmt}). In particular, it is not possible to maintain state for all the connections sending through a switch, which can easily be in the millions. 


%In other words, the switch admits packets of a flow even after it has sufficient packets from that flow to ensure high utilization,  which can lead to buffer exhaustion at a later time. 


%\smallskip
\noindent\textbf{Hardware assumptions.} Modern data center switches have made strides towards
greater flexibility~~\cite{sivaraman2016programmable,arista}, but they are not infinitely malleable and have real resource constraints. We make the following assumptions based on the capabilities of SwitchX.
\begin{CompactEnumerate}
    \item We assume the switch is programmable and supports stateful operations for hundreds of thousands of entries. SwitchX can maintain millions of register entries; the switch supports simple constant-time per-packet operations to update the state at line rate~\cite{domino}.
    \item The switch has a limited number of FIFO queues per egress port, meaning that flows must be multiplexed onto queues. SwitchX has 32 queues per 100G port and 128 per 400G port.
    The assignment of flows to queues is programmable. The scheduler can use deficit round-robin
    or priorities among queues, but packets within a queue are forwarded in FIFO order.
    \item Each queue can be independently paused and resumed without slowing down forwarding from other queues. However, when we pause a queue, that pauses {\em all} of the flows assigned to that queue.
    %In other words, head-of-line blocking is an inherent challenge caused by hardware design constraints; we cannot assume that the switch scheduler can pick arbitrarily from any of a large number of queued flows, in constant time. 
    \item The switch can pause/resume each queue separately from the (programmable) dataplane. Earlier switches can pause/resume individual queues, but only from the control plane. This is likely too slow for effective hop-by-hop control. In contrast, SwitchX allows for fast, programmable pause/resume scheduling from the dataplane itself.
    
    %Our goal here is a design that should be feasible to implement on a new generation of switches that will have the desired capability given the existing technology trends. For example, given the trend in programmable packet processing~\cite{sivaraman2016programmable,arista}, we believe flexible scheduling from the data plane will be available in the next generation of switches. 
    
    %\item We assume a programmable switch that supports stateful operations for tens of thousands of flows. This is consistent with the capabilities of existing switches. For example, NetCache~\cite{jin2017netcache} demonstrated an implementation on Tofino that maintains state for 64K items. Additionally, we assume the switch supports standard per-packet operations to update the state at line rate~\cite{domino}.
\end{CompactEnumerate}
 

%\smallskip
%\noindent
%\textbf{Strawman proposal:}

\subsection{A Strawman Proposal}
\label{s:strawman}

We originally thought stochastic fair queueing~\cite{sfq} with per-queue backpressure would meet our goals. Use a hash function on the flow header to consistently 
assign the packets of each flow to a randomly-chosen FIFO queue at its egress port. 
For simplicity, use the same hash function at each switch. Pause a queue whenever its buffer
exceeds the 1-hop bandwidth-delay product (BDP). 
%Above this point,we would (likely) have time to signal the upstream switch to resume sending before the queue completely drained.

\cut{
that way, when we pause a flow at an upstream switch, we pause all of the flows
that would share the same downstream queue. a flow is assigned to the same FIFO queue at all the switches on its path (assume the queues at each egress port are numbered). In order to generate pauses, for each queue, we maintain the amount of buffering in the switch from each incoming ingress port. We selectively pause a queue (at the upstream switch) if the amount of buffering of the queue from the corresponding ingress port becomes too large, 
e.g., one 1-hop bandwidth-delay product. Above this point,
we would (likely) have time to signal the upstream switch to resume sending before the queue completely drained.
Of course, there could be contention at the upstream switch that would prevent the queue from refilling quickly enough,
but let us leave that aside for the moment.
}

%When we need to pause a queue because a particular flow is consuming too much buffer, we need to pause all flows sharing the same FIFO queue at the upstream switch of the flow. Unlike traditional PFC, pauses in the strawman only affect flows that map to the same queue; flows in other queues can continue to be forwarded downstream and scheduled out of the switch.

This strawman needs only a small amount of state for generating the backpressure feedback and no state for queue assignment. It seems like we should be done, and this paper could be short.  However, the strawman proposal does not work well. With even a modest number of active flows,
there is a significant chance that any specific flow will land in an already-occupied FIFO queue. These collisions hurt latency for two reasons: (1) The packets for the flow will be delayed behind unrelated packets from other flows; for example, a short flow may land behind a long flow. (2) Queue sharing can cause HoL-blocking. If a particular flow is paused (because it is congested downstream), all flows sharing the same queue will be delayed. Furthermore, these delays can cause cascading pauses further upstream.  

\cut{If we need to pause a queue at the upstream (in response to a particular flow filling up the queue), any flow at any upstream switch that hashes to the same queue will potentially be affected by the pause. In other words, the pause due to a particular flow will propagate upstream
to affect other flows with the same hash value, even if they have different downstream routes. This ``cascading HoL-blocking'' is worse when a flow shares the queue with another flow experiencing heavy congestion (\eg a flow belonging to an incast), causing the queue to be paused for long durations. }

These problems occur with stochastic fair queueing even when we have enough physical resources
to give each active flow its own dedicated FIFO queue. We define an \emph{active} flow as one with 
queued packets at the switch. The birthday paradox~\cite{birthday_paradox} implies stochastic collisions between
active flows will be frequent. For example, when five active flows are assigned to 32 FIFO queues, the chance that at least two flows will be randomly assigned to the same queue is 28\%. 
%In this case, when a new flow arrives, the probability that it will share a queue with an existing flow is $\big(1 - (\frac{31}{32})^{5}\big)$ or 15\%! 
Further, a flow going through multiple switches can experience such collisions at each of its hops. Since data center operators care about tail latency (95$^{\text{th}}$ or 99$^{\text{th}}$ percentile), avoiding collisions, even to a small percentage of flows, is important. Moreover, collisions slow down flows and increase the number of active flows, driving up the collisions further.

To prevent collisions from affecting tail latency performance, the strawman requires significantly more queues than active flows. For example, at an egress port with $n$ active flows, to achieve fewer than 1\% collisions, we would need roughly 100$n$ queues.

%such a high collision probability will hurt tail latency significantly. As a result, the strawman requires a much large number of queues than flows to avoid Hol-blocking. \ma{The argument here about tail latency should be made more precise, at least with a good numerical example}



\subsection{Backpressure Flow Control (BFC)}
\label{s:bfc_overview}

Our design achieves the following properties:

\smallskip
\noindent\textbf{Minimal HoL-blocking:}
We assign flows to queues dynamically. As long as the number of active flows at an egress is less than the
number of queues, (with high probability) no two flows share a queue and there is no HoL-blocking. When a new flow arrives at the switch, it is assigned to an empty queue if one is available, sharing
queues only if all are in use.
% A newly active flow shares a queue with previous flows only if all the queues are in use. 
%(\pg{We actually assign a new flow to an empty and unpaused queue}) 
%To enable this flexible queue assignment, BFC pauses individual flows rather than queues. By decoupling the pause signal from queue assignment, BFC enables each switch to map an incoming flow to any empty queue, thereby avoiding unnecessary collisions.

%\noindent{\bf Reduce buffering without underutilization (\Sec{backpressure}):} BFC pauses a flow when the queue occupancy exceeds a small threshold. BFC's pause threshold is set aggressively to reduce buffering. In schemes like PFC, pausing aggressively would hurt link utilization, but BFC \pg{strives to} only pauses flows causing congestion (except in extreme scenarios). \ma{The last two sentences are a bit hand-wavy. Maybe we can cut from here and just say: BFC's pause threshold is set aggressively to reduce buffering while maintaining just enough packets in the queue to avoid underutilization.} \pg{Sadly the latter statement in not true with the new pausing strategy. See Pause threshold subheading in \S\ref{s:backpressure}. One option is to remove this as a design property. Second is to remove ``just'' from the framing.} The remaining flows can continue transmitting avoiding unnecessary underutilization. BFC's pausing mechanism is compatible with any scheduling policy (\eg fair queuing, hierarchical fair queuing, round robin etc.). For concreteness, we constrain our discussion to fair queuing.

\smallskip
\noindent{\bf Low buffering and high utilization:} BFC pauses a flow at the upstream when the queue occupancy exceeds a small threshold. BFC's pause threshold is set aggressively to reduce buffering. With a blanket pause system like PFC, pausing aggressively hurts link utilization, but BFC only pauses those flows causing congestion (except when collisions occur). The remaining flows at the upstream can continue transmitting, avoiding under-utilization. BFC's pausing mechanism is compatible with any scheduling policy (\eg priorities, hierarchical fair queuing, etc.). For concreteness, we constrain our discussion to fair queuing.


%BFC aims to store the minimum number of packets needed to keep downstream links busy, consistent with the switch's scheduling policy. In particular, BFC maintains just enough packets from each flow so that it can resume that flow at the upstream before running out of packets from it. BFC's pausing mechanism is compatible with any scheduling policy (\eg fair queuing, hierarchical fair queuing, round robin etc.). For concreteness, we constrain our discussion to fair queuing.

%aims at maintaining the minimum amount of buffering required to without a queue running out of packets due to pauses at the upstream. The pausing mechanism is orthogonal to the scheduling policy at the switches, and BFC can support a number of scheduling policies (\eg fair queuing, hierarchical fair queuing, round robin etc.). For concreteness, we will restrain our discussion to fair queuing.

\smallskip
\noindent\textbf{Hardware Feasibility:}  
%In contrast to prior schemes, BFC only maintains state for active flows -- flows with packets in the switch buffer -- reducing the memory requirement significantly. Additionally, to allow efficient lookup of the state associated with a flow, the state is stored in a flow table, an array indexed using hash of the flow identifier. The size of the flow table is limited (proportional to physical queues in the switch) and uses only a fraction of the dedicated stateful table memory (\eg < 8\% in SwitchX). Further, the operations for generating backpressure and reacting to it are simple. BFC's per packet operations can be implemented entirely in the dataplane at line rate.
%
BFC does not require per-flow state, and instead uses an amount of memory proportional to the number of physical queues in the switch. To allow efficient lookup of the state associated with a flow, the state is stored in a flow table, an array indexed using a hash of the flow identifier. The size of this array is set in proportion to the number of physical queues. In our SwitchX implementation, it consumes less than 10\% of the dedicated stateful memory. Critically, the mechanism for generating backpressure and reacting to it is simple and the associated operations can be implemented entirely in the dataplane at line rate.
%\Further, the operations for generating backpressure and reacting to it are simple and can be implemented entirely in the dataplane at line rate.

\smallskip
\noindent\textbf{Generality:} BFC does not make assumptions about the network topology or where congestion occurs in the network. By contrast, schemes like NDP~\cite{ndp}, pHost~\cite{phost} and Homa~\cite{homa} assume sufficient core network bandwidth and congestion is only at the last hop. Furthermore, unlike pFabric~\cite{pfabric} and Homa~\cite{homa}, BFC does not assume knowledge about flow sizes or deadlines. 
Such information can be incorporated into BFC's design to improve small flow performance (\App{impact_srf}), at a cost in deployability.

\smallskip
\noindent\textbf{Idempotent state:} Because fiber packets can be corrupted in flight~\cite{pktcorrupt}, BFC ensures that pause and resume state is maintained idempotently, 
in a manner resilient to packet loss.

%While such assumptions can be incorporated in BFC's design to achieve better performance (\eg using flow size for shortest-remaining-flow-first scheduling \App{impact_srf}), they limit BFC's operation regime. 

\noindent

\if 0

BFC has two additional properties, easing deployment:

\begin{itemize}
\item{In-order packet delivery:} BFC schedules packets from the same flow out the egress
port in the same order that they arrived at the switch ingress, and simplifies packet handling at the
destination server.

\item{Minimal configuration:}
While it is possible to auto-tune parameters, BFC has simpler and more intuitive configuration, that is more likely to work robustly across rapidly evolving workloads and topologies.
\end{itemize}

Providing a design that achieves these properties, along with an evaluation of how this general approach
affects performance, are the principal contributions of this work.

\fi %

%\input{table.tex}


%Table~\ref{tab:functionality} outlines the main components of BFC.

\subsubsection{Assigning flows to queues}
\label{s:qassignment}

To minimize sharing of queues and HoL-blocking, 
we dynamically assign flows to empty queues. 
As long as the flow is active (has packets queued at the switch), 
subsequent packets for that flow will be placed into the same FIFO queue. 
Each flow has a unique 5-tuple of the source and destination addresses, 
port numbers, and protocol; we call this the
flow identifier (FID). BFC uses the hash of the FID to track a flow's queue assignment.
To simplify locating an empty queue, BFC maintains a bit map of empty queues. When the
last packet in a queue is scheduled, BFC resets the corresponding bit for that queue.


With dynamic queue assignment, a flow can be assigned to different queues at different switches. To pause a flow, BFC
pauses the queue the flow came from at the upstream
switch (called the upstream queue).  The pause applies to all flows sharing the same upstream queue with the paused flow. We describe the pause mechanism in detail in \Sec{backpressure}.
The packet scheduler uses deficit round robin to implement fair queueing, among the  queues that
are not paused.
% When multiple flows are assigned to a  queue, we do not guarantee fair queueing among those flows.


%BFC pauses are signalled using the FID, but a pause applies to all flows sharing the same upstream queue with a paused flow.
\cut{As a result, in BFC pauses can't be generated based on queue number. Instead, a BFC switch pauses a flow at the upstream using the FID. Unlike the strawman, the queue assignment and pausing mechanism are decoupled. This implies that a flow in BFC will incur no HoL-blocking at an egress port (i.e., a flow will not share a queue with other flows), if the number of active flows at the port is less than the number of physical queues at the port.}



Since there is a limited number of queues, it is possible that all queues have
been allocated when a new flow arrives, at which point HoL-blocking is unavoidable.
For hardware simplicity, we assign the flow to a random queue in this case.
Packets assigned to the same queue are scheduled in FIFO order.

% we could leave this in but its extra space
% We could be more sophisticated, for example, by assigning the flow to the shortest queue (such an operation requires finding the minimum in an array). In practice, however, this would make little difference since such situations are infrequent with even a modest number of queues.% as we explain next.

\begin{figure}[t]
     \centering
     %\vspace{-1mm}
    \includegraphics[trim={0 0 0 4mm},clip,width=0.8\columnwidth]{images_nsdi21/number_of_active.pdf}
    \vspace{-5mm}
    \caption{\small Number of active flows versus aggregate load on a single 100\,Gbps link. Flow sizes are derived from the Facebook distribution, with Poisson flow arrivals.}
    \label{fig:number_of_active}
    \vspace{-6mm}
 \end{figure}
 
BFC incurs collisions only when the number of \emph{active flows} i.e., flows with packets in the switch, exceeds the number of queues at an egress port. (Note that the total number of connections (including idle flows) traversing the port may be much higher.)
A fundamental result of queueing theory is that the number of active flows at a fair queued
switch is surprisingly small, even at high load~\cite{kleinrock1976queueing, kortebi2005evaluating}. 
In particular, for an M/G/1-PS (Processor Sharing) queue with Poisson flow arrivals operating at average load $\rho < 1$, the number of active flows has a geometric distribution with mean $\frac{\rho}{1-\rho}$, independent of the link speed or the flow size distribution. Therefore, even at load $\rho=0.95$, the expected number of active flows is only 19. To illustrate this result in practice, \Fig{number_of_active} shows the cumulative distribution of the number of active flows 
for BFC at an egress port, with a workload using the Facebook flow size distribution and Poisson flow arrivals. We see that at 95\% load, the number of active flows is at most $\sim$30. The high-level intuition is that in a fair-queuing system, each flow gets equal service, and therefore a large, congested flow cannot disproportionately slow down other flows. By contrast, in a FIFO system, a single large flow can prevent service for many small flows, thereby sharply increasing the number of active flows. 
%See \Sec{discussion} for more details.

%Consider flows arriving as a Poisson process to a switch port running fair queuing. This can be modeled as a M/G/1-PS (Processor Sharing) queue. For a M/G/1-PS queue, if the average load is $\rho$, then the number of backlogged flows has a geometric distribution with mean $\frac{\rho}{1-\rho}$~\cite{kleinrock1976queueing}. Therefore, even at a high load of $\rho=0.9$, the expected number of backlogged flows is only 9. Note that the distribution of the number of backlogged flows in this model is independent of the flow size distribution and the link speed. In particular, at the same load $\rho$, increasing link speed does not imply an increase in the number of flows (and therefore collisions in BFC). 

% The number of such flows will be much smaller than all connections (including dormant ones) traversing the egress port. More importantly, in a system like BFC with fair-queuing scheduling, the number of active flows is often surprisingly small, even at high levels of load. As an example, \Fig{number_of_active} shows the cumulative distribution of the number of active flows for BFC at an egress port, with a workload using the Facebook flow size distribution and Poisson flow arrivals. We see that, even at 95\% load, the number of active flows is at most $\sim$30. Queuing theory shows that for Poisson flow arrivals, the number of active flows is small for any flow size distribution and link speed~\cite{kleinrock1976queueing} (see \Sec{discussion} for more details).  The high-level intuition is that in a fair-queuing system, each flow gets equal service, and therefore a large, congested flow cannot disproportionately slow down other flows. By contrast, in a FIFO system, a single large flow can prevent service for many small flows, thereby sharply increasing the number of active flows. Prior work has made similar observations about the behavior of the number of active flows in queuing systems with fair bandwidth sharing policies like fair queuing~\cite{kortebi2005evaluating}. 

%\Fig{number_of_active} shows the cumulative distribution of the number of active flows at an egress port with varying load. 

Of course, the number of active flows can still exceed the number of queues in settings with bursty flow arrivals (\eg incast). BFC incurs some HoL-blocking in such scenarios, but it
still outperforms prior approaches even in these extreme cases (see \S\ref{s:limits}). In particular, in case of an incast, BFC can leverage the large number of upstream queues feeding traffic to a switch to limit congestion spreading. The observation is that, when flows involved in an incast are spread among multiple upstream ports, BFC can assign these flows to separate queues at those ports, as long as the total number of flows does not exceed the total number of queues across {\em all} of the upstream ports. In such cases, BFC will not incur HoL-blocking at the upstream switches. As the size of the network increases and the fan-in to each switch gets larger, there will be even more queues at the upstream switches to absorb an incast, further reducing congestion spreading. 

%limiting the spread of HoL-blocking. Further more, in case the incast is large enough to cause HoL-Blocking at the upstream of the last-hop, the upstream could then again levrage the fanin from its upstream queues to
%In cast the incast degree is larger than the number of such upstream queues, there will be collisions, the HoL-blocking can spread from incast . However, each of the upstream egresses (with incast flows) can further leverage the FanIn of their upstream queues to further limit congestion spreading in the higher layers.
%\sout{With BFC, only flows that map to the same queue suffer HoL-blocking, and only with respect to other flows in the same queue. By contrast, with a single FIFO queue, all flows through the congested link suffer delays.}}
% \pg{check}
% \pg{Write an additional line to explain why we perform better. \eg In case of collisions, only flows sharing the queue with congestion suffer HoL-blocking. In contrast, with FIFO all flows sharing the same egress port will suffer HoL-blocking.}





\smallskip
\noindent\textbf{Mechanism:}
To keep track of queue assignment, BFC maintains an array indexed by the egress port of a flow and the hash of the FID. All flows that map to the same index are assigned to the same queue. We maintain the following state per entry: the physical queue assignment (\texttt{\small qAssignment}), and the number of packets in the queue from the flows mapped to this entry (\texttt{\small size}). The pseudocode is as follows (we defer switch-specific implementation issues to \S\ref{s:tofino2}):

\vspace{1mm}
\begin{lstlisting}[basicstyle=\footnotesize]
On Enqueue(packet):
    key = <packet.egressPort, hash(packet.FID)>
    if flowTable[key].size == 0:
        reassignQueue = True:
    flowTable[key].size += 1
    if reassignQueue:
        if empty q available at packet.egressPort:
            qAssignment = emptyQ
        else:
            qAssignment = randomQ
        flowTable[key].qAssignment = qAssignment
    packet.qAssignment = flowTable[key].qAssignment

On Dequeue(packet):
    key = <packet.egressPort, hash(packet.FID)>
    flowTable[key].size -= 1
\end{lstlisting}
\vspace{-1mm}
%The above code ensures ensures that a flow's queue assignment will not change if it has packets in the switch. 


%The above code ensures two things. First, once a flow has been assigned to a queue, all packets from that flow must be assigned to the same queue until all of the packets from that flow have left the switch to prevent reordering the flow's packets. Second, it enables dynamic queue assignment when there are no existing packets in the switch for an index.

In the flow table, if two flows map to the same index they will use the same queue (collision). Since flows going through different egress ports cannot use the same queue, the index also includes the egress port. Index collisions in the flow table can hurt performance. These collisions decrease with the size of the table, but the flow table cannot be arbitrarily large as the switch has a limited stateful memory. In our design, we set the size of the flow table to 100 $\times$ the number of queues in the switch. This ensures that if the number of flows at an egress port is less than the number of queues, then the probability of index collisions is less than 1\%. If the number of flows exceeds the number of queues, then the index collisions do not matter as there will be collisions in the physical queues regardless. SwitchX has 4096 queues in aggregate, and hence the size of the flow table is 409,600 entries, which is less than 10\% of the switch's dedicated stateful memory. 
%SwitchX has 4096 queues in aggregate, and hence the size of the flow table is 409,600 entries, which is well within its capabilities.  %\ma{Have you checked if we're allowed to give all these specific numbers for SwitchX?}\pg{No but he changed exact numbers everywhere else in the paper. Maybe say this instead? For SwitchX, the flow table consumes less than 8\% of the dedicated stateful memory.} \ma{yes that's ok. in general check all the numbers with him. this is the kind of thing that they could be sensitive about in the last minute}

While using an array is not memory efficient, accessing state involves simple operations. Existing solutions for maintaining flow state either involve slower control plane operations, or are more complex~\cite{pontarelli2019flowblaze, barbette2020high}. In the future, if the number of queues increases substantially, we can use these solutions for the flow table, however at the moment, the additional complexity is unnecessary.


\subsubsection{Backpressure mechanism}
\label{s:backpressure}
BFC pauses a flow if the occupancy of the queue assigned to that flow exceeds the pause threshold \emph{$Th$}. To pause/resume a flow, the switch could signal the flow ID to the upstream switch, which can then pause/resume the queue associated with the flow. While this solution is possible in principle, it is difficult to implement on today's programmable switches. The challenge is that, on receiving a pause, the upstream switch needs to perform a reverse lookup to find the queue assigned to the flow and some additional bookkeeping to deal with cases when a queue has packets from multiple flows (some of which might be paused and some not).

We take a different approach. Switches directly signal to the upstream device to pause/resume a specific queue. Each upstream switch/source NIC inserts its local queue number in a special header field called \texttt{\small upstreamQ}. The downstream switch stores this information in the flow table and uses it to pause the queue at the upstream. 
% true but overkill
% This idea of communicating state (i.e., the queue assignment) across switches is similar to {\em dynamic packet state} in CSFQ~\cite{stoica1998core}, where the edge routers encode the rate estimation to be used by the core routers.

\smallskip
\noindent\textbf{Mechanism:} 
%This alone is not enough, even though collisions are not common, there might be situations where a physical queue at the upstream contains multiple flows, potentially going through different egress ports at the downstream. In this case, if any one of these flows sharing the \texttt{\small upstreamQ} is causing congestion at the downstream, we need to pause the \texttt{\small upstreamQ}. 
%\ma{I don't understand why we need the above explanation.. can't we just say, ``To determine when to pause and resume an upstream queue, we use a data structure called Pause Counter.} \pg{That is fine I think, the only reason I had it is to explain the complexity of the problem} To achieve this, we use another datastructure, pause counter. 
Recall that, in general, multiple flows can share a queue even if that is the rare case. 
This has two implications. First,
we track the queue length (and not just the \texttt{\small flowTable.size}) and use that to determine
if the flow's upstream queue should be paused.  Second, each upstream queue can, in general, feed
data into multiple queues at multiple egresses. We pause an upstream queue
if \emph{any} of its flows are assigned a congested queue, and we resume when \emph{none}
of its flows have packets at a congested queue (as measured at the time the packet arrived at
the switch). 
% \pg{I think its fine now, assuming the parenthesis holds for the entire sentence.}
%\pg{(tom): got it), ok now?} \pg{Sorry but this description is maybe not 100\% right, 1) We pause a flow when the packet for it goes to a congested queue. 2) An upstream , sorry if this annoys you imeant my commenting live} \pg{no that's fine - better to catch the errors when I write them} \pg{maybe its fine, I dont like the first point still. The second point is correct.}

We monitor this using a Pause Counter, an array
indexed by the ingress port and the \texttt{\small upstreamQ} of a packet. The upstream queue is paused if
and only if its Pause Counter at the downstream switch is non-zero. On enqueue of a packet, 
if its flow is assigned a queue that exceeds the pause threshold, 
we increment the pause counter at that index by 1. 
When this packet (the one that exceeded $Th$) leaves the switch we decrement the counter by 1. 
Regardless of the number of flows assigned to the \texttt{\small upstreamQ}, 
it will be resumed only once all of its packets that exceeded the pause threshold (when the packet arrived) 
have left the switch. 


% To determine when to pause and resume an upstream queue, we use a data structure called Pause Counter.
% Pause counter is an array indexed by the ingress port and the \texttt{\small upstreamQ} of a packet. The pause counter counts the number of packets in the switch that exceeded the pause threshold on arrival for each index. If the pause counter is greater than 0 for a given index, then the \texttt{\small upstreamQ} associated with the index should be paused, otherwise the queue should be resumed. The pseudo code is as follows.

\vspace{-1mm}
\begin{lstlisting}[basicstyle=\footnotesize,mathescape=true]
On Enqueue(packet):
    key = <packet.ingressPort, packet.upstreamQ>
    if packet.qAssignment.qLength > $Th$:
    if pauseCounter[key] == 0:
            //Pause the queue at upstream
            sendPause(key)
        pauseCounter[key] += 1
        packet.metadata.counterIncr = True
        
On Dequeue(packet):
    key = <packet.ingressPort, packet.upstreamQ>
    if packet.metadata.counterIncr == True:
        pauseCounter[key] -= 1
        if pauseCounter[key] == 0:
            //Resume the queue at upstream
            sendResume(key)
\end{lstlisting}
%\vspace{-1mm}

% On enqueue of a packet, if the queue occupancy exceeds the pause threshold, we increment the pause counter at that index by 1. When this packet (the one that exceeded $Th$) leaves the switch we decrement the counter by 1. On enqueue of a packet, if the queue occupancy exceeds the pause threshold, we increment the pause counter at that index by 1. When this packet (the one that exceeded $Th$) leaves the switch we decrement the counter by 1.
% Regardless of the number of flows assigned to the \texttt{\small upstreamQ}, it will be resumed only if all of its packets that exceeded the pause threshold have left the downstream switch. In particular, it handles the situation where packets from the same \texttt{\small upstreamQ} belonging to different flows reside in multiple queues (possibly at multiple egress ports) at the downstream switch.

% \pg{depending on layout, move this paragraph before the figure to get it to layout on one page}
To minimize bandwidth consumed in sending pause/resumes, we only send a pause packet when the pause counter for an index goes from 0 to 1, and a resume packet when it goes from 1 to 0. For reliability against pause/resume packets being dropped, we also periodically send a bitmap of the queues that should be paused at the upstream (using the pause counter). Additionally, the switch uses a high priority queue for processing the pause/resume packets. This reduces the number of queues available for dynamic queue assignment by 1, but it eliminates performance degradation due to delayed pause/resume packets.



%\pg{In particular, this also handles situations when there are multiple flows at that\texttt{\small upstreamQ} are going through different egress ports at the downstream}
%\pg{In particular, when an upstream queue contains multiple flows that are going through different egress ports at the downstream. The \texttt{\small upstreamQ} will be resumed only when the downstream switch has drained all the packets that exceeded $Th$ from the \texttt{\small upstreamQ}.}


The memory required for the pause counter is small compared to the flow table. For example, if each upstream switch has 128 queues per egress port, then for a 32-port downstream switch, the pause counter is 4096 entries.


%The memory required for the pause counter is smaller compared to the flow table. In particular, we assume that each upstream can have up to 1000 physical queues\footnote{If the upstream has more queues, then the upstream can simply mark (queue assignment \% 1000) as the local queue assignment on the packet.}. \ma{I don't think we need to assume 1000. Just give this as an example. For example, if the upstream switch has 1000.... Also I'd cut the footnote -- it's weird to have queues but pause multiple of them simultaneously} For a 32 port switch, the pause counter is 32,000 entries. 

\if 0
A detail is that the host NIC must be engineered to accept
pause resume packets, to avoid potentially overfilling the
first level switch. \pg{\sout{In contrast to hardware-based transport schemes like DCQCN and HPCC, the NIC operations are simpler and require fewer computation cycles.}} \ma{Perhaps move this discussion of the NIC to the discussion section that comes later}
\fi
%We assume the NIC has sufficient hardware to maintain a queue per flow, simplifying the logic. Note that this assumption is implicit in other hardware-based transport schemes like DCQCN and HPCC,  as they require the ability to set per flow rate/window at the NIC. 


%BFC user per-flow pauses as a backpressure signal. At each ingress link, the switch periodically sends the set of paused flows to the upstream every $\tau$ seconds via a bloom filter (e.g., $\tau = 1$~$\mu$s in our experiments). On receiving a pause for a flow, the switch pauses the physical queue associated with the flow.

\smallskip
\noindent\textbf{Pause threshold.}
BFC treats any queue buildup as a sign of congestion. BFC sets the pause threshold $Th$ to 1-Hop BDP
at the queue drain rate.
\cut{BFC treats any queue buildup as a sign of congestion. BFC sets the pause threshold $Th$ to 1-Hop BDP
at the egress drain rate. In other words a queue can build up at most 1-Hop RTT ($HRTT$) 
of buffering before BFC triggers a pause. More often, when a link is congested, there will be multiple
non-empty queues, and BFC pauses more aggressively. \pg{still wrong I think, regardless the threshold is 1 -hop bdp at egress queue drain rate mean buffering is 1HRTT at queue drain rate}}
% \pg{\sout{but typically BFC will trigger pauses much earlier than that.} This is wrong I think?}
%
%to reduce the queue length. 
%
%\ma{repetitive} \sout{Since BFC selectively pauses upstream queues causing congestion, we are able to set a much smaller threshold $Th$ for pausing compared to PFC. In particular,}
%
% To calculate the pause threshold we first compute the rate at which the queue is draining. 
Let $N_{active}$ be the number of {\em active queues} at an egress, i.e. queues with data to transmit that are not paused, $HRTT$ be the 1-Hop RTT to the upstream, and $\mu$ be the port capacity. Assuming fair queuing as the scheduling policy, the average drain rate for a queue at the egress is $\mu/N_{active}$. The pause threshold $Th$ is thus given by  $(HRTT) \cdot (\mu / N_{active})$. 
% Note that $Th$ is not a constant and 
When the number of active queues increases, $Th$ decreases. In asymmetric topologies, egress ports can have different link speeds; as a result, we calculate a different pause threshold for every egress based on its speed. Similarly, ingress ports can have different 1-Hop RTTs.
Since a queue can have packets from different ingresses, 
% we can not use a single $HRTT$ value for $Th$. Instead, 
we use the max of $HRTT$ across all the ingresses to calculate $Th$. 
We use a pre-configured match-action table indexed with $N_{active}$ and $\mu$ to compute $Th$. 

% \pg{Is the discussion that follows hard to understand? In particular the upstream/downstream stuff might be confusing. I also feel that we are using the downstream incorrectly, the downstream switch should just be switch? But IDK, I am wrong?}\pg{(tom)I think its ok}

BFC does not guarantee that a flow will never run out of packets due to pausing. First, a flow can be paused unnecessarily if it is sharing its upstream queue with other paused flows. 
Second, a switch only resumes an upstream queue once all its packets (that exceeded the pause threshold when they arrived) have left the downstream switch. Since the resume takes an $HRTT$ to take effect, a flow can run out of packets at the downstream switch for an $HRTT$, potentially hurting utilization. However, this scenario is unlikely\,---\,a pause only occurs when a queue builds up, typically because multiple flows are competing for the same egress port. In this case, the 
other flows at the egress will have packets to occupy the link, preventing under-utilization. 

We might reduce the (small) chance of under-utilization by resuming the upstream queue earlier, for example, when a flow's queue at the downstream drops below $Th$, or more precisely, when \emph{every} 
queue (with a flow
from the same upstream queue) drops below $Th$.
% Recall that there can be multiple flows from the same \texttt{\small upstreamQ} to different egress ports 
% and queues at the downstream switch. We should only resume the \texttt{\small upstreamQ} if the queue lengths
% for all flows from the same \texttt{\small upstreamQ} are below $Th$. 
Achieving this would require 
% us to keep track of all the queues that have a packet from a given \texttt{\small upstreamQ}, 
extra bookkeeping, complicating the design. 

Increasing the pause threshold would reduce the number of pause/resumes generated,
% and further reduces cases where a flow unnecessarily runs out of packets, 
but only at the expense of increased buffering (\Fig{qdepth}). In \App{impact_th}, we analyze the impact of $Th$ on under-utilization and peak buffer occupancy in a simple model, and we show that a flow runs out of packets at most 20\% of the time when $Th$ is set to 1-hop BDP. Our evaluation results show that BFC achieves much better throughput than this worst case in practice (Table~\ref{tab:mot_bfc_noincast}, \S\ref{s:eval}).

\smallskip
\noindent\textbf{Sticky queue assignment:} 
Using \texttt{\small upstreamQ} for pausing flows poses a challenge. Since a switch does not know the current queue assignment of a flow at the upstream, it uses the \texttt{\small upstreamQ} conveyed by the last packet of the flow to pause a queue. However, if a flow runs out of packets at the upstream switch (e.g., because it was 
bottlenecked at the downstream switch but not the upstream), then its queue assignment may change for subsequent packets, causing it to temporarily evade the pause signal sent by the downstream switch. Such a flow will be paused again when the downstream receives packets with 
the new \texttt{\small upstreamQ}. The old queue will likewise be unpaused
when its last packet (that exceeded $Th$) departs the downstream switch.

To reduce the impact of such queue assignment changes, we add a timestamp to the flow table state,
% This \texttt{\small timestamp} is 
updated whenever a packet is enqueued or dequeued. A new queue assignment only happens if the \texttt{\small size} value in the flow table is 0, and the timestamp is older than a ``sticky threshold'' (\ie the entry in the flow table has had no packets in the switch for at least this threshold). Since with BFC's backpressure mechanism a flow can run out of packets for an $HRTT$, we set the sticky threshold to a small multiple of $HRTT$ (2 $HRTT$). 
% true but a tangent
% Increasing the sticky threshold affects BFC's ability to use queues efficiently. For example, if the sticky threshold is infinity, all the flows mapped to same index in the flow table will always use the same queue, and BFC would thus be reduced to the strawman proposal.

While sticky queue assignments reduce the chance that a backlogged flow will change queues, it doesn't completely eliminate it (\eg packets from the same flow may arrive slower than this interval due to an earlier bottleneck).
% . If the upstream switch is receiving packets from a flow slowly 
% (\eg when the flow is bottlenecked earlier in the network), then the flow's queue assignment can change. 
Such situations are rare, and we found that BFC performs nearly identically to an ideal (but impractical) variant that pauses flows directly using the flow ID without sticky queue assignments. 
% \pg{I think its overkill which is why I dropped it}
%\pg{Should we say: Increasing the sticky threshold affects BFC's ability to use queues efficiently. E.g., if the sticky threshold is infinity, all the flows mapped to same index in the flow table will always use the same queue, BFC is thus reduced to the strawman proposal.}











\cut{
\smallskip
\noindent\textbf{Pause threshold.} The goal for pausing in \bfc{} is to maintain the minimum amount of buffering without running out of packets of the paused flow. Unlike PFC where a pause blocks all traffic on a link, in normal BFC operation a pause only affects a single flow. 
Thus, instead of delaying pauses as long as possible hoping to avoid them, we pause aggressively 
to preserve space in the congested switch 
for other flows to transit the switch unaffected.  We first describe the simpler case of how \bfc{} computes the pause/resume threshold when each flow queued at the egress port has its own physical queue. We then describe the more general case.

%\noindent\textbf{Case 1: Active virtual flows < physical queues:} 
Any pause/resume for a flow will take at least one hop RTT ($HRTT$) to take effect. 
The pause/resume message must reach the upstream switch and then the traffic must stop/resume 
at the downstream switch. Moreover, since the pause/resume are 
only sent every $\tau$ seconds, they can take an additional 
time $\tau$ to take effect. A queue in \bfc{} needs
to build up buffering before pausing so that it does not run out of packets 
during this window. However, the queue does not need an entire $HRTT + \tau$ bandwidth-delay
product, because the drain rate is shared (in fair queueing, evenly) among all active queues. 

More formally, a queue needs ($HRTT + \tau$) of buffering at its expected drain rate   
before pausing the flow associated with the queue. 
Let $N_{active}$ be the number of {\em active queues} at an egress port, i.e. queues with data to transmit that are not paused. Then assuming fair queuing as the scheduling policy,  
the pause threshold $Th$ is $(HRTT + \tau) \cdot (\mu / N_{active})$,
where $\mu$ is the capacity of the egress port. Likewise, we re-enable a flow when its
queue falls below this threshold.

Note that this threshold does not guarantee that a queue will never run out of packets due to pausing,
for two reasons. First, the upstream link may be congested, e.g., with data for unrelated downstream
egress ports. If so, it may provide data too slowly to refill the buffer before it empties.
Second, the drain rate is only approximate; the number of active queues is dynamic and can change
over short time intervals, e.g., the queue may drain more quickly than expected.  
In practice, our results show that BFC achieves good throughput despite this simplification.




\cut{
keep The reason is that the drain rate of the queue used to calculate $Th$ could increase after we have already paused the upstream. This could occur, for example, if the other queues at the egress port run out of packets or are paused. The only way to provide a guarantee in the worst case is to set $Th > (HRTT+\tau) \cdot \mu$. However, this is very pessimistic and causes excessive buffering. Our results show that BFC achieves excellent throughput in practice even with threshold $(HRTT + \tau) \cdot (\mu / N_{active})$.}

Because BFC uses pause/resume rather than explicit credits (as in earlier ATM schemes),
in the worst case, each unpaused flow can send at the line rate for $(HRTT + \tau)$ before being
paused. This means $Th +(HRTT + \tau)\cdot \mu$ of buffering per flow may be needed to avoid packet loss.
In practice, a flow's packets are likely be interleaved with other flows and so less buffering
is needed, but it is important to realize that we do not guarantee zero packet loss in the worst case.

\if 0
Because the pause takes $HRTT + \tau$ to take effect, one might think we should pause
earlier than $Th$, to account for packets in flight or those that will be sent
before the pause can take effect. If switch buffering was
highly constrained, for example, we could monitor the rate at which data is arriving 
for a particular flow to estimate the precise moment that we should pause. 
Or, instead of a blanket unpause, we could give the upstream switch a specific number of credits
to use for filling the downstream buffer. Instead, we simply acknowledge that pauses take
some time to take effect, and therefore the amount of buffering consumed can exceed $Th$,
in the worst case, by $(HRTT + \tau) \cdot \mu$. The excess buffering is assuming that the to-be-paused flow will send at line rate. In practice, the flow's packet will be interleaved with other flows and the excess buffering from threshold would me much lesser.
\fi 

When a physical queue receives a pause from a downstream switch, it immediately stops sending,
but it does not necessarily transmit the pause
to its upstream in turn.
Instead, it uses its local value of $N_{active}$ to compute the desired buffer length it would need if it were
{\em not} paused, and forwards a pause upstream when (or if) a packet is received that exceeds that threshold.
This way, when the queue is eventually resumed, there is sufficient buffering in place to
keep the link busy until its upstream can be resumed in turn.  
Note that we compute a flow's pauses/resumes only on packet arrival/departure for that flow.
We do not recalculate
the set of paused flows every time $N_{active}$ changes.

The parameter $\tau$ presents a trade-off. Reducing $\tau$ lowers $Th$, reducing buffer occupancy. However, it increases the bandwidth overhead as the bloom filter must be sent more frequently. Setting a $\tau$ much lower than $HRTT$ has diminishing returns on buffer occupancy.
%, as the minimum value of $Th$ is $HRTT \cdot (\mu/N_{active})$ (with $\tau = 0$) . 
In our simulations, we use $\tau = 0.5 \cdot HRTT$.
}

\cut{
\smallskip
\noindent\textbf{Resuming multiple flows.} 
%\label{s:resuming_multiple}
We next discuss how pausing and resuming works when multiple flows
are assigned to the same queue. It is important to keep
in mind that while the different flows sharing a
queue use the same egress port, they may come from different ingress ports.

A strawman approach would be to pause as before, whenever a flow's packet
arrives if the queue is too large. When resuming, we could unpause
all $n$ flows associated with the queue if the queue length
drops below the threshold.  The problem is that each of the $n$ newly unpaused
flows could potentially send at line rate (if they originated on different
ingress ports). This could build unnecessary buffering and potentially exhaust the switch buffers
if applied across every congested egress queue.%, requiring a blanket pause to avoid packet loss.

To avoid this extra buffering, we adopt a simple heuristic: we
resume at most two flows per $HRTT$  for each queue. 
When a flow is to be resumed, we temporarily put it on a ``to-be-resumed'' queue.  
Every bloom filter update interval $\tau$ (half of $HRTT$), we take one flow off the ``to-be-resumed'' queue and unpause it.
%and clear its information from the bloom filter.
The choice to resume two flows per $HRTT$ also helps in the 
scenario where a resumed flow does not have any, or only has a few, packets at the upstream. 
Since BFC schedules resumes in round-robin order, it provides coarse-grained fairness. As a result, when flows start sharing queues, BFC doesn't incur a sudden degradation in performance.% under such a scenario.

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images_sigcomm20/bloom_design.pdf}
    \vspace{-4mm}
    \caption{\small Illustration. Updates to the bloom filter and its corresponding counter when a flow is resumed. The bit positions that are reset in the bloom filter are shown in red.}
    \label{fig:bloom_diagram}
    \vspace{-4.5mm}
 \end{figure}
\smallskip
\noindent\textbf{Communicating pauses.}
We next turn to the mechanics of communicating and implementing pauses. Instead of a bloom
filter, we could explicitly send a list of FIDs to pause/resume at the upstream switch. 
% Since we only pause (and therefore resume) a flow at most once per packet
% arrival, with batching this would bound the link overhead to a reasonable level.
We did not take this approach, however, as it would require 
communicating pauses {\em reliably},
e.g., with a mechanism to detect and retransmit the pause packet if it was corrupted by
the transmission link.

Instead, we communicate pauses periodically using a small, idempotent multistage bloom filter~\cite{multistagebloom}.
Multistage bloom filters are ideal for communicating sparse bit maps and are convenient for processing updates
in parallel. \cut{The switch maintains a separate bloom filter for every ingress, representing all paused (and implicitly all unpaused) flows on the upstream from the ingress link.} The bloom filter is sent periodically,
at a rate of one every $\tau = 0.5 HRTT$.  These frames do not need to be synchronized across inputs. The switch maintains a separate bloom filter for every ingress, representing all paused (and implicitly all unpaused) flows on the upstream from the ingress link.

To resume a flow with a particular FID, we need to remove it from the bloom filter of its ingress. However, we must be careful to not reset a bit in the bloom filter corresponding to a different flow paused at that port. We solve this problem by keeping a separate counting bloom filter at the
switch (per ingress), with a small counter corresponding to each bit in the bloom filter. When resuming a flow, we first decrement all the counters that the flow's FID hashes into. Only if a counter reaches zero, the corresponding bit at the same position in the bloom filter is set to zero.  \Fig{bloom_diagram} shows an example. 

\if 0
We remove pauses by keeping an internal counting bloom filter at the 
switch (per ingress), with a small counter per bit in the bloom filter.
If two paused FIDs map to the same bloom filter bit position, the count will be two, so that when the time comes
to unpause one of the FIDs, the bit transmitted upstream will still reflect the other FID. \Fig{bloom_diagram} shows these updates to the bloom filter and the counter when a flow is resumed. The switch reduces the counter by 1 on all hash positions given the FID. If the counter goes to zero, the bloom filter value is updated to zero at the same position. 
\fi

In our evaluation we use 4 hash functions for the bloom filter, and 
a bloom filter size of 128 bytes. For an update frequency of once every microsecond, this signaling overhead is about 1~Gbps (1\% on a 100~Gbps link). 
The size of the bloom filter is proportional to the expected number of active flows; we show that this does not change with link speed (\S\ref{s:discussion}). Thus, the bloom filter overhead will be even lower in the future as link speed increases. Other than the bloom filter, BFC does not require any additional header bits, reducing its signaling overhead compared to existing schemes. For example, HPCC puts a 40 B INT Header in both the packet and the corresponding ACK, for an overhead of at least 80 B per data packet. 
%\cut{Assuming 1000 B packet, the overhead is 12\% relative to the load. We also note that, bandwidth overhead can be substantial on lower link speeds. We advocate using a smaller bloom filter on such links to reduce overhead.}

\if 0
For a $X$ Gbps link and a frequency of half of one hop round trip, this
implies a signalling overhead of about 1Gbps or $\frac{100}{X}$\% (only 1\% on 100 Gbps links).
The size of the bloom filter need not be changed, as the link capacity increases, thus, this overhead will decrease with future increases in link speed. Since all the feedback is communicated via the bloom filter, BFC doesn't require any additional header bits or acknowledgments (ACKs), reducing the bandwidth overhead compared to existing schemes. For example, HPCC uses per packet ACKs, and 40 B INT Header both in the packet and the corresponding ACK. The overhead is 120 B per packet. \cut{Assuming 1000 B packet, the overhead is 12\% relative to the load. We also note that, bandwidth overhead can be substantial on lower link speeds. We advocate using a smaller bloom filter on such links to reduce overhead.}
\fi

Of course, a bloom filter can have false positives; in our setting, this can mean pausing flows unintentionally. With no HoL-blocking,
there are at most 32 queued flows to be paused per ingress. 
With 4 hash functions, the likelihood of a false positive is less then 1 in 5 million. 
The false positive rate goes up with incast workloads and high levels of congestion; however,
in these settings, there is likely to be other flows with packets to transmit in place of an unintentionally-paused flow.

When the upstream switch receives a bloom filter, it cannot easily invert it into a set of paused FIDs. Instead, we check the first packet of each queue at the egress port
against the bloom filter; if there is a match (i.e. FID matches against the bloom filter on all four hash positions), we pause that physical queue. This implicitly
pauses all other packets in the same queue. Equally, if the first packet is not paused,
the second packet might be if it is for a different FID. Thus, we recompute the match 
against the bloom filter after dequeuing every packet. 

A detail is that the host network interface card (NIC) must be engineered to accept
bloom filter pause frames, to avoid potentially overfilling the
first level switch. 
We assume the NIC has sufficient hardware to maintain a queue per flow, simplifying the logic. Note that this assumption is implicit in other hardware-based transport schemes like DCQCN and HPCC,  as they require the ability to set per flow rate/window at the NIC. 

}

\cut{
\subsubsection{Bookkeeping}
\label{s:bookkeeping}

BFC maintains the following state per FID: which physical queue it is assigned to, whether it is paused, and how many packets does it have 
queued. 
%Unlike ATM switches that implement credit-based per-flow flow control~\cite{kung1995credit}, 
Unlike approaches that maintain per-connection state~\cite{kung1995credit}, BFC keeps state only for {\em active} flows that have a queued packet; the state is reclaimed when the last packet
of the flow leaves the switch.
During normal operation, even a heavily used switch will only have a few hundred active flows (\S\ref{s:discussion}). A switch under incast can have more, and in the limit we could have as many
active flows as there are packets in the switch buffer.

When a packet arrives at a switch, we need to look up its FID to locate
its state and update it. Since it happens
on every packet, this lookup needs to be fast. 
We use a hash table with a bucket size of four. We choose the number of buckets so that collisions are rare. 
%FID space to be large enough that these collisions are rare. 
In our simulations, we use a hash table with 8K buckets and 32K overall entries. Each entry in the table takes 15 bytes of space: 12 bytes for the FID (5-tuple), 2 bytes for the number of queued packets, 1 byte for the assigned queue number and 1 bit for whether the flow is paused or not. The hash table takes 480\,KB, or 4\% of the 12~MB of packet buffer available
in the switch. The size of the hash table can easily be reduced further with standard techniques, e.g., by using a more compact FID.

%We note that instead of using the full 5-tuple, we could use a shorter FID to reduce the size of our flow hash table. For example, the sender could mark flows with an additional 2-byte source identifier (similar to QCN), a flow can then be uniquely identified at the switch by the source IP and source identifier. The FID as a result would only take 6 bytes of space, reducing the size of the flow hastable by 40\%. However for simplicity, we just use 5-Tuple as the FID. \ma{this is correct but not really needed. i don't think most people will think 480K of state is unreasonable}

%An array might work,
%but a switch is unlikely to have more than a few hundred active flows
%at any one time, while the FID space is much larger.
%Thus, a linear array would be sparse and inefficient.


A consequence of using a hash table with buckets is that the buckets
may fill from time to time. \cut{We maintain a small (100 entry) associative cache
for these overflow FIDs.  If the overflow cache overflows,} If the bucket corresponding to a FID is full, then we put the
packets of the flow into a special per-egress overflow queue which is scheduled
along with the other queues in the normal manner. This is not perfectly order
preserving, as the hash table bucket may become free at some point
in the future, (rarely) leading to packets in both the overflow queue and a regular 
queue.
}

==> discussion.tex <==
% Discussion 1) Credit based 4) Why BFC need PFC or IRN 5) Number of active flows 6) Feasibility on existing hardware
\section{Discussion}
\label{s:discussion}

%\pg{Should we add a limitation/breaking point section? I have decided to skip the discussion on hardware feasibility in the interest of space. Let me know if you guys think otherwise. I think people get confused by the bloom filter, should we just say upfront that it doesnt affect performance compared to sending individual pauses.}

\noindent\textbf{Guaranteed losslessness.} BFC does not guarantee losslessness. In particular, a switch in \bfc{} pauses an \texttt{\small upstreamQ} only after receiving a packet from it. This implies an \texttt{\small upstreamQ} can send packets for up to an $HRTT$ to the bottleneck switch before being paused, even if the switch is congested. In certain mass incast scenarios, this might be sufficient to trigger drops.% However, in our evaluation, drops were extremely rare with BFC. 
%In settings with very simple loss recovery mechanisms (\eg a RDMA setting with Go-Back-N retransmission), we can use PFC as a safe-guard to avoid performance degradation due to drops.% in the extreme cases.
\ Using credits~\cite{anderson1993high,kung1995credit} could address this at the cost of added complexity. We leave an investigation of such prospective variants of BFC to future work. In our evaluation with realistic switch buffer sizes, BFC never incurred drops except under a 2000-to-1 incast (\S\ref{s:limits}) and even then only 0.007\% of the packets were dropped.


% had been in related work but belongs here
%\smallskip
\noindent\textbf{Deadlocks:} Pushback mechanisms like PFC have been shown to be vulnerable to deadlocks in the presence of
cyclic buffer dependencies (CBD) or misbehaving NICs~\cite{hu2016deadlocks,rdmascale}. BFC NICs do not generate any backpressure and as a result cannot cause deadlocks. Since NICs always drain, in the absence of CBD, BFC cannot have deadlocks (see \App{deadlock} for a formal proof). A downstream switch in BFC \emph{will} resume an \texttt{\small upstreamQ} if it drains all the packets sent by the \texttt{\small upstreamQ}. If a downstream is not deadlocked, it will eventually drain packets from the upstream, and as a result, the corresponding upstream cannot be deadlocked.

To prevent CBD, we can reuse prior approaches for deadlock prevention. These approaches can be classified into two categories. The first is to redesign routing protocols to avoid installing routes that might cause CBD~\cite{bolt, stephens2016deadlock}. 
The other is to identify a subset of possible ingress/egress pairs that are provably CBD free, and only
send pause/resume along those pairs~\cite{hu2017tagger}.
For a fat-tree topology, this would allow up-down paths but not temporary loops or detour routes~\cite{f10}. 
% can potentially create CBD and elide/alter the
% backpressure pause/resume on those pairs to break cycles~\cite{hu2017tagger}. 
% For example, up-down paths in a fat-tree topology have \emph{no} such pairs, but detour routes do~\cite{f10}. 
% \sout{The other is to identify a subset of ingress/egress pairs that are provably CBD free and only propagate backpressure on those pairs~\cite{hu2017tagger}. For example, this would include all up-down paths in a fat-tree topology, but not its detour routes~\cite{f10}.}
%
In BFC, we use the latter approach. Given a topology, we pre-compute a match action table indexed by the ingress and egress port, and simply elide the backpressure pause/resume signal if it is disallowed. See \App{deadlock} for details.
% However, these solutions are hard to deploy as the new routing protocols differ heavily from the ones supported by commodity switches~\cite{hu2017tagger}. 
% (e.g., approach, is to identify packets that can cause CBD at the switch \emph{locally}, and, remove or modify the backpressure for such packets to break cycles~\cite{hu2017tagger}.
% If a packet has a hit in this table at a switch, then we don't execute the backpressure operations (\S\ref{s:backpressure}) for it at the switch.


%Given a topology, we can use Tagger~\cite{hu2017tagger} to precompute a rule table for every switch in the network to \emph{locally} identify packets (\ie only using information at the switch) for which the switch shouldn't generate backpressure. The rules in the table are only of the form, don't generate backpressure if the packet came from a certain ingress port and is going to a certain egress port. For clos topologies, this just means packets that are coming from a higher layer and going to higher layer (can happen due to rerouting in case of link failures). Removing backpressure for these packets is simple in BFC, and only involves not executing the backpressure operations (\S\ref{s:backpressure}) at the switch. Tagger's approach can thus be implemented as a single additional match action table to check whether to execute the backpressure operations or not.

%The solutions applied to scale PFC for RDMA within Azure can apply here~\cite{rdmascale}: use up-down or other deadlock-free routes~\cite{bolt}; never use
%pushback for multicast or broadcast packets, treating them as lossy; treat NICs that fall behind as lossy
%rather than allowing them to do pushback; and so forth.

%\noindent\textbf{Credit based hop-by-hop CC:} An alternate approach for limiting buffer occupancy would be for a switch to allocate credits to the upstream switch/NIC for packet transmission. With such an approach, switches can exert a greater degree of control on traffic compared to \bfc{}. A naive implementation of such a scheme would require rate limiting and per-flow queues at the switches~\cite{kung1995credit}. A practical scheme for credit based hop-by-hop CC remains an open problem.

%\smallskip
\noindent\textbf{Incremental Deployment:} In a full deployment, BFC would not require end-to-end 
congestion control. In a partial deployment, 
% when deployed in the entire network. In the scenario, where only a fraction of the network (switches/NICs) is running BFC, 
we advocate some form of end-to-end congestion control, such as capping the number of inflight packets
of a flow. A common upgrade strategy is to upgrade switches more rapidly than server NICs. 
If only switches and not NICs are running BFC, capping inflight packets prevents a source 
NIC from overrunning the buffers of the first hop switch. The same strategy can be used
for upgrading one cluster's switches before the rest of the data center~\cite{minimalrewire}.
% This is to ensure that a switch without BFC doesn't keep on receiving packets from the upstream, exhausting the buffer. 
In our evaluation, we show incremental deployment would have some impact on buffer occupancy at the edge
but minimal impact on performance (\App{incr_deploy}). 
% If one cluster within the data center is upgraded before the rest, traffic within that
% cluster e.g., %Note that, in case legacy NICs are using a non-trivial end-to-end CC (\eg HPCC), BFC switches also need to be modified to separate such traffic and mark appropriate CC feedback for the legacy NICs.

%\smallskip

%\smallskip
\cut{
\noindent\textbf{Traffic characteristics and the number of queues.}
Flows in BFC can incur HoL-blocking when they share a queue with other flows. While BFC tries to minimize such collisions, it still incurs them when the number of flows at an egress port exceed the number of queues. However, in our evaluation we found that such cases were relatively rare; in the absence of incast the collision rate was less than 1\%.  

A standard result in queuing theory provides insight into this phenomenon. Consider flows arriving as a Poisson process to a switch port running fair queuing. This can be modeled as a M/G/1-PS (Processor Sharing) queue. For a M/G/1-PS queue, if the average load is $\rho$, then the number of backlogged flows has a geometric distribution with mean $\frac{\rho}{1-\rho}$~\cite{kleinrock1976queueing}. Therefore, even at a high load of $\rho=0.9$, the expected number of backlogged flows is only 9. Note that the distribution of the number of backlogged flows in this model is independent of the flow size distribution and the link speed. In particular, at the same load $\rho$, increasing link speed does not imply an increase in the number of flows (and therefore collisions in BFC). 

%of the number of backlogged flows is geometric, with 1-$\rho$ as the success probability. The expected number of flows at a port can be given by $\frac{\rho}{1-\rho}$ ~\cite{kleinrock1976queueing}. Even for high load values ($\rho = 0.9$), the expected number of flows at a port is only 9! With 32 physical queues per port; in expectation the number of active flows will be lesser than the number of physical queues. Note that the distribution of active flows is independent of the flow size distribution and link speed. Thus under this model, increasing link speeds do not translate to an increase in collisions.

This theoretical result only applies for a single link with Poisson flow arrivals. In our evaluation, we studied this question for realistic data center topologies, under bursty flow arrivals, high load, and massive incast (\S\ref{s:simulation}). }

%We found that in all these scenarios, BFC achieves excellent performance with a modest number of queues. 

%In practice, the arrival process could be more burstier with incast events increasing the number of active flows, causing collisions. We evaluate such scenarios later.

\if 0

To deal with such scenarios, \bfc{} can either use PFC to pause all the flows when buffer starts filling; or it can use smart retrasnmission strategies like IRN for dealing with drops. We hypothesize that such scenarios where the \bfc{} buffer overflows are rare. In our evaluation we ran \bfc{} with PFC. We found that even under heavy incast scenarios PFC was never triggered.

% this is fairly weak; better to wait until we've implemented it in P4
\noindent\textbf{Feasibility in hardware:} All the datapath operations described in \bfc{} are supported in the P4 programming language for commodity switches~\cite{bosshart2014p4}. The control path operations include an independent thread for pausing physical queues on receiving the bloom filter and another thread for resuming virtual flows from the paused list. Running such threads on existing switches is also feasible. Having said that, current switches don't support pausing/resuming physical queues dynamically as required by \bfc{}. Our conversations with switch vendors indicate that this feature will be supported in the next generation of switches. 

% this is mostly covered in the intro to the design
\noindent\textbf{Characteristics of concurrently active flows:} 
\bfc{} improves FCT by enabling selective pushback while minimizing collisions in the physical queues. A switch might experience collisions if the number of active virtual flow at an egress port is greater than the number of physical queues. In our evaluation, we found that even under high load with incast there were no collisions 99\% of the time, i.e. the number of active virtual flows were lesser than the number of physical queues most of the time. 

A mathematical argument for this phenomenon is based on a core queuing theory result. For a switch doing fair queuing and flows with poisson arrival pattern, the system can be modeled as a M/G/1-PS system. In such a system, if the load is $\rho$ then the expected number of flows ($E(N)$) at an egress port is independent of the flow size distribution, and $E(N)$ can be given by $\frac{\rho}{1-\rho}$ ~\cite{kleinrock1976queueing}. This implies that even for high load values ($\rho = 0.9$), the expected number of flows in the queue is only 9! This implies that for existing switches that support upto 32 physical queues per port; in expectation the number of active flows (hence the number of active virtual flows) will be lesser than the number of physical queues. Incast events can increase the number of active virtual flows temporarily, causing collisions. We believe that the next generation of switches will be able support a higher number of physical queue per port, reducing collisions even further.

\fi

==> evaluation.tex <==
\section{Evaluation}
\label{s:eval}
We evaluate the performance of \bfc{} and compare it against several other schemes using NS3~\cite{ns3} and the DCQCN implementation from ~\cite{zhu2016ecn}.
 
 
 \begin{figure*}[tbh]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_incast_fct.pdf}
        \vspace{-7mm}
        \caption{\small{FCT \cut{(normal)}}}
        \label{fig:google_incast:fct}
    \end{subfigure}
    \cut{\begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_incast_fct_incast.pdf}
        \vspace{-7mm}
        \caption{\small{FCT (incast)}}
        \label{fig:google_incast:fct_incast}
    \end{subfigure}}
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_incast_buffer.pdf}
        \vspace{-7mm}
        \caption{\small{Buffer occupancy}}
        \label{fig:google_incast:buffer}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_incast_pfc.pdf}
        \vspace{-7mm}
        \caption{\small{PFC Time}}
        \label{fig:google_incast:pfc}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small Google distribution with 55\% load + 5\% 100-1 incast. BFC tracks the ideal behavior and improves FCTs\cut{ for both normal (non-incast) and incast traffic}. BFC reduces buffer occupancy and avoids pauses. For FCT slowdown, both the x and y axis are log scaled.}
    \label{fig:google_incast}
    \vspace{-4.5mm}
\end{figure*}

 \begin{figure*}
    \centering
    \begin{subfigure}[tbh]{0.46\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_fct_2.pdf}
        \vspace{-7mm}
        \caption{FCT}
        \label{fig:google:fct}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_buffer.pdf}
        \vspace{-7mm}
        \caption{Buffer Occupancy}
        \label{fig:google:buffer}
    \end{subfigure}
        \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/active_flows.pdf}
        \vspace{-7mm}
        \caption{Active Flows}
        \label{fig:google:active}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small FCT slowdown and buffer occupancy for Google distribution with 60\% load. For all the schemes, PFC was never triggered. \Fig{google:active} shows the CDF of active flows at a port with and without incast. The vertical line shows the total number of queues per port.}
    \label{fig:google}
    \vspace{-3mm}
\end{figure*}
 
 \subsection{Setup}
 \label{ss:setup}
 
% \smallskip
 \noindent\textbf{Network Topology:}  We use a Clos topology with 128 leaf servers, 8 top of the rack (ToR) switches and 8 Spine switches (2:1 over subscription). Each Spine switch is connected to all the ToR switches, each ToR has 16 servers, and each server is connected to a single ToR. All the links are 100\,Gbps with a propagation delay of 1\,us. The maximum end-to-end base round trip time (RTT) is 8\,$\boldsymbol{\mu}$s and the 1-Hop RTT is 2\,$\boldsymbol{\mu}$s. The switch buffer size is set to 12 MB. Relative to the ToR switch capacity of 2.4\,Tbps, the ratio of buffer size to switch capacity is 40\,$\boldsymbol{\mu}$s, same as Broadcom's Tomahawk3 from \Fig{mot_broadcom}. We use an MTU of 1KB and unless specified otherwise we use Go-Back-N for retransmission. Our experiments use the shared buffer memory model, common in existing switches~\cite{broadcom}. We use flow-level ECMP for all the schemes.
 
 %\smallskip
 \noindent\textbf{Comparison:} \noindent\textit{HPCC:} HPCC is a end-to-end control algorithm that uses explicit link utilization
information to reduce buffer occupancy and drops/PFCs at the congested switch. We use the author's implementation of HPCC in NS3, with parameters from the paper, $\eta = 0.95$ and $maxStage = 5$. The PFC threshold is set to trigger when traffic from an input port occupies more than 11\% of the free buffer. We use the same PFC thresholds for all other schemes.% and other variants of HPCC.
 
\noindent\textit{DCQCN:} DCQCN uses ECN bits and end-to-end control to manage buffer use at the congested switch. We use the author's implementation in NS3. The ECN marking threshold triggers before PFC (K$_{min}$ = 100KB and K$_{max}$ = 400KB).
 
 \noindent\textit{DCTCP:} We use the NS3 implementation from ~\cite{hpcc}. The ECN marking threshold is same as DCQCN. Flows start at line rate to avoid degradation in flow completion times from slow-start.
 
 \noindent\textit{\bfc{}:} We use 32 physical queues per port (consistent with existing switch capabilities ~\cite{afq,bosshart2014p4}) and our flow hash table has 8K buckets.  The hash table takes 480 KB of memory, ($\sim$ 4\% of the switch buffer). The bloom filter is 128 Bytes, so pause frames use 1\,Gbps per link ($\sim$ 1\% of the link speeds). We chose per-flow fair queuing as our scheduling mechanism; all the comparison schemes strive for per-flow fairness, thus, fair queuing provides for a just comparison.\cut{; 2) Unlike fair queuing, shortest flow first scheduling (and its approximations) make assumptions about knowing the flow sizes apriori.}
 
 \noindent\textit{Ideal-FQ:} To understand how close \bfc{} comes to optimal performance, we simulate ideal fair queuing with infinite buffering at each switch. The NICs use a window cap of 1 BDP. Note that Ideal-FQ is not realizable in practice; its role is to bound how well we might possibly do.
 
 
 %\smallskip
 \noindent\textbf{Performance metrics:} We consider four performance metrics. 1) Flow completion time (FCT) normalized to the best possible FCT for the same size flow, running at link rate (referred as the FCT slowdown); 2) The overall buffer occupancy at the switch; 3) Percentage of time links were paused due to PFC; 4) Throughput of individual flows.

%\smallskip 
 \noindent\textbf{Workloads:}  We synthesized a trace to match the flow size distributions from the industry workloads discussed in \Fig{mot_flowsize}. 1) Aggregated workload from all applications in a Google data center; 2) Hadoop cluster at Facebook (FB\_Hadoop). The flow arrival pattern follows a lognormal distribution with $\sigma$ = 2. For each flow arrival, the source-destination pair is derived from a uniform distribution. We consider scenarios with and without incast, different traffic load settings\footnote{Since our topology is oversubscribed, on average links in the core (Spine-ToR) will be more congested than the ToR-leaf server links. In our experiments, by X\% load we mean X\% load on the links in the core.}, and incast ratios. %We report the FCT slowdown for the normal (non-incast) and incast traffic separately.

 \subsection{Performance}
 

 \Fig{google_incast} and ~\ref{fig:google} show our principal results. The flow sizes are drawn from the Google distribution and 
the average load is set to 60\% of the network capacity. For \Fig{google_incast}, the average load includes a 5\% 100-to-1 incast traffic. The incast size is 20MB in aggregate. We report the tail buffer occupancy, the FCT slowdowns at average, 95$^{\text{th}}$ and 99$^{\text{th}}$ percentile, and the fraction of time links were paused due to PFC. We report the FCT slowdowns for the incast traffic separately in \App{incast_fct}.  
 
Out of all the schemes, DCQCN is worst on latency for small flow sizes, both at the average and the tail. Compared to DCQCN, DCTCP improves latency as it uses per-ACK feedback instead of periodic feedback via QCN.\cut{ the feedback to the sender is more frequent, every ACK instead of periodic feedback via QCN (55us or 5 RTT). }
However, the frequent feedback is not enough, and the performance is far from optimal (Ideal-FQ). The problem is that both
 DCQCN and DCTCP are slow in responding to congestion. 
 Since flows start at line rate, a flow can build up an entire end-to-end bandwidth-delay product 
 (BDP) of buffering (100 KB) at the bottleneck
 before there is any possibility of reducing its rate.
% This leads to long delays particularly at the tail.  Excessive PFC pauses make this even worse.
 The problem is aggravated during incast events. 
The bottleneck switch can potentially accumulate one BDP of packets per incast flow (10MB in aggregate for 100-to-1 incast).

Both protocols have low throughput for long flows. When capacity becomes available, a long flow may fail 
to ramp up quickly enough, reducing throughput and shifting its work to busier periods where it can impact other flows. 

HPCC improves on DCQCN and DCTCP by using link utilization instead of ECN and a better control algorithm. 
Compared to DCQCN and DCTCP, HPCC reduces tail latency, tail buffer occupancy, and PFC pauses (in case of incast). Compared to \bfc{}, however, HPCC has 6-30$\times$ worse tail latency for short flows with incast, and 2.5-4 $\times$ worse without. Long flows do worse with HPCC than DCQCN and DCTCP. HPCC aims to maintain small buffers to improve tail latency for short flows, and this means the switch can run of out of packets before the flows ramp up when bandwidth becomes available.
 
Ideal-FQ achieves the lowest latency among all the schemes. However,
buffer occupancy can grow to an unfeasible level.

BFC achieves the best latency (both average and tail) among all realizable schemes (close to optimal). Without incast, BFC performance
closely tracks optimal.  With incast, incoming flows exhaust the number of physical queues, triggering
head of line blocking and hurting tail latency.
This effect is largest for the smallest flows at the tail. \Fig{google:active} shows the of number of active flows at a port. In the absence of incast, the number of active flows is smaller than the total queues 99\% of the time, and collisions are rare. This is in line with the queuing theory result stated in \S~\ref{s:discussion}. \footnote{Our setup doesn't meet all the assumptions of the result. In particular, i) The arrival process is a burstier lognormal instead of poisson. ii) The topology is multi-layered with multiple points of congestion. Despite this, most of the time, the active flows are fewer than the total queues.} With incast, the number of active flows increase, causing collisions. However,
the tail latency for short flows with BFC is still 6-30 $\times$ better than existing schemes.

BFC also improves the performance of incast flows, 2$\times$ better at the tail compared to HPCC (see \App{incast_fct}). In the absence of incast, the buffer occupancy for BFC is higher than HPCC, but this extra buffering is necessary to ensure that flows don't run out of packets at the switch and lose throughput. 
\cut{, as it doesn't incur any PFC pauses and switches maintain sufficient per-flow buffering.% to ensure packets in the queue.
Overall, physical queues are used efficiently, and buffers are managed to prevent PFCs and cascading HoL-blocking.}

\cut{\Fig{google:active} shows the of number of active flows at a port. In the absence of incast, the number of active flows is smaller than the total queues 99\% of the time, and collisions are rare. This is in line with the queuing theory result stated in \S~\ref{s:discussion}. \footnote{Our setup doesn't meet all the assumptions of the result. In particular, i) The arrival process is a burstier lognormal instead of poisson. ii) The topology is multi-layered with multiple points of congestion. Despite this, most of the time, the active flows are fewer than the total queues.} With incast, the number of active flows increase.}%, thus, collisions are more frequent.} 

Note that, compared to \bfc{} and Ideal-FQ, latency for medium flows (200-1000KB) is slightly better with existing schemes. Because they slow down long flows relative to perfect fairness, medium flows have room to get through more quickly. Conversely, tail latency for long flows is better with \bfc{} and Ideal-FQ than with medium flows. Long flows achieve close to the long term average available bandwidth, while medium flows are more affected
by transient congestion.
 
  \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/fb_incast_fct.pdf}
        \vspace{-7mm}
        \caption{55\% + 5\% 100-1 incast}
        \label{fig:fb:incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/fb_fct.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:fb:no_incast}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small FCT slowdown (99$^{th}$ percentile) for Facebook distribution with and without incast. }
    \label{fig:fb}
    \vspace{-5mm}
\end{figure}

 
 We repeated the experiment in \Fig{google_incast} and ~\ref{fig:google} with the Facebook distribution. \Fig{fb} shows the 99$^{th}$ percentile FCT slowdown. The trends in the FCT slowdowns are similar to that of the Google distribution. We omit other statistics presented earlier in the interest of space, but the trends are similar to \Fig{google_incast} and ~\ref{fig:google}. Note that the x-axis in \Fig{fb} is different as the Facebook flow size distribution is different from \Fig{google_incast} and ~\ref{fig:google}. Henceforth, all the experiments use the Facebook workload.% (for reducing RAM consumption in simulations). With the Google workload, flow sizes are smaller, as a result total number of flows in the experiment duration is higher. All the simulators in our evaluation create an application per flow, and the RAM consumption is very high.
 

  \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/srf_incast.pdf}
        \vspace{-7mm}
        \caption{55\% + 5\% 100-1 incast}
        \label{fig:srf:incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/srf.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:srf:no_incast}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small Impact of scheduling policy. BFC + SRF (shortest remaining first) reduces FCTs by prioritizing short flows.}
    \label{fig:srf}
    \vspace{-5mm}
\end{figure}
 
%\smallskip
\noindent\textbf{Impact of scheduling policy:}
The design of BFC is orthogonal to the scheduling policy. We repeated the experiment from \Fig{fb}, but changed the scheduling policy at the switch from fair queuing (FQ) to shortest remaining flow first (SRF). SRF schedules flows in the order of remaining flow sizes, and has been shown to be optimal for optimizing FCTs ~\cite{pfabric}. \Fig{srf} shows the 99$^{th}$ percentile FCT slowdowns. We also show Ideal-SRF, an ideal realization of SRF without any restrictions on the number of queues or buffer size. For BFC + SRF and Ideal-SRF, we assume the flow size is known apriori. As expected, BFC + SRF reduces FCTs compared to BFC + FQ in both the scenarios. BFC + SRF tracks the optimal (Ideal-SRF) quite closely. With SRF, flows finish faster, thus, the number of active flows per-port is smaller than with FQ, and BFC + SRF incurs fewer collisions than BFC + FQ.

In the presence of incast, for both BFC + SRF and Ideal-SRF, there is jump in the FCT for flows with size bigger than the incast flow size (200 KB, shown as a vertical line in \Fig{srf:incast}). This is because SRF schedules the incast flows ahead of these longer flows. Note that while SRF reduces FCTs, it doesn't ensure fairness. Thus, the choice of scheduling policy depends on the requirements of the data center operator.
 
   \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/fb_incast_fct_variants.pdf}
         \vspace{-7mm}
        \label{fig:fb_variants:incast}
        \caption{55\% + 5\% incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/fb_fct_variants.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:fb_variants:noincast}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Comparison with variants of HPCC in \Fig{fb}.}
    \label{fig:fb_variants}
    \vspace{-4mm}
\end{figure}
 
 
 %\smallskip
 \noindent\textbf{Comparison with enhanced variants:}
 To further understand where the benefits in BFC are coming from, we repeated the experiment in \Fig{fb}, but we added features to the existing schemes. \Fig{fb_variants} reports the FCTs with these variants. We also show BFC and the original HPCC (with PFC) in the results.
 
\textit{Scheduling:} First, we evaluate HPCC+SFQ, a scheme that combines HPCC with better scheduling at the switch. Each egress port does stochastic fair queuing on incoming flows. To match BFC we use 32 physical queues. Adding scheduling improves tail latency by allowing different flows to be scheduled from different physical queues. However, the FCT slowdowns are still worse than BFC, because of two reasons. (i) There are collisions in assigning flows to physical queues. A small flow sharing the queue with other flows will see its packets delayed. (ii) HPCC+SFQ adjusts flow rates in an end-to-end manner. With incast, it builds deep buffers and experiences PFC pauses at the same rate as HPCC, both of which hurt latency. 
% Moreover, for long flows, adding SFQ doesn't help in either scenario, and the throughput is still worse compared to BFC.
 
\textit{Retransmission:} Next, we replace PFC in HPCC with perfect retransmission.  Without incast, the performance is identical to HPCC as PFC is never triggered in this scenario. With incast, HPCC + Perfect Retransmission improves performance compared to HPCC but is still far from BFC. Retransmission on its own doesn't reduce buffer occupancy, hurting latency. Retransmission does help tail latency of medium flows with incast.
\cut{Moreover, with incast the switch experiences drops, retransmitted packets incur additional delay and consume bandwidth hurting latency of other flows. So while retransmission improves performance, it does not remove the need for congestion control.
 As mentioned earlier, the FCTs for medium flows can be better than BFC as all variants of HPCC only slow down long flows, and medium flows can get through quicker.}
 
\textit{Slow-start:} We also evaluate the impact of using TCP slow-start instead of starting flows at line rate in Figure~\ref{fig:ss}. We compare the original DCTCP with slow start (DCTCP + SS) with an initial window of 10 packets versus the modified DCTCP used so far (initial window of the BDP). With incast, DCTCP + SS reduces buffer occupancy by reducing the intensity of incast flows, improving latency. However, in the absence of incast, slow start increases the tail latency for medium flows (0.5-5 BDP). Flows start at a lower rate, taking longer to ramp up to the desired rate.  However, short flows are still slower than with BFC, because slow start does not remove burstiness in buffer occupancy in the tail.

  \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/ss_incast.pdf}
        \vspace{-7mm}
        \caption{55\% + 5\% 100-1 incast}
        \label{fig:ss:incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/ss.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:ss:no_incast}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Impact of using slow start on 99\% tail latency. DCTCP + SS (slow start) reduces FCTs in the presence of incast. However, in the absence of incast, it increases the tail FCT for medium flows without affecting the tail FCT for short flows.}
    \label{fig:ss}
    \vspace{-4mm}
\end{figure}



\noindent\textbf{Cross data center traffic:}
\begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.22\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/datacentre_fct.pdf}
         \vspace{-7mm}
        \caption{99$^{th}$ percentile FCT }
        \label{fig:cross:fct}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.25\textwidth}
        \includegraphics[width=0.86\textwidth]{images_sigcomm20/datacentre_utilization2.pdf}
        \vspace{-2mm}
        \caption{Utilization at the interconnect.}
        \label{fig:cross:utilization}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Performance in cross data center environment where two data center are connected by a 200 $\mu$s link. The left figure shows the FCT for intra-data center flows. The right figure shows the average utilization of the link connecting the two data centers.}
    \label{fig:cross}
    \vspace{-5mm}
\end{figure}
For fault tolerance, many data center applications replicate their data to nearby data centers (\eg within a metro area). We evaluate
the impact of BFC on managing cross-data center congestion in such scenarios. 
We consider the ability of different systems to achieve good throughput for the inter-data center traffic,
and we also consider the impact of the cross-data center traffic on tail latency of local traffic, as
the larger bandwidth-delay product means more data is in-flight when it arrives at the bottleneck.

%a metro area, 
We created a Clos topology with 64 leaf servers, and 100\,Gbps links and 12\,MB switch buffers.
Two gateway switches connect the data centers using a 200\,Gbps link with 200\,$\mu$s of one-way delay (i.e. the base round
trip delay of the link is 400\,$\mu$s). A longer hop will require more buffering in BFC to keep the link busy, 
and so we configured the buffer size of the gateway switch to be 64\,MB. 
The experiment consists of intra-data center flows derived from the Facebook distribution (60\% load). Additionally, there are 20 long-lived inter-data center flows in both the directions.

\Fig{cross:fct} shows the tail latency in FCT slowdown for intra-data center flows for BFC, HPCC and DCQCN. \Fig{cross:utilization} shows the average utilization of the link connecting the two data centers (interconnect), a proxy for the aggregate throughput of the long-lived inter-data center flows.
BFC is better for both types of flows. 
With BFC the utilization at the interconnect is close to 100\%, and the tail FCTs for intra-data center flows is lower. 
The degradation in performance with HPCC and DCQCN is a consequence of slow end-to-end reaction of the inter-data center flows. The congestion state on the links within a data center is changing rapidly because of the shorter intra-data center flows. By the time a inter-data center flow receives congestion feedback and adjusts its rate, the congestion state in the network might have already changed. When capacity becomes available, an inter-data center flow can fail to ramp up quickly enough, hurting its throughput. Likewise, on sudden onset of congestion, the long-lived flow will take an end-to-end RTT to reduce its rate, and can build up to 1 BDP (or 500 KB) of buffering, hurting the tail latency of intra-data center traffic.

In contrast, \bfc{} reacts at the scale of the hop-by-hop RTT.
Even though inter-data center flows have higher end-to-end RTTs, on switches within the data center, 
\bfc{} will pause/resume flows on a hop-by-hop RTT timescale (2\,$\mu$s).
As a result, with BFC, tail latencies of intra-data center flows are unaffected by the presence of inter-data
center flows, while the opposite is true of DCQCN and HPCC. We confirmed this experimentally in a 
separate experiment where we removed all the inter-data center traffic. The tail latency with DCQCN and HPCC
improved in this case, while it had no effect on BFC.
Additionally, when capacity becomes available on a link within the data center, the upstream of the long-lived flow can send packets within 1-Hop RTT avoiding any unnecessary loss in throughput. 



\subsection{Understanding the limits of BFC}
\label{s:limits}
The performance of BFC depends on the characteristics of the workload (traffic load, incast ratio, etc.) and the available resources (number of physical queues, size of the flow hash table, etc.). We evaluate the impact of these factors.% on BFC. 


 \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/load_long.pdf}
         \vspace{-7mm}
        \caption{FCT for long flows}
        \label{fig:load_var:long}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/load_small.pdf}
        \vspace{-7mm}
        \caption{FCT for short flows}
        \label{fig:load_var:small}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Impact of traffic load on performance.}
    \label{fig:load_var}
    \vspace{-5mm}
\end{figure}

%\smallskip
\noindent\textbf{Load:}
We vary the average load from 50 to 90\% (without incast). Recall that the load factor is for oversubscribed core switches; leaf switches have more capacity. \Fig{load_var:long} shows the median slowdown for long flows (> 3MB). \Fig{load_var:small} shows the 99$^{th}$ percentile slowdown for short flows (< 3KB). %Note that the yaxis for long and short flows is different.

HPCC only supports loads up to 70\%. At higher loads, it does not converge, in part due to the overhead of the INT header (80\,B per-packet). All other schemes were stable across all load values. 
% (12\% relative to the average load). %In contrast the overhead for BFC is only 1\%.\cut{, for DCQCN and DCTCP the overhead is 4\% (with 40KB ACK).}

At loads $\leq$ 80\%, BFC achieves both lower tail latency for short flows and higher throughput for long flows. The tail latency for short flows is close to the ideal value of 1 except at 90\% load. At higher loads, flows remain queued at the bottleneck switch for longer periods of time, raising the frequency that we run out of physical queues, leading to head of line blocking. This particularly hurts tail performance for short flows as they might get stuck behind a long flow sharing the same queue. Since BFC provides coarse-grained fairness among flows sharing the same physical queue with round robin resumes(\S\ref{s:backpressure}), the impact of collisions is limited for long flows.

\cut{ leave for the Appendix, no need to mention it here, as its a non-result
In our setup, the links in the core are more congested than the ToR-leaf links. We repeated the experiment in \Fig{load_var} with spacial locality in source-destination pairs such that the average load on all links across the network is same. The trends with spacial locality are similar. BFC incurs HoL blocking for short flows only at 90\% load (see \App{load_var:locality}).
}


\begin{figure}[t]
     \centering
    \includegraphics[width=0.99\columnwidth]{images_sigcomm20/incast_var.pdf}
    \vspace{-4mm}
    \caption{\small Impact of incast degree on 99$^{th}$ flow completion times.}
    \label{fig:incast_var}
    \vspace{-6mm}
 \end{figure}
%\smallskip
\noindent\textbf{Incast degree:}
If the size of an incast is large enough, it can exhaust physical queues and hurt performance.
\Fig{incast_var} shows the effect of varying the degree of incast on tail latency.
The average load is 60\% and includes a 5\% incast. The incast size is 20MB in aggregate, but we vary the degree of incast from 10 to 1000. BFC is shown as BFC + Flow FQ for per flow fair queuing.

BFC's performance tracks the optimal (IdealFQ) at the lowest incast degree. As the incast increases, BFC starts sharing physical queues, triggering HoL blocking for short flows. In the 1000-1 case, the incast can exhaust switch buffers even with backpressure, because each flow can send up to one hop BDP to the bottleneck. However, BFC outperforms HPCC across all scenarios.

To reduce contention for physical queues, we tried a variant of BFC that uses per-destination fair queuing -- all flows to the same destination share the same queue. In \Fig{incast_var}, this is shown as BFC + Dest. FQ. Regardless of the incast degree, BFC + Dest. FQ doesn't incur HoL blocking from running out of physical queues, and it outperforms all other schemes. Performance is even better than IdealFQ (per flow). When there are multiple incast flows at an egress port, per-flow fair queuing will allocate more bandwidth to the incast flows in aggregate than per-destination fair queuing, reducing performance for the non-incast flows.

While per-destination fair queuing is better than per-flow fair queuing under massive incasts, it presents a trade-off. With per-destination fair queuing, flows to the same destination share a physical queue. A destination that receives a mixture of short and long flows will incur significant delays for short flows in the tail of the distribution. This effect worsens as load increases. We also considered a hybrid approach, where the sender labels incast flows (similar to ~\cite{homa}). This performs best but assumes application help, and so we use a more
conservative design for the main body of our evaluation.
% In the interest of space, we omit their description. 
% We assign a single physical queue to the incast flows. For the non-incast flows, the switch uses the original queue assignment and simply does per flow fair queuing. As a result, the hybrid scheme is able to achieve good performance both under massive incasts and high loads. Since the feasibility in practice is unknown, we chose per flow fair queuing as our baseline scheme. We note that both the variants of BFC discussed above require modifications to bookkeeping. In the interest of space, we omit their description. 

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.46\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/pq_load.pdf}
        \vspace{-7mm}
        \caption{60\% and 90\% load}
        \label{fig:pq:load}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/pq_incast_fct.pdf}
        \vspace{-7mm}
        \caption{55\% +5\% incast}
        \label{fig:pq:incast}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/pq_incast_fct_collisions.pdf}
        \vspace{-7mm}
        \caption{Collisions (incast)}
        \label{fig:pq:incast+hol}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Impact of number of physical queues.}
    \label{fig:pq}
    \vspace{-5mm}
\end{figure}
%\smallskip
\noindent\textbf{Number of physical queues:} We evaluate the impact of the number of physical queues on performance. We vary the number of physical queues per port from 8 to 128. \Fig{pq:load} shows the 99$^{th}$ percentile FCT slowdowns with 60 and 90\% load (no incast). \Fig{pq:incast} shows the FCT slowdown with 55\% load + 5\% incast (100-1). \Fig{pq:incast+hol} shows the fraction of flows that share the same physical queue (collisions) in the incast scenario. Both the experiments use the Facebook distribution.

As expected, decreasing the number of physical queues causes collisions. In the absence of incast, the degradation in performance is gradual. With 60\% load, the performance plateaus at 16 queues. With 90\% load, the number of active flows increase, and the performance plateaus at 64 queues. With incast, the knee of the curve is at 32 queues, while increasing queues beyond 64 doesn't improve performance. With 64 queues, the collisions primarily occur at the last hop, i.e., at the egress port connecting the ToR and the incast server. We do not allow servers to pause the ToR, so these collisions don't hurt the tail latency much (performance is close to IdealFQ). This implies that any incast within a rack will have minimal impact. In larger topologies than the ones we simulate, where the fan into the ToR is higher, per-flow backpressure will be spread out over more upstream switches, dissipating the effect except for very large incasts.


\cut{Interestingly, with 64 queues, the collisions primarily occur at the last hop, i.e., at the egress port connecting the ToR and the incast leaf server; the incast flows are spread out at the higher layers and the number of active incast flows is smaller than the last hop. BFC maintains the buffer occupancy of a physical queue at a low level, and collisions degrade performance primarily because of hol-blocking from pauses. Since egress ports at the last hop cannot be paused by the upstream leaf server, these collisions don't hurt the tail latency much (performance is close to IdealFQ).
This implies BFC can handle bigger incasts, if the incasts are within the same ToR. Additionally, in larger topologies where the FanIn from Core to ToR is higher, the collisions will primarily occur at the very last hop and won't degrade performance as much. \cut{\pg{Can we say this without explicit experiments? The experiment with locality in incast is easy to run.}}

% I cut these two paragraphs too.  This is speculation.  If you want to say it, say it earlier when we discuss trends in switch design (e.g., that we'll be able to pause in the datapath.
Note that across all the scenarios (heavy load and incast), the required number of physical queues is 64, higher than the number in existing switches. The results in this section make a case for increasing the physical queues in switches. We believe that the number of physical queues can be scaled to a few hundreds without hurting the capacity of existing switches.

% OK to include the appendix, but no need to mention it.
We also repeated the experiment in \Fig{pq:incast} but varied the size of the bloom filter and the flow hash table instead. BFC's performance is not sensitive to either of these resource constraints (see ~\App{sensitivity} for details). 

}


\subsection{Design choices}
\label{s:desgin_choices}


%\smallskip
 \noindent\textbf{Physical queue assignment:}
 \begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=1.0\textwidth]{images_sigcomm20/qassign_fct.pdf}
    \vspace{-7mm}
    \subcaption{99$^{th}$ percentile FCT}
    \label{fig:indirection:fct}
    \end{subfigure}
     \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=1.0\textwidth]{images_sigcomm20/qassign_collisions.pdf}
    \vspace{-7mm}
    \subcaption{Collisions}
    \label{fig:indirection:collisions}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Performance of BFC with stochastic queue assignment, for the workload
    in \Fig{pq:incast}. \bfc{} + Stochastic incurs more queue collisions leading to worse tail latency compared to \bfc{} + Dynamic.}
    \label{fig:indirection}
    \vspace{-5mm}
 \end{figure}
 To understand the importance of dynamically assigning flows to physical queues, we repeated the experiment in \Fig{pq:incast} with a variant of \bfc{}, \bfc{} + Stochastic, where we use stochastic hashing to statically assign flows to physical queues (as in SFQ). In \bfc{} (referred as \bfc{} + Dynamic here), the physical queue assignment is dynamic. To isolate the effect of changing the physical queue assignment, the pause thresholds are the same as \bfc{} + Dynamic.

 
 \Fig{indirection:fct} shows the tail latency. Compared to \bfc{}, tail latency for \bfc{} + Stochastic is much worse for all
 flow sizes. 
 Without the dynamic queue assignment, flows are often hashed to the same physical queue, triggering HoL-blocking and hurting tail latency, even when there are unoccupied physical queues. \Fig{indirection:collisions} is the CDF of such collisions. \bfc{}+Stochastic experiences collisions in a high fraction of cases and flows end up being paused unnecessarily. 
 % As a result, flows finish later, further increasing the number of active flows and collisions.
 % In contrast, \bfc{} + Dynamic the collisions are fewer (< 2 \%). 
 Even with incast, the number of active flows in BFC is smaller
 than the physical queues almost all of the time.

%\smallskip
\noindent\textbf{Buffer occupancy management:}
 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/incast.pdf}
    \vspace{-3mm}
    \caption{\small Queue size as a function of the number of concurrent flows. \bfc{} limits the physical queue size to 2-Hop BDP.}
    \label{fig:buffersize}
    \vspace{-4mm}
 \end{figure}
In ~\Sec{backpressure}, we introduced an optimization to limit the buffering at a physical queue 
when multiple flows are mapped to it. To test the effectiveness of this optimization, 
we created concurrent long lived flows destined to the same receiver. We varied the number of concurrent flows from 8 to 256. This implies that the average number of flows per physical queue varied from 0.25 to 8 (32 physical queues per port). We also ran a variant of our scheme without the buffer optimization (\bfc{}-BufferOpt). In \bfc{}-BufferOpt, an egress port resumes all flows associated with a physical queue when the physical queue goes below the pause threshold.

\Fig{buffersize} shows the tail (99$^{th}$ percentile) per physical queue buffer occupancy at the switch. By limiting the rate we resume flows per physical queue (two per 1-Hop RTT), BFC keeps worst case buffer utilization to about twice the per-hop BDP, regardless of the number of concurrent flows sharing a particular physical queue.  Note that this result
does not apply for all workloads; a flood consisting entirely of one or two packet flows can drive buffer
occupancy up, even for BFC. 

Without this optimization, once all the queues are utilized, the buffer size grows linearly with the number of concurrent flows.



==> evaluation_nsdi21.tex <==
\section{Evaluation}
\label{s:eval}

We present a proof-of-concept evaluation of our SwitchX implementation. To compare performance of BFC against existing schemes, we perform large scale ns-3~\cite{ns3} simulations.





\subsection{SwitchX evaluation}
\label{s:tofino2}
\noindent\textbf{Testbed:} For evaluation, we were able to gain remote access to a SwitchX switch. Using a single switch, we created a simple multi-switch topology (\Fig{testbed}) by looping back packets from the egress port back into the switch. All the ports are 100 Gbps, each port has 16 queues.\footnote{For 100 Gbps ports, SwitchX has 32 queues, but in loopback mode only 16 queues are available.} The experiments include three groups of flows. 
\begin{CompactItemize}
\item Sender Group 1 $\rightarrow$ Switch 1 $\rightarrow$ Switch 2 $\rightarrow$ Receiver 1.
\item Sender Group 2 $\rightarrow$ Switch 1 $\rightarrow$ Switch 2 $\rightarrow$ Receiver 2.
\item Sender Group 3 $\rightarrow$ Switch 3 $\rightarrow$ Switch 2 $\rightarrow$ Receiver 2.
\end{CompactItemize}
To generate traffic we use the on-chip packet generator with no end-to-end congestion control.

\begin{figure}[t]
     \centering
    \includegraphics[width=0.75\columnwidth]{images_nsdi21/tofino2_topology.pdf}
    \vspace{-2mm}
    \caption{\small {\bf Testbed topology.} The colored lines show the path for different flow groups.}
    \label{fig:testbed}
    \vspace{-5mm}
 \end{figure}

  \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/qdepth.pdf}
        \vspace{-7mm}
        \caption{Queue Length}
        \label{fig:qdepth:qdepth}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/qdepth_utilization.pdf}
        \vspace{-7mm}
        \caption{Under-utilization}
        \label{fig:qdepth:utilization}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small {\bf Queue length and under-utilization.} 2 flows are competing at a 100 Gbps link. BFC achieves high utilization and low buffering.}
    \label{fig:qdepth}
    \vspace{-5mm}
\end{figure}

\noindent\textbf{Low buffering, high utilization:} \Fig{qdepth:qdepth} shows the queue length for a flow when two flows are competing at a link (a group 2 flow is competing with a group 3 flow at the switch 2 $\rightarrow$ receiver 2 link). The pause threshold is shown as a horizontal black line. BFC's pausing mechanism is able to limit the queue length near the pause threshold ($Th$). The overshoot from $Th$ is for two reasons. First, it takes an $HRTT$ for the pause to take effect. Second, SwitchX has small hardware queues after the egress pipeline, and a pause from the downstream cannot pause packets already in these hardware queues. 

Notice that the queue length goes to 0 temporarily. Recall that a downstream switch only resumes the \texttt{\small upstreamQ} when it has drained all the packets from the \texttt{\small upstreamQ} that exceeded $Th$. As a result, a flow at the downstream can run out of packets for an $HRTT$. %In the \emph{absence} of competing active queues, this can hurt link utilization. 
%
This can cause under-utilization when the queues for the two flows go empty simultaneously. 
% The frequency of such events depends on the pause threshold (\S\ref{s:backpressure}). 
We repeat the above experiment but vary the pause threshold. \Fig{qdepth:utilization} shows the average queue length and the under-utilization of the congested link. With a pause threshold of 2 $\mu$s, BFC achieves close to 100\% utilization with an average queue length of 15 KB. %\pg{do we need to say more?}%Note that this is possible because SwitchX pauses/resumes queues quickly (from the dataplane).  

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images_nsdi21/congestion_spreading.pdf}
    \vspace{-4mm}
    \caption{\small {\bf Congestion spreading.} Dynamic queue assignment reduces HoL-blocking, improving FCTs on average and at the tail.}
    \label{fig:congestion_spreading}
    \vspace{-5.5mm}
 \end{figure}
 
 
\noindent\textbf{Queue assignment and congestion spreading:} We next evaluate the impact of queue assignment on HoL-blocking and performance. We evaluate three different queue assignment strategies with BFC's backpressure mechanism: (1) ``BFC + single'': All flows are assigned to a single queue (similar to PFC); (2) ``BFC + stochastic'': Flows are assigned to queues using stochastic hashing; (3) ``BFC + dynamic'': Dynamic queue assignment as described in \S\ref{s:qassignment}. 

The setup consists of two group 1 flows, eight group 3 flows, and a number of group 2 flows varied between four to twenty. All flows are 1.5 MB in size. The experiment is designed such that for group 2 and 3 flows, the bottleneck is the switch 2 $\rightarrow$ receiver 2 link. The bottleneck for group 1 flows is the switch 1 $\rightarrow$ switch 2 link. Switch 2 will pause queues at switch 1 in response to congestion from group 2 flows. Notice that group 1 and group 2 flows are sharing the switch 1 $\rightarrow$ switch 2 link. If a group 1 flow shares a queue with a group 2 flow (a collision), the backpressure due to the group 2 flow can slow down the group 1 flow, causing HoL-blocking and increasing its flow completion time (FCT) unnecessarily.

\Fig{congestion_spreading} shows the average FCT for group 1 flows across four runs. The whiskers correspond to one standard deviation in the FCT. BFC + single achieves the worst FCT as group 1 and 2 flows always share a queue. With stochastic assignment, the FCT is substantially lower, but the standard deviation in FCT is high. In some runs, group 1 and 2 flows don't share a queue and there is no HoL-blocking. In other runs, due to the stochastic nature of assignment, they do share a queue (even when there are other empty queues), resulting in worse performance. With dynamic assignment, BFC achieves the lowest average FCT and the best tail performance. In particular, the standard deviation is close to 0 when the number of flows at the switch 1 $\rightarrow$ switch 2 link (group 1 + group 2 flows) is lower than the number of queues. In such scenarios, group 1 flows consistently incur no collisions. 
% BFC + dynamic achieves the best FCT not only on average but at the tail as well. 
When the number of flows exceed the queues, collisions are inevitable, and the standard deviation in FCT increases.

\subsection{Simulation-based evaluation}
\label{s:simulation}
We also implemented BFC in ns-3~\cite{ns3}. For DCQCN we use~\cite{dcqcn_code}, and for all other schemes we use~\cite{hpcc_code}.
 
 
 \begin{figure*}[tbh]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/google_incast_fct2.pdf}
        \vspace{-7mm}
        \caption{\small{FCT \cut{(normal)}}}
        \label{fig:google_incast:fct}
    \end{subfigure}
    \cut{\begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/google_incast_fct_incast.pdf}
        \vspace{-7mm}
        \caption{\small{FCT (incast)}}
        \label{fig:google_incast:fct_incast}
    \end{subfigure}}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/google_incast_buffer2.pdf}
        \vspace{-7mm}
        \caption{\small{Buffer occupancy}}
        \label{fig:google_incast:buffer}
    \end{subfigure}
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/google_incast_pfc.pdf}
        \vspace{-7mm}
        \caption{\small{PFC Time}}
        \label{fig:google_incast:pfc}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small Google distribution with 55\% load + 5\% 100-1 incast. BFC tracks the ideal behavior, improves FCTs, and reduces buffer occupancy. For FCT slowdown, both the x and y axis are log scaled.}
    \label{fig:google_incast}
    \vspace{-4.7mm}
\end{figure*}

 \begin{figure*}
    \centering
    \begin{subfigure}[tbh]{0.48\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/google_fct2.pdf}
        \vspace{-7mm}
        \caption{FCT}
        \label{fig:google:fct}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/google_buffer2.pdf}
        \vspace{-7mm}
        \caption{Buffer Occupancy}
        \label{fig:google:buffer}
    \end{subfigure}
        \begin{subfigure}[tbh]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/google_active_flows.pdf}
        \vspace{-7mm}
        \caption{Active Flows}
        \label{fig:google:active}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small FCT slowdown and buffer occupancy for Google distribution with 60\% load. For all the schemes, PFC was never triggered. \Fig{google:active} shows the CDF of active flows at a port with and without incast. The vertical line shows the total number of queues per port.}
    \label{fig:google}
    \vspace{-5.5mm}
\end{figure*}
 
 \subsubsection{Setup}
 \label{ss:setup}
 
% \smallskip
 \noindent\textbf{Network Topology:}  We use a Clos topology with 128 leaf servers, 8 top of the rack (ToR) switches and 8 Spine switches (2:1 over subscription). Each Spine switch is connected to all the ToR switches, each ToR has 16 servers, and each server is connected to a single ToR. All links are 100\,Gbps with a propagation delay of 1\,us. The maximum end-to-end base round trip time (RTT) is 8\,$\boldsymbol{\mu}$s and the 1-Hop RTT is 2\,$\boldsymbol{\mu}$s. The switch buffer size is set to 12 MB. Relative to the ToR switch capacity of 2.4\,Tbps, the ratio of buffer size to switch capacity is 40\,$\boldsymbol{\mu}$s, the same as Broadcom's Tomahawk3 from \Fig{mot_broadcom}. We use an MTU of 1KB and unless specified otherwise we use Go-Back-N for retransmission. Our experiments use the shared buffer memory model, common in existing switches~\cite{broadcom}. We use flow-level ECMP for all the schemes.
 
 %\smallskip
 \noindent\textbf{Comparison:} \noindent\textit{HPCC:} HPCC is an end-to-end control algorithm that uses explicit link utilization
information from the switches to reduce buffer occupancy and drops/PFCs at the congested switch. We use the parameters from the paper, $\eta = 0.95$ and $maxStage = 5$. The dynamic PFC threshold is set to trigger when traffic from an input port occupies more than 11\% of the free buffer (as in the HPCC paper). We use the same PFC thresholds for DCQCN and DCTCP.% and other variants of HPCC.
 
\noindent\textit{DCQCN:} DCQCN uses ECN bits and end-to-end control to manage buffer use at the congested switch. The ECN threshold triggers before PFC (K$_{min}$ = 100KB and K$_{max}$ = 400KB).
 
 \noindent\textit{DCTCP:} The ECN  threshold is same as DCQCN. Flows start at line rate to avoid degradation in FCTs from slow-start.
 
 \noindent\textit{\bfc{}:} We use 32 physical queues per port (consistent with SwitchX) and our flow table has 76K entries.  The flow table takes 400 KB of memory. We chose per-flow fair queuing as our scheduling mechanism; all the comparison schemes strive for per-flow fairness, thus, fair queuing provides for a just comparison.\cut{; 2) Unlike fair queuing, shortest flow first scheduling (and its approximations) make assumptions about knowing the flow sizes apriori.}
 
 \noindent\textit{Ideal-FQ:} To understand how close \bfc{} comes to optimal performance, we simulate ideal fair queuing with infinite buffering at each switch. The NICs cap the in-flight packets of a flow to 1 BDP. Note that infinite buffering is not realizable in practice; its role is to bound how well we might possibly do on FCTs.
 
 
 %\smallskip
\noindent\textbf{Performance metrics:} We consider three performance metrics: (1) FCT normalized to the best possible FCT for the same size flow, running at link rate (referred as the FCT slowdown); (2) Overall buffer occupancy at the switch; (3) Throughput of individual flows.  %3) Percentage of time links were paused due to PFC;

%\smallskip 
 \noindent\textbf{Workloads:}  We synthesized a trace to match the flow size distributions from the industry workloads discussed in \Fig{mot_flowsize}: (1) Aggregated workload from all applications in a Google data center; (2) a Hadoop cluster at Facebook (FB\_Hadoop). The flow arrival pattern is open-loop and follows a \emph{bursty} lognormal inter-arrival-time distribution with $\sigma$ = 2. For each flow arrival, the source-destination pair is derived from a uniform distribution. We consider scenarios with and without incast, different traffic load settings, and incast ratios. Since our topology is oversubscribed, on average links in the core (Spine-ToR) will be more congested than the ToR-leaf server links. In our experiments, by X\% load we mean X\% load on the links in the core.
 %We report the FCT slowdown for the normal (non-incast) and incast traffic separately.

 \subsubsection{Performance}
 \label{s:eval_performance}

 \Fig{google_incast} and ~\ref{fig:google} show our principal results. The flow sizes are drawn from the Google distribution and 
the average load is set to 60\% of the network capacity. For \Fig{google_incast} (but not \Fig{google}), 5\% of the traffic (on average) is from incast flows. The incast degree is 100-to-1 and the size is 20MB in aggregate. A new incast event starts every 500\,$\mu$s. Since the best-case completion time for an incast is 1.6 ms (20\,MB/100\,Gbps), multiple incasts coexist simultaneously in the network. We report the tail buffer occupancy, the FCT slowdowns at the average, 95$^{\text{th}}$ and 99$^{\text{th}}$ percentile, and the fraction of time links were paused due to PFC. We report the FCT slowdowns for the incast traffic separately in \App{incast_fct}.  
 
Out of all the schemes, DCQCN is worst on latency for small flow sizes, both at the average and the tail. Compared to DCQCN, DCTCP improves latency as it uses per-ACK feedback instead of periodic feedback via QCN.\cut{ the feedback to the sender is more frequent, every ACK instead of periodic feedback via QCN (55us or 5 RTT). }
However, the frequent feedback is not enough, and the performance is far from optimal (Ideal-FQ). The problem is that both
 DCQCN and DCTCP are slow in responding to congestion. 
 Since flows start at line rate, a flow can build up an entire end-to-end bandwidth-delay product 
 (BDP) of buffering (100 KB) at the bottleneck
 before there is any possibility of reducing its rate.
% This leads to long delays particularly at the tail.  Excessive PFC pauses make this even worse.
 The problem is aggravated during incast events. 
The bottleneck switch can potentially accumulate one BDP of packets per incast flow (10MB in aggregate for 100-to-1 incast).

Both protocols have low throughput for long flows. When capacity becomes available, a long flow may fail 
to ramp up quickly enough, reducing throughput and shifting its work to busier periods where it can impact other flows. Moreover, on sudden onset of congestion, a flow may not reduce its rate fast enough, 
slowing short flows.
% further increasing the buffering.

HPCC improves on DCQCN and DCTCP by using link utilization instead of ECN and a better control algorithm. 
Compared to DCQCN and DCTCP, HPCC reduces tail latency, tail buffer occupancy, and PFC pauses (in case of incast). Compared to \bfc{}, however, HPCC has 5-30$\times$ worse tail latency for short flows with incast, and 2.3-3$\times$ worse without. Long flows do worse with HPCC than DCQCN and DCTCP. HPCC aims to maintain small buffers to improve tail latency for short flows, and this means the switch can run of out of packets before the flows ramp up when bandwidth becomes available.
 
Ideal-FQ achieves lower latency than all the schemes. However,
buffer occupancy can grow to an unfeasible level.

BFC achieves the best latency (both average and tail) among all the schemes.
% (close to optimal). 
Without incast, BFC performance
closely tracks optimal.  With incast, incoming flows exhaust the number of physical queues, triggering
HoL-blocking and hurting tail latency.
This effect is largest for the smallest flows at the tail. \Fig{google:active} shows the average number of active flows at a port. In the absence of incast, the number of active flows is smaller than the total queues 99\% of the time, and collisions are rare. 
% This is in line with the queuing theory result stated in \S~\ref{s:discussion}. \footnote{Our setup doesn't meet all the assumptions of the result. In particular, i) The arrival process is a burstier lognormal instead of poisson. ii) The topology is multi-layered with multiple points of congestion. Despite this, most of the time, the active flows are fewer than the total queues.} 
With incast, the number of active flows increase, causing collisions. However,
the tail latency for short flows with BFC is still 5-30$\times$ better than existing schemes. BFC also improves the performance of incast flows, achieving 2$\times$ better FCTs at the tail compared to HPCC (see \App{incast_fct}). 

In the absence of incast, the buffer occupancy for HPCC is similar to that of BFC, but this low buffering comes at the cost of link under-utilization and high FCT for long flows. 

%BFC also improves the performance of incast flows, 2$\times$ better at the tail compared to HPCC (see \App{incast_fct}). In the absence of incast, the buffer occupancy for BFC is higher than HPCC, but this extra buffering is necessary to ensure that flows don't run out of packets at the switch and lose throughput. 

\cut{\Fig{google:active} shows the of number of active flows at a port. In the absence of incast, the number of active flows is smaller than the total queues 99\% of the time, and collisions are rare. This is in line with the queuing theory result stated in \S~\ref{s:discussion}. \footnote{Our setup doesn't meet all the assumptions of the result. In particular, i) The arrival process is a burstier lognormal instead of poisson. ii) The topology is multi-layered with multiple points of congestion. Despite this, most of the time, the active flows are fewer than the total queues.} With incast, the number of active flows increase.}%, thus, collisions are more frequent.} 

Note that, compared to \bfc{} and Ideal-FQ, latency for medium flows (200-1000KB) is slightly better with existing schemes. Because they slow down long flows relative to perfect fairness, medium flows have room to get through more quickly. Conversely, tail slowdown is better for long flows than medium flows with \bfc{} and Ideal-FQ. Long flows achieve close to the long term average available bandwidth, while medium flows are more affected
by transient congestion. %Finally, BFC also improves the performance of incast flows, 2$\times$ better at the tail compared to HPCC (see \App{incast_fct}).
 

  \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip, width=\textwidth]{images_nsdi21/fb_incast_fct.pdf}
        \vspace{-7mm}
        \caption{55\% + 5\% 100-1 incast}
        \label{fig:fb:incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/fb_fct.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:fb:no_incast}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small FCT slowdown (99$^{th}$ percentile) for Facebook distribution with and without incast. }
    \label{fig:fb}
    \vspace{-5.5mm}
\end{figure}
 
 We repeated the experiment in \Fig{google_incast} and ~\ref{fig:google} with the Facebook distribution. \Fig{fb} shows the 99$^{th}$ percentile FCT slowdown. The trends in the FCT slowdowns are similar to that of the Google distribution. We omit other statistics presented earlier in the interest of space, but the trends are similar to \Fig{google_incast} and ~\ref{fig:google}. Note that the x-axis in \Fig{fb} from \Fig{google_incast} and ~\ref{fig:google} because the flow size distribution is different. Henceforth, all the experiments use the Facebook workload.% (for reducing RAM consumption in simulations). With the Google workload, flow sizes are smaller, as a result total number of flows in the experiment duration is higher. All the simulators in our evaluation create an application per flow, and the RAM consumption is very high.
 




   \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/fb_incast_fct_variants2.pdf}
         \vspace{-7mm}
        \label{fig:fb_variants:incast}
        \caption{55\% + 5\% incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/fb_fct_variants2.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:fb_variants:noincast}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small FCT slowdown (99$^{th}$ percentile) of HPCC variants, using the setup in \Fig{fb}.}
    \label{fig:fb_variants}
    \vspace{-5mm}
\end{figure}
 
 
 %\smallskip
 \noindent\textbf{Comparison with HPCC and DCTCP variants:}
 To better understand the benefits of BFC, we added advanced features to HPCC and repeated the experiment in \Fig{fb}. \Fig{fb_variants} reports the FCTs with these variants. We also show BFC and the original HPCC (with PFC) in the results.
 
\textit{Scheduling:} First, we evaluate HPCC+SFQ, a scheme that combines HPCC with better scheduling at the switch. Each egress port does stochastic fair queuing on incoming flows. To match BFC we use 32 physical queues. Adding scheduling improves tail latency by allowing different flows to be scheduled from different physical queues. However, the FCT slowdowns are still worse than BFC, because: (i) There are collisions in assigning flows to physical queues. A small flow sharing the queue with other flows will see its packets delayed. (ii) Regardless of scheduling, HPCC adjusts rates in an end-to-end manner, leading to poor control of buffer occupancy and low throughput for long flows. In particular, with incast, HPCC+SFQ builds deep buffers and experiences PFC pauses at the same rate as HPCC, both of which hurt latency. 
% Moreover, for long flows, adding SFQ doesn't help in either scenario, and the throughput is still worse compared to BFC.
 
\textit{Retransmission:} Next, we replace PFC in HPCC with perfect retransmission.  Without incast, the performance is identical to HPCC as PFC is never triggered in this scenario. With incast, HPCC + Perfect Retransmission improves performance compared to HPCC but is still far from BFC. Retransmission on its own doesn't reduce buffer occupancy, but it does help tail latency of medium flows with incast.
\cut{Moreover, with incast the switch experiences drops, retransmitted packets incur additional delay and consume bandwidth hurting latency of other flows. So while retransmission improves performance, it does not remove the need for congestion control.
 As mentioned earlier, the FCTs for medium flows can be better than BFC as all variants of HPCC only slow down long flows, and medium flows can get through quicker.}
 
\textit{Slow-start:} We also evaluate the impact of using TCP slow-start instead of starting flows at line rate. We compare the original DCTCP with slow start (DCTCP + SS) and our modified DCTCP where flows start at the line rate. With incast, DCTCP + SS reduces buffer occupancy by reducing the intensity of incast flows, improving tail latency. However, it also increases median FCTs by up to 2$\times$. Flows start at a lower rate, taking longer to ramp up to the desired rate. In the absence of incast, it increases both the tail and median FCT for short flows. See \App{ss} for details.


%We compare the original DCTCP with slow start (DCTCP + SS) with an initial window of 10 packets versus the modified DCTCP used so far (initial window of the BDP). With incast, DCTCP + SS reduces buffer occupancy by reducing the intensity of incast flows, improving latency. However, in the absence of incast, slow start increases the tail latency for medium flows (0.5-5 BDP). Flows start at a lower rate, taking longer to ramp up to the desired rate.  However, short flows are still slower than with BFC, because slow start does not remove burstiness in buffer occupancy in the tail.
\cut{
  \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/ss_incast.pdf}
        \vspace{-7mm}
        \caption{55\% + 5\% 100-1 incast}
        \label{fig:ss:incast}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/ss.pdf}
        \vspace{-7mm}
        \caption{60\%}
        \label{fig:ss:no_incast}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Impact of using slow start on 99\% tail latency. DCTCP + SS (slow start) reduces FCTs in the presence of incast. However, in the absence of incast, it increases the tail FCT for medium flows without affecting the tail FCT for short flows.}
    \label{fig:ss}
    \vspace{-4mm}
\end{figure}
}

\subsubsection{Stress-testing BFC}
\label{s:limits}
In this section we stress-test BFC under high load and large incast degree. Flow arrivals follow a bursty lognormal distribution ($\sigma=2$). We evaluate BFC under two different queue configurations: (1) 32 queues per port (BFC 32); (2) 128 queues per port (BFC 128). We show the average slowdown for long flows (> 3MB) and 99$^{th}$ percentile slowdown for short flows (< 3KB).

%We use the Facebook distribution for flow sizes. 


 \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/load_long_avg.pdf}
         \vspace{-7mm}
        \caption{Average FCT for long flows}
        \label{fig:load_var:long}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/load_short2.pdf}
        \vspace{-7mm}
        \caption{Tail FCT for short flows}
        \label{fig:load_var:short}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Average FCT slowdown for long flows, and 99$^{th}$ percentile tail FCT slowdown for small flows, as a function of load.}% At very high loads, BFC 32 incurs substantial HoL-blocking due to collisions. These collisions degrade the tail latency for short flows but not the throughput of long flows.}
    \label{fig:load_var}
    \vspace{-3.5mm}
\end{figure}

%\smallskip
\noindent\textbf{Load:}
%We vary the average load from 50 to 90\% (without incast). 
%Recall that the load factor is for oversubscribed core switches; leaf switches have more capacity. 
%\Fig{load_var:long} shows the median slowdown for long flows (> 3MB). \Fig{load_var:small} shows the 99$^{th}$ percentile slowdown for short flows (< 3KB). 
\Fig{load_var} shows the performance as we vary the average load from 50 to 95\% (without incast). HPCC only supports loads up to 70\%. At higher loads, it becomes unstable (the number of outstanding flows  grows without bound), in part due to the overhead of the INT header (80\,B per-packet). %BFC and DCTCP were stable across all load values. 
All other schemes were stable across all load values.

% (12\% relative to the average load). %In contrast the overhead for BFC is only 1\%.\cut{, for DCQCN and DCTCP the overhead is 4\% (with 40KB ACK).}


At loads $\leq$ 80\%, BFC 32 achieves both lower tail latency (\Fig{load_var:short}) for short flows and higher throughput for long flows (\Fig{load_var:long}). The tail latency for short flows is close to the perfect value of 1. At higher loads, flows remain queued at the bottleneck switch for longer periods of time, raising the likelihood that we run out of physical queues, leading to head of line blocking. This particularly hurts tail performance for short flows as they might be delayed for an extended period if they are assigned to the same queue as a long flow.
% get paused unnecessarily for a while when sharing the queue with a long flow causing congestion at the downstream. 
At the very high load of 95\%, the HoL-blocking degrades tail latency substantially for BFC 32. However, it still achieves good link utilization, and the impact of collisions is limited for long flows. 

Increasing queues, reduces collisions and the associated HoL-blocking. BFC 128 achieves better tail latency for short flows at load $\geq 90\%$.

\cut{Across all the load values, BFC achieves both lower tail latency (\Fig{load_var:short}) for short flows and higher throughput for long flows (\Fig{load_var:long}). The tail latency for short flows is close to the ideal value of 1 except at 90\% load. At higher loads, flows remain queued at the bottleneck switch for longer periods of time, raising the frequency that we run out of physical queues, leading to head of line blocking. This particularly hurts tail performance for short flows as they might get stuck behind a long flow sharing the same queue. BFC achieves high link utilization even in the presence of collisions, and the impact of collisions is limited for long flows.}

%Since BFC provides coarse-grained fairness among flows sharing the same physical queue with round robin resumes(\S\ref{s:backpressure}), the impact of collisions is limited for long flows.

\cut{ leave for the Appendix, no need to mention it here, as its a non-result
In our setup, the links in the core are more congested than the ToR-leaf links. We repeated the experiment in \Fig{load_var} with spacial locality in source-destination pairs such that the average load on all links across the network is same. The trends with spacial locality are similar. BFC incurs HoL blocking for short flows only at 90\% load (see \App{load_var:locality}).
}


 \begin{figure}[t]
    \centering
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/incast_long_avg.pdf}
         \vspace{-7mm}
        \caption{Average FCT for long flows}
        \label{fig:incast_var:long}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.235\textwidth}
        \includegraphics[trim={0 0 0 4mm}, clip,width=\textwidth]{images_nsdi21/incast_short.pdf}
        \vspace{-7mm}
        \caption{Tail FCT for short flows}
        \label{fig:incast_var:short}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Average FCT slowdown for long flows, and 99$^{th}$ percentile tail FCT slowdown for small flows, as a function of incast degree.}% The x-axis is not to scale.} %As the incast degree increases, the frequency of collisions and the associated HoL-blocking increases, degrading FCTs.}
    \label{fig:incast_var}
    \vspace{-5.5mm}
\end{figure}

\noindent\textbf{Incast degree:}
If the size of an incast is large enough, it can
exhaust physical queues and hurt performance. \Fig{incast_var} shows the effect of varying the degree of incast on performance. The average load is 60\% and includes a 5\% incast. The incast size is 20MB in aggregate, but we vary the degree of incast from 10 to 2000. %BFC is shown as BFC (32) for 32 physical queues per port.

For throughput, both BFC 32 and BFC 128 perform well as long as the incast degree is moderate compared
to the number of queues. Both start to degrade around 15$\times$ the number of queues per port.
Below this, BFC can leverage the fanin from the larger number of upstream queues (and greater
aggregate upstream buffer space) to keep the incast
from impeding unrelated traffic (\S\ref{s:qassignment}). As the incast degree scales up farther, 
BFC 32 is able to retain some of its advantage relative to HPCC and DCTCP.
% \pg{\sout{This suggests that under moderately severe collisions, BFC does not underutilize the network.}}

For high incast degree, the tail latency for short flows converges to that of HPCC and DCTCP (\Fig{incast_var:short}). The tail is skewed by the few percent of small requests
that happen to go to the same destination as the incast. (Across the 128 leaf servers in our setup, several servers are the target of an incast at any one time, and these also receive their share 
of normal traffic.) 
% this seemed overkill tbh
% \footnote{\pg{A simple calculation shows that the fraction of such requests is atleast 2.5\%. In our setup, a new incast event starts every 500\,$\mu$s and lasts atleast 1.6\,ms (20\,MB/100\,Gbps). This implies the average number of active incasts is > 3.2 (1.6\,ms/500\,$\mu$s). Since there are 128 leaf servers, at a given time, on average > 2.5\% of the destinations would be receiving an active incast (3.2/128).}}
As the incast degree increases, more small flows share physical queues with incast flows, leading
to more HoL-blocking.

% (at the destination egress and its upstreams)} 
%As the incast degree increases, more and more flows start sharing physical queues at the destination egress, and HoL blocking for short flows increases.  

% abuffers to keep the incast from 
% BFC 32 performs well up to moderate incast degree values (15$\times$ the number of queues) because it can leverage the upstream buffers
% As the incast increases, more and more flows start sharing physical queues, and HoL blocking for short flows increases. At higher incast degree values ($\geq$ 500), the tail latency for short flows converges to that of HPCC and DCTCP (\Fig{incast_var:short}). The throughput of long flows also degrades with incast degree (\Fig{incast_var:long}). 

%Increasing queues, reduces collisions and the associated HoL blocking. 

% Compared to BFC 32, BFC 128 incurs fewer collisions and performs better as a result. In particular, the throughput of long flows is high even when the incast degree is 2000 (15$\times$ the number of queues). This suggests that under moderately severe collisions, BFC does not underutilize the network.


%For the incast flows sharing the queue collisions don't matter much.

%In particular, even at the higher incast degree (2000 or 15$\times$ the number of queues), BFC only marginally underutilizes the network and the throughput of long flows is high.

%In particular, the throughput of long flows degrades marginally even when the incast degree is 2000 (15$\times$ the number of queues). This suggests that under moderately severe collisions, BFC doesn't underutilize the network.  

\if 0
\begin{figure}[t]
     \centering
    \includegraphics[width=0.99\columnwidth]{images_nsdi21/massive_incast.pdf}
    \vspace{-4mm}
    \caption{\small Performance with large incast fan-in (1000-1).}
    \label{fig:incast_var}
    \vspace{-6mm}
 \end{figure}

%\smallskip
\noindent\textbf{Massive Incast:}
If the size of an incast is large enough, it can exhaust physical queues and hurt performance.
\Fig{incast_var} shows the average and tail latency when the degree of incast is 1000:1. The average load is 60\% including the 5\% load from incast traffic. The incast size is 20MB in aggregate. %BFC is shown as BFC (32 queues) for 32 queues per port.

With 32 queues per port (BFC (32)), BFC incurs frequent collisions in the physical queues. These collisions cause HoL blocking, and the performance deviates from IdealFQ. However, BFC still outperforms HPCC by up to 3$\times$. \pg{clarify. Notice that in case of collisions, BFC only pauses flows sharing the queue with the flow causing congestion, and therefore a limited fraction of the flows incur HoL blocking.}% In contrast, with HPCC all flows sharing the egress port with a congested flow incur HoL blocking. 

Increasing physical queues, reduces collisions and the associated HoL blocking. With 128 queues, the performance is close to IdealFQ.
\fi

%the collisions primarily occur at the last hop, i.e., at the egress port connecting the ToR and the incast receiver. Since we do not allow servers to pause the ToR, these collisions don't hurt the tail latency much (performance is close to IdealFQ). This implies that any incast within a rack will have minimal impact. In larger topologies than the one we simulate, where the fan-in into the ToR is higher, the backpressure will be spread out over more upstream switches, dissipating the effect except for very large incasts.

\cut{To reduce contention for physical queues, we tried a variant of BFC that uses per-destination fair queuing -- all flows to the same destination share the same queue. In \Fig{incast_var}, this is shown as BFC + Dest. FQ. Regardless of the incast degree, BFC + Dest. FQ doesn't incur HoL blocking from running out of physical queues, and it outperforms all other schemes. Performance is even better than IdealFQ (per flow). When there are multiple incast flows at an egress port, per-flow fair queuing will allocate more bandwidth to the incast flows in aggregate than per-destination fair queuing, reducing performance for the non-incast flows.

While per-destination fair queuing is better than per-flow fair queuing under massive incasts, it presents a trade-off. With per-destination fair queuing, flows to the same destination share a physical queue. A destination that receives a mixture of short and long flows will incur significant delays for short flows in the tail of the distribution. This effect worsens as load increases. We also considered a hybrid approach, where the sender labels incast flows (similar to ~\cite{homa}). This performs best but assumes application help, and so we use a more
conservative design for the main body of our evaluation.}
% In the interest of space, we omit their description. 
% We assign a single physical queue to the incast flows. For the non-incast flows, the switch uses the original queue assignment and simply does per flow fair queuing. As a result, the hybrid scheme is able to achieve good performance both under massive incasts and high loads. Since the feasibility in practice is unknown, we chose per flow fair queuing as our baseline scheme. We note that both the variants of BFC discussed above require modifications to bookkeeping. In the interest of space, we omit their description. 

\cut{
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.46\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/pq_load.pdf}
        \vspace{-7mm}
        \caption{60\% and 90\% load}
        \label{fig:pq:load}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/pq_incast_fct.pdf}
        \vspace{-7mm}
        \caption{55\% +5\% incast}
        \label{fig:pq:incast}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/pq_incast_fct_collisions.pdf}
        \vspace{-7mm}
        \caption{Collisions (incast)}
        \label{fig:pq:incast+hol}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Impact of number of physical queues.}
    \label{fig:pq}
    \vspace{-5mm}
\end{figure}
%\smallskip
\noindent\textbf{Number of physical queues:} We evaluate the impact of the number of physical queues on performance. We vary the number of physical queues per port from 8 to 128. \Fig{pq:load} shows the 99$^{th}$ percentile FCT slowdowns with 60 and 90\% load (no incast). \Fig{pq:incast} shows the FCT slowdown with 55\% load + 5\% incast (100-1). \Fig{pq:incast+hol} shows the fraction of flows that share the same physical queue (collisions) in the incast scenario. Both the experiments use the Facebook distribution.

As expected, decreasing the number of physical queues causes collisions. In the absence of incast, the degradation in performance is gradual. With 60\% load, the performance plateaus at 16 queues. With 90\% load, the number of active flows increase, and the performance plateaus at 64 queues. With incast, the knee of the curve is at 32 queues, while increasing queues beyond 64 doesn't improve performance. With 64 queues, the collisions primarily occur at the last hop, i.e., at the egress port connecting the ToR and the incast server. We do not allow servers to pause the ToR, so these collisions don't hurt the tail latency much (performance is close to IdealFQ). This implies that any incast within a rack will have minimal impact. In larger topologies than the ones we simulate, where the fan into the ToR is higher, per-flow backpressure will be spread out over more upstream switches, dissipating the effect except for very large incasts.}


\cut{Interestingly, with 64 queues, the collisions primarily occur at the last hop, i.e., at the egress port connecting the ToR and the incast leaf server; the incast flows are spread out at the higher layers and the number of active incast flows is smaller than the last hop. BFC maintains the buffer occupancy of a physical queue at a low level, and collisions degrade performance primarily because of hol-blocking from pauses. Since egress ports at the last hop cannot be paused by the upstream leaf server, these collisions don't hurt the tail latency much (performance is close to IdealFQ).
This implies BFC can handle bigger incasts, if the incasts are within the same ToR. Additionally, in larger topologies where the FanIn from Core to ToR is higher, the collisions will primarily occur at the very last hop and won't degrade performance as much. \cut{\pg{Can we say this without explicit experiments? The experiment with locality in incast is easy to run.}}

% I cut these two paragraphs too.  This is speculation.  If you want to say it, say it earlier when we discuss trends in switch design (e.g., that we'll be able to pause in the datapath.
Note that across all the scenarios (heavy load and incast), the required number of physical queues is 64, higher than the number in existing switches. The results in this section make a case for increasing the physical queues in switches. We believe that the number of physical queues can be scaled to a few hundreds without hurting the capacity of existing switches.

% OK to include the appendix, but no need to mention it.
We also repeated the experiment in \Fig{pq:incast} but varied the size of the bloom filter and the flow hash table instead. BFC's performance is not sensitive to either of these resource constraints (see ~\App{sensitivity} for details). 

}



\subsubsection{Additional experiments}
%\smallskip

\noindent\textbf{Incremental Deployment:} 
We repeated the experiment in \Fig{fb:incast} in the scenario where (i) BFC is deployed in part of the network; (ii) The switch doesn't have enough capacity to handle all the recirculations. The impact on FCTs is minimal under these scenarios (see \App{incr_deploy}).

\noindent\textbf{Impact of scheduling policy:}
The design of BFC is orthogonal to the scheduling policy. We repeat the experiment in \Fig{fb}, but change the scheduling policy from fair queuing (FQ) to shortest remaining flow first (SRF). With SRF, BFC reduces FCTs by prioritizing short flows (see \App{impact_srf}).

\noindent\textbf{Performance in asymmetric topologies:} BFC makes no assumption about the topology, link speeds and link delays. We evaluate the performance of BFC in a multi-datacenter topology. BFC achieves low FCT for flows within the datacenter, and high link utilization for the inter-datacenter links (see \App{cross}). 

\noindent\textbf{Importance of dynamic queue assignment:} We  repeat  the  experiment in \Fig{fb:incast} but use stochastic hashing to statically assign flows to physical queue instead. With stochastic assignment, collisions in physical queue increase, hurting FCTs (see \App{qassign}).

\noindent\textbf{Size of flow table:} Reducing the size of the flow table can increase index collisions in the flow table, potentially hurting FCTs. We repeat the experiment in \Fig{fb:incast} and evaluate the impact of size of flow table. Reducing the size impacts the short flow FCTs partly (see \App{sensitivity}).


\noindent\textbf{Reducing contention for queues:} We tried a variant of BFC where the sender labels incast flows explicitly (similar to~\cite{homa}). All the incast flows at an egress port are assigned to the same queue. This frees up queues for non-incast traffic and reduces collisions substantially under large incasts. (see \App{isolate_incast}).



==> intro.tex <==
\newcommand{\introsec}{Introduction}
\section{\introsec}
\label{s:intro}

Single and multi-tenant data centers have become one of the largest and fastest growing segments of the computer industry.
Data centers are increasingly dominating the market for all types of high end computing,
including enterprise services, parallel computing, large scale data analysis, fault tolerant
middleboxes, and global distributed applications~\cite{googlecloud,azure,s3}.  These workloads
place enormous pressure on the data center network to deliver, at low cost,
ever faster throughput with low tail latency even for highly bursty traffic~\cite{dean2013tail,zats2012detail}.

Although details vary, almost all data center networks today use a combination of endpoint congestion control,
FIFO queues at switches, 
% priority for a small amount of latency-sensitive traffic, 
and explicit feedback of switch state back to the endpoint control loop.  
As link speeds continue to increase, 
however, the design of the control loop becomes more difficult. More traffic fits within a single round trip,
making it more difficult to use feedback effectively. Traffic remains highly bursty, so that
network load is not a stable property except over very short time scales. The amount of switch
buffering is decreasing relative to link speeds. And switch buffer occupancy 
must be kept low to reduce tail latency, which can have a multiplicative effect on application performance. 
As a result, most network operators run their networks at very low average load, throttle long flows
at far below network capacity, and even then see significant congestion loss.

\if 0
To help address these demands, RDMA (Remote Direct Memory Access) has emerged as a popular
protocol for very high-bandwidth end host communication.
With RDMA, applications directly read and write protected regions of memory on other
machines, with the protocol implemented in hardware without the 
need to interrupt or process requests in software on the remote node,
and with an assumption that network packet losses are very low.
As such, RDMA is simple enough to be implemented
for 100\,Gbps links and beyond~\cite{mellanox}.

An ongoing challenge for deploying RDMA, particularly for multi-tenant data centers,
is network congestion control. A commonly used option is PFC (Priority Flow Control)~\cite{PFC},
where switches send blanket pause frames one hop upstream to prevent buffer overflow and packet loss.
These pause frames can cause head-of-line (HoL) blocking where unrelated traffic
is stalled waiting for other flows to release downstream buffers. To address this, most data center operators
add some form of end-to-end congestion control to avoid triggering pause frames.  Two examples are
DCQCN~\cite{dcqcn} and HPCC~\cite{hpcc}; these use sophisticated control theory to rate-limit 
individual flows to better manage resources in the middle of the network.

Unfortunately, tail latency performance -- often the key metric for applications
using RDMA -- degrades with DCQCN or HPCC under load, to a far greater degree
than would be predicted by queueing theory. One could add better switch scheduling 
algorithms, such as fair queueing, but we show that even the combination of DCQCN
and fair queueing remains far from optimal for tail latency for typical network
workloads and configurations.  This gap is likely to widen as network speeds increase.
\fi

Instead, we propose a different approach, to revisit the idea of per-hop per-flow
flow control.  The key challenge for data center networks, in our view, is to efficiently 
allocate buffer space at congested network switches. This becomes easier and simpler when control actions
are taken per flow and per hop.  

Per-hop per-flow flow control is not a new idea, 
having been introduced with ATM networks over two decades ago~\cite{anderson1993high,kung1995credit}.  
These earlier schemes required per-flow state at each switch even for quiescent flows, something
that would not be practical with today's space-limited switch chips. Instead, we show that
per-hop per-flow flow control can be implemented with a small amount of switch state and
a modest amount of signalling overhead. We note that our approach is approximate, and so unlike ATM
we are not completely loss-free. Instead, we assume an end-to-end recovery system 
such as TCP or IRN~\cite{irn}.

We evaluate our approach, called BFC (Backpressure Flow Control), using ns3~\cite{ns3} on synthetic traces
drawn to be consistent with measured workloads from Google and Facebook data centers~\cite{homa} and a
multi-level Clos network topology. We show that BFC, unlike previous approaches such as 
DCTCP, DCQCN, and HPCC, achieves close to optimal tail latency performance on these workloads for 
short, medium, and long flows, 
even when the network is heavily loaded or disrupted by incast traffic.

Our specific contributions are:

\begin{CompactItemize}
    \item A discussion of the fundamental limits of end-to-end congestion control for high bandwidth data
    center networks.
    \item A detailed protocol for per-hop per-flow flow control, called BFC, that uses a small amount of
    metadata to achieve near-optimal tail-latency performance for typical data center workloads.
%    \item An idealized CUT model of data center network congestion control, to explain when per-hop flow control will and will not outperform end-to-end congestion control.
    \item An evaluation of BFC against both widely used and recently proposed end-to-end 
    congestion control algorithms, on synthetic traces drawn from measured data center workloads.
\end{CompactItemize}

\noindent Our code and simulation harness is public and can be made available to the reviewers on request.
A limitation of our work is that it requires a few features not available on today's commercially available 
programmable switches, but our approach is compatible with the likely near-term evolution of those switches.

\if 0
% don't think we need any of these anymore.  The hardware limitation is still there, but best discussed later.
There are several important limitations to our work. 

(ii) Our approach is designed to be able to be combined with different switch scheduling algorithms,
such as hierarchical round robin and priority scheduling. In this paper, however, we only compare to fair queueing.
(iii) We have not completed a detailed hardware design for BFC, and so we are unable to give a precise
estimate of the VLSI chip area needed for its implementation. BFC could be implemented in P4, but
it requires scheduling control beyond
the capability of current generation Openflow v2 switches.
(iv) Our evaluation is limited to RDMA congestion control algorithms.
We believe our hop-by-hop approach will compare favorably to TCP congestion control ~\cite{dctcp, bolt},
but we do not present a quantitative comparison at this time. 

\fi

% \pg{\tom{i think that's implicit.} Maybe w should say SACK/smart retransmission explicitly for TCP.}

\if 0

\pg{A short introduction assuming some of the key properties/design principles will be demonstrated in section 2}

\tom{Need a bit more stage setting to begin with.  Not sure but maybe the better place is to start with an assumption of RDMA, and its one-sided nature means that traditional feedback cc doesn't work that well, even with pause frames and heavy duty control theory.  then pivot to the trends that make this worse.}

\tom{or if the pitch is dcn cc in general, this might work:} \pg{I like it, integrating.}
In part due to the commercial importance of data centers, data center network congestion control has received lots of attention from both industry (~\cite{dcqcn}, ~\cite{hpcc}) and academic researchers (~\cite{homa}, ~\cite{timely}).  Despite the more constrained environment for data center networks (constrained topologies, small spread of link speeds relative to the Internet, small spread of end to end delays), achieving both good performance and high utilization remains a challenge (cite).

An ongoing problem is the inevitable tradeoff between designs that are good for different types of applications.  Some apps are very latency sensitive, and particularly tail latency sensitive -- e.g., send frequent short messages, such as for RPC or remote memory access (RDMA).  Meanwhile other applications need to use the network for transfering larger blocks of data, but are more latency tolerant provided they can consume the available bandwidth without impacting the latency requirements of low latency flows.  Measured data from existing data center networks implies that most communication requests are small, but most bytes are in large requests. Several trends are making this situation worse.

In the recent years, data center networks have experienced a steady increase in the link speed. While increasing link speeds can improve throughput for applications, they can make maintaining low tail latencies challenging for short flows. Traditional data center congestion control algorithms (DCQCN~\cite{dcqcn}, DCTCP~\cite{dctcp}, Timely~\cite{timely}, HPCC~\cite{hpcc}) adjust their rates/congestion window based on the feedback from switches (e.g., ecn or int marks). Because of this feedback delay, these protocols react on the scale of a RTT and might take multiple RTTs to converge. With increasing link speeds, a flow/message instead of taking multiple RTTs to complete might now finish within a couple of RTTs (e.g., a 150KB message can finish within 12us ($\sim$ 1 RTT) on 100Gbps links). The fraction of traffic contributed by such short flows (size $<$ 1-2 BDP) is increasing with increasing link speeds. These short flows can thus fill up the buffer before the congestion control can even reduce their rates, increasing tail latencies. 


\pg{Should we talk more about the fact some of these problems for short flow are because they flows start at line rate, changing that would result in higher FCTs? Maybe we can bring this up in the design principles section as a property of our system.}
\tom{I wouldn't - the issue isn't that short flows start at line rate, its that I want low latency for short flows (which implies that they should start at line rate!), but I still want congestion management for short flows when they overwhelm the network (e.g., incast).  Meanwhile I want long flows to use up the remainder.}

\tom{not sure you should introduce buffering here. Or if you do, isn't it: advanced scheduling (like afq and others) offers a possible answer by allowing short flows to be scheduled preferentially ahead of long flows, but a challenge is managing buffering}

There are two trends which make the problem of achieving low tail latencies on high speed links even more challenging. First, switch buffers are not scaling as fast as link speeds because of chip density constraints. This implies that during congestion episodes, the switch buffer will fill up quicker, causing drops or pausing links (e.g., via PFC~\cite{PFC}), both of which hurt latency and throughput. Second, the flow size distribution of data center workloads in not scaling with the increase in link speeds, instead the flow sizes are getting shorter ~\cite{homa}. In a data center workload trace released by google, more than 50\% of the traffic is contributed by flows with size lesser than 150KB (1 BDP on 100Gbps links). Decreasing or similar flow sizes imply that a larger fraction of the traffic is contributed by short flows that finish within a couple of RTTs, before the congestion control protocol can even reduce their rates to avoid buffer build up. \pg{should we put a figure on flow size distribution similar to HOMA?}


\tom{i would say the problem with long flows is that the same scheduling solutions like afq that work for short flows, make the control loop behavior of long flows untenable - bursty priority traffic means it is very hard to pick a stable flow.  flooding when there is available bandwidth requires driving the buffers up, which then causes problems.  Don't you need to introduce the idea of HoL blocking in here somewhere?} \pg{Not sure if we should tie the problem to the scheduling.} \pg{Adding to that, maybe we should also say that for first 1-2 BDP of packets for longer flows one might face problems similar short flows?}
Moreover, for longer flows, these congestion control protocols also face a trade-off between either being too slow to grab the available bandwidth and causing underutilization or being too aggressive and filling up the buffers. Another caveat is that on higher speed links the flows finish faster, therefore, the rate at which available bandwidth varies increases, aggravating this trade-off. These schemes have a variety of parameters one can tune to control this trade-off. The right set of parameters for a scheme depends on both the link speed and the flow size distribution. In practice, it requires a lot of manual tuning  to get a reasonable set of parameters for a particular scheme in a given environment~\cite{hpcc}.

\tom{not quite clear what the figure is supposed to show?  tail latency fct is worse with higher link speeds?  is the problem the pause frames or just that DCQCN throttles back too much in an attempt to avoid pause frames.  If the latter,  I might instead compare DCQCN for tail latency vs. a system with arbitrary switch buffers (maybe that's what you mean?).  That is, DCQCN (and presumably HPCC) doesn't get close to optimal, so there remains room for improvement, and in fact they are getting farther away from optimal as we increase link speeds for typical request distributions.  I might also try throwing a 1 percent incast workload - that is, a problem is that these systems are multi-tenant, and so you can't control what other apps are doing, and even small temporary overloads are enough to disrupt performance for small flows.}


Supplementing congestion control with scheduling of flows at the switches (e.g., deploying Stochastic Fair Queuing with DCQCN) can help reduce head of line blocking due to buffer build up to a certain degree ~\cite{afq}. But scheduling alone is not enough, the problem is that adding scheduling in itself doesn't limit the amount of buffer build up. As a result, during congestion episodes, the switches can experience drops or paused links hurting performance. 

A potential solution to this problem is moving congestion control to the switches enabling finer granularity control over the traffic. Priority-based Flow Control ~\cite{PFC}, is one such mechanism (used in both DCQCN and HPCC) that tries to limit the buffer build up at the switch by pausing traffic from incoming links in case the switch buffer starts filling up. While, by moving some control to the switches PFC is able to reduce the drops significantly, it causes head of line blocking for flows as it pauses all the flows (belonging to a particular priority) even if some of them are not building up the buffers. This results in an unnecessary degradation in tail latencies for such flows. 

\tom{system naming: Selective Pause Frames? to distinguish from per-flow credits.  maybe I think there are too many of these systems that have C in the title so they all sound similar.}
We propose Backpressure Flow Control (BFC), a practical scheme that enables a switch to pause the flows at the upstream switch that are filling up the buffers at the current switch. BFC enables finer granularity congestion control to reduce buffering without causing head of line blocking or compromising throughput of a flow. Current switches support multiple FIFO Queues per egress port at a switch. On a new flow arrival the switch assigns the flow to a particular physical queue at the egress port corresponding to the flow. Based on congestion information from the downstream switch, the switch pauses/resumes these physical queues to mimic hop-by-bop per flow pausing. A switch only keeps track of a limited number of flows with packets in the switch, the switch uses this per flow information for deciding which flows to pause/resume at the upstream switch and to look up the physical queue assigned to a flow on arrival of a packet. BFC supports a variety of scheduling policies on the physical queues, e.g., Round Robin, Hierarchical Fair Queuing, etc. A key property of BFC is that it decouples the scheduling from the pausing mechanism. NICs in BFC are fairly simple and don't do any congestion control except pausing/resuming flows based on the congestion information from the downstream switch. The NIC schedules the unpaused flows at the line rate. BFC doesn't require manual tuning of parameters and is robust to changes in flow size distribution and link speed. We also establish bounds on memory required by BFC for book keeping at the switch and the bandwidth required for communicating congestion information across switches, and, show that BFC is realizable in practice.
\pg {Introduce buffer pooling in the design principles or here?}

\pg{We evaluated BFC in simulation using the ns-3 simulator. Our key findings are:}
\tom{also: key contributions, e.g., effective selective pause frames without per flow state}

\fi




%1. Explain the trends in modern data centers. Things are happening. Short (picture HOMA flow size distribution, Normalized buffer size)  (RDMA tranpsport moved into hardware -> PFC creates concnern about congestion spreading, congestion control have been designed to reduce PFC triggers, incast
%2.  Trends making this design challenging. Buffer Size, LinkSpeed, Short message sizes, fi). 
%2. Consequences of the trends -> More reactive stuff required. 
%3. Use Cases . 

==> intro_nsdi21.tex <==
\newcommand{\introsec}{Introduction}
\section{\introsec}
\label{s:intro}

Single and multi-tenant data centers have become one of the largest and fastest growing segments of the computer industry.
Data centers are increasingly dominating the market for all types of high-end computing,
including enterprise services, parallel computing, large scale data analysis, fault-tolerant
middleboxes, and global distributed applications~\cite{googlecloud,azure,s3}.  These workloads
place enormous pressure on the data center network to deliver, at low cost,
ever faster throughput with low tail latency even for highly bursty traffic~\cite{dean2013tail,zats2012detail}.

Although details vary, almost all data center networks today use a combination of endpoint congestion control,
FIFO queues at switches, 
% priority for a small amount of latency-sensitive traffic, 
%and explicit feedback of switch state back to the endpoint control loop.  
and end-to-end feedback of congestion signals like delay or explicit switch state to the endpoint control loop.\footnote{We refer to schemes that rely on feedback signals delayed by an entire round-trip-time as {\em end-to-end} schemes, to contrast them with hop-by-hop mechanisms.}
As link speeds continue to increase, 
however, the design of the control loop becomes more difficult. First, more traffic fits within a single round trip,
making it more difficult to use feedback effectively. Second, traffic becomes increasingly bursty, so that
network load is not a stable property except over very short time scales. 
% The amount of switch buffering is decreasing relative to link speeds. 
And third, switch buffer capacity is not keeping up with increasing link speeds,  making it even more challenging to handle traffic bursts. 
%And switch buffer occupancy must be kept low to reduce tail latency.
% , which can have a multiplicative effect on application performance. 
Most network operators run their networks at very low average load, throttle long flows
at far below network capacity, and even then see significant congestion loss.

\if 0
To help address these demands, RDMA (Remote Direct Memory Access) has emerged as a popular
protocol for very high-bandwidth end host communication.
With RDMA, applications directly read and write protected regions of memory on other
machines, with the protocol implemented in hardware without the 
need to interrupt or process requests in software on the remote node,
and with an assumption that network packet losses are very low.
As such, RDMA is simple enough to be implemented
for 100\,Gbps links and beyond~\cite{mellanox}.

An ongoing challenge for deploying RDMA, particularly for multi-tenant data centers,
is network congestion control. A commonly used option is PFC (Priority Flow Control)~\cite{PFC},
where switches send blanket pause frames one hop upstream to prevent buffer overflow and packet loss.
These pause frames can cause head-of-line (HoL) blocking where unrelated traffic
is stalled waiting for other flows to release downstream buffers. To address this, most data center operators
add some form of end-to-end congestion control to avoid triggering pause frames.  Two examples are
DCQCN~\cite{dcqcn} and HPCC~\cite{hpcc}; these use sophisticated control theory to rate-limit 
individual flows to better manage resources in the middle of the network.

Unfortunately, tail latency performance -- often the key metric for applications
using RDMA -- degrades with DCQCN or HPCC under load, to a far greater degree
than would be predicted by queueing theory. One could add better switch scheduling 
algorithms, such as fair queueing, but we show that even the combination of DCQCN
and fair queueing remains far from optimal for tail latency for typical network
workloads and configurations.  This gap is likely to widen as network speeds increase.
\fi

Instead, we propose a different approach.
% , to revisit the idea of per-hop per-flow flow control.  
The key challenge for data center networks, in our view, is to efficiently 
allocate buffer space at congested network switches. 
This becomes easier and simpler when control actions
are taken per flow and per hop, rather than end-to-end. 
Despite its advantages, per-hop per-flow flow control appears to require 
per-flow state at each switch, even for quiescent flows~\cite{anderson1993high,kung1995credit},
something that is not practical at data center scale.
% Per-hop per-flow flow control is not a new idea, 
% having been introduced with ATM networks over two decades ago~\cite{anderson1993high,kung1995credit}.  
% These earlier schemes required per-flow state at each switch even for quiescent flows, something
% that would not be practical with today's space-limited switch chips. 
% Our approach doesn't make simplifying assumptions about network characteristics (\eg NDP~\cite{ndp}, Homa~\cite{homa} assume congestion is only at the last-hop), and generalizes to asymmetric and/or oversubscribed topologies. We note that our approach is approximate, and so unlike ATM
% we are not completely loss-free. Instead, we assume an end-to-end recovery system 
% such as TCP or IRN~\cite{irn}.

Our primary contribution is to show that 
per-hop per-flow flow control can be \emph{approximated} with a 
modest and limited amount of switch state, using only simple constant-time switch operations on a modern programmable switch.
Unlike receiver-driven congestion control like NDP~\cite{ndp} and Homa~\cite{homa}, 
our approach assumes congestion can occur anywhere (not just the last hop) and 
generalizes to asymmetric and oversubscribed topologies. Unlike prior work in
per-hop flow control, our approach is not completely loss-free,
%\footnote{\textcolor{red}{However, losses are rare and typically only occur in extreme scenarios (\S\ref{s:discussion}).}} 
 so we assume an end-to-end recovery system such as Go-back-N, SACK~\cite{sack}, or IRN~\cite{irn}.

We have implemented our approach, {\em Backpressure Flow Control (BFC)}, on a 
state-of-the-art P4-based programmable switch ASIC supporting 12.8 Tbps of switching capacity. 
%400\,Gbps links.
To preserve anonymity we refer to this as SwitchX. 
Our implementation uses less than 10\% of the dedicated stateful memory on SwitchX. 
All per-packet operations are implemented entirely in the dataplane; 
BFC runs at full switch capacity. 
% We also present a proof-of-concept evaluation on a Tofino2 switch.

To evaluate performance, we run large-scale ns-3~\cite{ns3} simulations using synthetic traces
drawn to be consistent with measured workloads from Google and Facebook data centers~\cite{homa} on an oversubscribed multi-level Clos network topology.
We show that BFC, unlike DCTCP, DCQCN, and HPCC, 
achieves close to optimal throughput and tail latency performance for short, medium, and long flows, 
even when the network is heavily loaded or disrupted by incast traffic. Compared to existing schemes, 
BFC achieves 2.3\,-\,60$\times$ better tail flow completion times (FCTs) for short flows, and 1.6\,-\,5$\times$ better average performance for long flows.
Our simulation code will be made public and is available to the reviewers on request.

\cut{
We show that BFC, unlike previous approaches such as 
DCTCP, DCQCN, and HPCC, achieves close to optimal tail latency performance on these workloads for 
short, medium, and long flows, 
even when the network is heavily loaded or disrupted by incast traffic.

We evaluate our approach, called BFC (Backpressure Flow Control), using ns3~\cite{ns3} on synthetic traces
drawn to be consistent with measured workloads from Google and Facebook data centers~\cite{homa} and a
multi-level Clos network topology. We show that BFC, unlike previous approaches such as 
DCTCP, DCQCN, and HPCC, achieves close to optimal tail latency performance on these workloads for 
short, medium, and long flows, 
even when the network is heavily loaded or disrupted by incast traffic.}

Our specific contributions are:

\begin{CompactItemize}
    \item A discussion of the fundamental limits of end-to-end congestion control for high bandwidth data
    center networks.
    \item A practical protocol for per-hop per-flow flow control, called BFC, that uses a small, constant
    amount of state to achieve near-optimal tail-latency performance for typical data center workloads.
    \item An implementation and proof-of-concept evaluation of BFC on a commodity switch. To our knowledge, this is the first implementation of a per-hop per-flow flow control scheme for a multi-Tbps switch. %(\pg{can/should we say something stronger?}
\end{CompactItemize}

%    \item An idealized CUT model of data center network congestion control, to explain when per-hop flow control will and will not outperform end-to-end congestion control.
%    \item \sout{Evaluation of BFC against both widely used and recently proposed end-to-end 
%    congestion control algorithms, on synthetic traces drawn from measured data center workloads.}
% \noindent \pg{Our simulation harness and code can be made available to the reviewers on request. A limitation of our work is that it requires a few features that are not-yet available on other commercially available programmable switches, but our approach is compatible with the likely near-term evolution of those switches.} \pg{say this here or in hardware assumptions?}

\cut{Our code and simulation harness is public and can be made available to the reviewers on request.
A limitation of our work is that it requires a few features not available on today's commercially available 
programmable switches, but our approach is compatible with the likely near-term evolution of those switches.}




\if 0
% don't think we need any of these anymore.  The hardware limitation is still there, but best discussed later.
There are several important limitations to our work. 

(ii) Our approach is designed to be able to be combined with different switch scheduling algorithms,
such as hierarchical round robin and priority scheduling. In this paper, however, we only compare to fair queueing.
(iii) We have not completed a detailed hardware design for BFC, and so we are unable to give a precise
estimate of the VLSI chip area needed for its implementation. BFC could be implemented in P4, but
it requires scheduling control beyond
the capability of current generation Openflow v2 switches.
(iv) Our evaluation is limited to RDMA congestion control algorithms.
We believe our hop-by-hop approach will compare favorably to TCP congestion control ~\cite{dctcp, bolt},
but we do not present a quantitative comparison at this time. 

\fi

% \pg{\tom{i think that's implicit.} Maybe w should say SACK/smart retransmission explicitly for TCP.}

\if 0

\pg{A short introduction assuming some of the key properties/design principles will be demonstrated in section 2}

\tom{Need a bit more stage setting to begin with.  Not sure but maybe the better place is to start with an assumption of RDMA, and its one-sided nature means that traditional feedback cc doesn't work that well, even with pause frames and heavy duty control theory.  then pivot to the trends that make this worse.}

\tom{or if the pitch is dcn cc in general, this might work:} \pg{I like it, integrating.}
In part due to the commercial importance of data centers, data center network congestion control has received lots of attention from both industry (~\cite{dcqcn}, ~\cite{hpcc}) and academic researchers (~\cite{homa}, ~\cite{timely}).  Despite the more constrained environment for data center networks (constrained topologies, small spread of link speeds relative to the Internet, small spread of end to end delays), achieving both good performance and high utilization remains a challenge (cite).

An ongoing problem is the inevitable tradeoff between designs that are good for different types of applications.  Some apps are very latency sensitive, and particularly tail latency sensitive -- e.g., send frequent short messages, such as for RPC or remote memory access (RDMA).  Meanwhile other applications need to use the network for transfering larger blocks of data, but are more latency tolerant provided they can consume the available bandwidth without impacting the latency requirements of low latency flows.  Measured data from existing data center networks implies that most communication requests are small, but most bytes are in large requests. Several trends are making this situation worse.

In the recent years, data center networks have experienced a steady increase in the link speed. While increasing link speeds can improve throughput for applications, they can make maintaining low tail latencies challenging for short flows. Traditional data center congestion control algorithms (DCQCN~\cite{dcqcn}, DCTCP~\cite{dctcp}, Timely~\cite{timely}, HPCC~\cite{hpcc}) adjust their rates/congestion window based on the feedback from switches (e.g., ecn or int marks). Because of this feedback delay, these protocols react on the scale of a RTT and might take multiple RTTs to converge. With increasing link speeds, a flow/message instead of taking multiple RTTs to complete might now finish within a couple of RTTs (e.g., a 150KB message can finish within 12us ($\sim$ 1 RTT) on 100Gbps links). The fraction of traffic contributed by such short flows (size $<$ 1-2 BDP) is increasing with increasing link speeds. These short flows can thus fill up the buffer before the congestion control can even reduce their rates, increasing tail latencies. 


\pg{Should we talk more about the fact some of these problems for short flow are because they flows start at line rate, changing that would result in higher FCTs? Maybe we can bring this up in the design principles section as a property of our system.}
\tom{I wouldn't - the issue isn't that short flows start at line rate, its that I want low latency for short flows (which implies that they should start at line rate!), but I still want congestion management for short flows when they overwhelm the network (e.g., incast).  Meanwhile I want long flows to use up the remainder.}

\tom{not sure you should introduce buffering here. Or if you do, isn't it: advanced scheduling (like afq and others) offers a possible answer by allowing short flows to be scheduled preferentially ahead of long flows, but a challenge is managing buffering}

There are two trends which make the problem of achieving low tail latencies on high speed links even more challenging. First, switch buffers are not scaling as fast as link speeds because of chip density constraints. This implies that during congestion episodes, the switch buffer will fill up quicker, causing drops or pausing links (e.g., via PFC~\cite{PFC}), both of which hurt latency and throughput. Second, the flow size distribution of data center workloads in not scaling with the increase in link speeds, instead the flow sizes are getting shorter ~\cite{homa}. In a data center workload trace released by google, more than 50\% of the traffic is contributed by flows with size lesser than 150KB (1 BDP on 100Gbps links). Decreasing or similar flow sizes imply that a larger fraction of the traffic is contributed by short flows that finish within a couple of RTTs, before the congestion control protocol can even reduce their rates to avoid buffer build up. \pg{should we put a figure on flow size distribution similar to HOMA?}


\tom{i would say the problem with long flows is that the same scheduling solutions like afq that work for short flows, make the control loop behavior of long flows untenable - bursty priority traffic means it is very hard to pick a stable flow.  flooding when there is available bandwidth requires driving the buffers up, which then causes problems.  Don't you need to introduce the idea of HoL blocking in here somewhere?} \pg{Not sure if we should tie the problem to the scheduling.} \pg{Adding to that, maybe we should also say that for first 1-2 BDP of packets for longer flows one might face problems similar short flows?}
Moreover, for longer flows, these congestion control protocols also face a trade-off between either being too slow to grab the available bandwidth and causing underutilization or being too aggressive and filling up the buffers. Another caveat is that on higher speed links the flows finish faster, therefore, the rate at which available bandwidth varies increases, aggravating this trade-off. These schemes have a variety of parameters one can tune to control this trade-off. The right set of parameters for a scheme depends on both the link speed and the flow size distribution. In practice, it requires a lot of manual tuning  to get a reasonable set of parameters for a particular scheme in a given environment~\cite{hpcc}.

\tom{not quite clear what the figure is supposed to show?  tail latency fct is worse with higher link speeds?  is the problem the pause frames or just that DCQCN throttles back too much in an attempt to avoid pause frames.  If the latter,  I might instead compare DCQCN for tail latency vs. a system with arbitrary switch buffers (maybe that's what you mean?).  That is, DCQCN (and presumably HPCC) doesn't get close to optimal, so there remains room for improvement, and in fact they are getting farther away from optimal as we increase link speeds for typical request distributions.  I might also try throwing a 1 percent incast workload - that is, a problem is that these systems are multi-tenant, and so you can't control what other apps are doing, and even small temporary overloads are enough to disrupt performance for small flows.}


Supplementing congestion control with scheduling of flows at the switches (e.g., deploying Stochastic Fair Queuing with DCQCN) can help reduce head of line blocking due to buffer build up to a certain degree ~\cite{afq}. But scheduling alone is not enough, the problem is that adding scheduling in itself doesn't limit the amount of buffer build up. As a result, during congestion episodes, the switches can experience drops or paused links hurting performance. 

A potential solution to this problem is moving congestion control to the switches enabling finer granularity control over the traffic. Priority-based Flow Control ~\cite{PFC}, is one such mechanism (used in both DCQCN and HPCC) that tries to limit the buffer build up at the switch by pausing traffic from incoming links in case the switch buffer starts filling up. While, by moving some control to the switches PFC is able to reduce the drops significantly, it causes head of line blocking for flows as it pauses all the flows (belonging to a particular priority) even if some of them are not building up the buffers. This results in an unnecessary degradation in tail latencies for such flows. 

\tom{system naming: Selective Pause Frames? to distinguish from per-flow credits.  maybe I think there are too many of these systems that have C in the title so they all sound similar.}
We propose Backpressure Flow Control (BFC), a practical scheme that enables a switch to pause the flows at the upstream switch that are filling up the buffers at the current switch. BFC enables finer granularity congestion control to reduce buffering without causing head of line blocking or compromising throughput of a flow. Current switches support multiple FIFO Queues per egress port at a switch. On a new flow arrival the switch assigns the flow to a particular physical queue at the egress port corresponding to the flow. Based on congestion information from the downstream switch, the switch pauses/resumes these physical queues to mimic hop-by-bop per flow pausing. A switch only keeps track of a limited number of flows with packets in the switch, the switch uses this per flow information for deciding which flows to pause/resume at the upstream switch and to look up the physical queue assigned to a flow on arrival of a packet. BFC supports a variety of scheduling policies on the physical queues, e.g., Round Robin, Hierarchical Fair Queuing, etc. A key property of BFC is that it decouples the scheduling from the pausing mechanism. NICs in BFC are fairly simple and don't do any congestion control except pausing/resuming flows based on the congestion information from the downstream switch. The NIC schedules the unpaused flows at the line rate. BFC doesn't require manual tuning of parameters and is robust to changes in flow size distribution and link speed. We also establish bounds on memory required by BFC for book keeping at the switch and the bandwidth required for communicating congestion information across switches, and, show that BFC is realizable in practice.
\pg {Introduce buffer pooling in the design principles or here?}

\pg{We evaluated BFC in simulation using the ns-3 simulator. Our key findings are:}
\tom{also: key contributions, e.g., effective selective pause frames without per flow state}

\fi




%1. Explain the trends in modern data centers. Things are happening. Short (picture HOMA flow size distribution, Normalized buffer size)  (RDMA tranpsport moved into hardware -> PFC creates concnern about congestion spreading, congestion control have been designed to reduce PFC triggers, incast
%2.  Trends making this design challenging. Buffer Size, LinkSpeed, Short message sizes, fi). 
%2. Consequences of the trends -> More reactive stuff required. 
%3. Use Cases . 

==> motivation.tex <==
\section{Motivation}
\label{s:motivation}


Over the last decade, researchers and data center operators have proposed a variety of congestion control algorithms for data centers, including DCTCP~\cite{dctcp}, Timely~\cite{timely}, Swift~\cite{swift}, DCQCN~\cite{dcqcn}, and HPCC~\cite{hpcc}. The primary goals of these protocols are to achieve high throughput, low tail packet delay, and high resilience to bursts and incast traffic patterns.  Operationally, these protocols rely on {\em end-to-end} feedback loops, with senders adjusting their rates based on congestion feedback signals echoed by the receivers.
%\footnote{We discuss schemes like pFabric, pHost, NDP, and Homa that go beyond congestion control later.}  
Irrespective of the type of signal (e.g., ECN marks, multi-bit INT information~\cite{hpcc, kim2015band}, delay), the feedback delay for these schemes is a network round-trip time (RTT). This delay has an important role in the performance of end-to-end schemes. In particular, senders require at least one RTT to obtain feedback, and therefore face a hard tradeoff in deciding the starting rate of a flow. They can either start at a high rate and risk causing congestion, or start at a low rate and risk under-utilizing the network. Moreover, even after receiving feedback, senders can struggle to determine the right rate if the state of the network (e.g., link utilization and queuing delay) changes quickly compared to the RTT. 

We argue that three trends are making these problems worse over time, and will make it increasingly difficult to achieve good performance with end-to-end protocols.


%\smallskip
\noindent\textbf{Trend 1: Rapidly increasing link speed.}
\Fig{mot_broadcom} shows the switch capacity of top-of-the-line data center switches manufactured by Broadcom~\cite{broadcom,switchtrend}.  
Switch capacity and link speeds have increased by a factor of 10 over the past six years with no signs
of stopping. 
%As a result, much more data can be transmitted within a single round trip; for example, with a 100\,Gbps network link and 12\,$\mu$s round trip delay, there can be up to 150\,KB in flight before {\em any} feedback is received at the sender, making it more difficult for end-to-end protocols to manage congestion.


\begin{figure}[t]
     \centering
     %\vspace{-1mm}
    \includegraphics[width=0.8\columnwidth]{images_motivation/buffersize_linkspeed.pdf}
    \vspace{-4.5mm}
    \caption{\small  Hardware trends for top-of-the-line data center switches from Broadcom. Switch capacity and link speed have been growing rapidly, but buffer size is not keeping up with increases in switch capacity.}
    \label{fig:mot_broadcom}
    \vspace{-6mm}
 \end{figure}
 

 %\smallskip
 \noindent\textbf{Trend 2: Most flows are short.}
\Fig{mot_flowsize} shows the byte-weighted cumulative distribution of flow sizes for three industry data center workloads~\cite{homa}: (1) All applications in a Google data center, (2) Hadoop cluster in a Facebook center, and (3) a WebSearch workload.  Each point is the fraction of all bytes sent that belong to flows smaller than a threshold for that workload. For example, for the Google workload, flows that are shorter than 100~KB represent nearly half of all bytes.  Flows that are smaller than the bandwidth-delay-product (BDP) can ideally complete within one RTT, if the sender begins transmitting at line rate. As link speed increases, such flows represent a growing fraction of traffic. For example, most Facebook Hadoop traffic is likely to fit within one round trip within the next decade. %the churn in the number of active  ows at a link also increases with higher link speed since  ows arrive and depart more quickl
% not sure this is worth arguing about
% Note that the web search workload were measured from packet traces based on periods of inactivity in TCP connections, and are likely to have overestimated application-level transfers~\cite{homa}. 
%, with the web search traffic to follow the same trend shortly thereafter. 
While some have argued 
that data center flows are increasing in size~\cite{atulhotos}, the trend is arguably in the opposite direction with the growing use of RDMA for fine-grained remote memory access.


%\smallskip
\noindent\textbf{Trend 3: Buffer size is not scaling with switch capacity.}
 \Fig{mot_broadcom} shows that the switch buffer size relative to its capacity has decreased by a factor of 2 (from 80\,$\boldsymbol{\mu}$s to 40\,$\boldsymbol{\mu}$s) over the past six years. 
 With smaller buffers relative to link speed, buffers now fill up more quickly, making it more difficult for end-to-end congestion control to manage those buffers. The limiting factor is chip area\,---\,buffers and switching capacity compete for room on the same die, and better management of switch buffers 
 would allow for higher capacity switches.
 
\begin{figure}[t]
     \centering
     %\vspace{-1mm}
    \includegraphics[width=0.8\columnwidth]{images_motivation/mot_distribution.pdf}
    \vspace{-4mm}
    \caption{\small Cumulative bytes contributed by different flow sizes for three different industry workloads. The three vertical lines show the BDP for a 10~Gbps, 40~Gbps, and 100~Gbps network, assuming a 12~$\boldsymbol{\mu}$s RTT.}
    \label{fig:mot_flowsize}
    \vspace{-4mm}
 \end{figure}

\subsection{Limits of End-to-End Congestion Control}
 \label{s:mot-example}
 This combination\,---\,very fast links, short flows, and inadequate buffers\,---\,create the perfect storm for end-to-end congestion control protocols. Flows that complete within one or a few RTTs (which constitute an increasingly larger fraction of traffic) either receive no feedback, or last for so few feedback cycles that they cannot find the correct rate~\cite{sperc}. For longer flows, the rapid arrival and departure of cross-traffic creates significant fluctuations in available bandwidth at RTT timescales, making it difficult to find the correct rate. The result is loss of throughput and large queue buildup. Insufficient switch buffering further exacerbates these problems, leading to packet drops or link-level pause events  (PFC~\cite{PFC}) that spread congestion upstream. %\pg{Should we explicitly say that churn in active flows increases with link speeds?}

 \begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[trim={0 0 0 4mm},clip,width=\textwidth]{images_motivation/mot_noincast_ts.pdf}
        \vspace{-7mm}
        \caption{Variance in fair-share rate}
        \label{fig:mot:ll:ts}
    \end{subfigure}
    \begin{subfigure}[t]{0.17\textwidth}
        \includegraphics[trim={0 0 0 4mm},clip,width=\textwidth]{images_nsdi21/mot_noincast_tput.pdf}
        \vspace{-8mm}
        \caption{Throughput}
        \label{fig:mot:ll:tput}
    \end{subfigure}
    \begin{subfigure}[t]{0.17\textwidth}
        \includegraphics[trim={0 0 0 4mm},clip,width=\textwidth]{images_nsdi21/mot_noincast_qdelay.pdf}
        \vspace{-8mm}
        \caption{Queuing Delay}
        \label{fig:mot:ll:delay}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Variance in fair share rate, average throughput of a long-lived flow, and 99$^{th}$ percentile queuing delay experienced by single-packet flows. The available capacity for the long-lived flow in these experiments is 40\%.}
    % Increasing switch speed increases the variations in the fairshare rate and decreases the mean throughput of long flows.
    \label{fig:mot_noincast}
    \vspace{-5.5mm}
\end{figure}

\Fig{mot_noincast} shows the variance in the fair share rate for a long-lived flow competing on a single link with flows derived from the Facebook workload. We repeat the experiment at 10, 40, and 100~Gbps, and set the average load of the cross-traffic flows to be 60\% of the link capacity in each case. As link speed increases, cross-traffic flows arrive and finish more quickly, and the fair-share rate at the bottleneck link changes more rapidly. We also simulate two state-of-the-art congestion control protocols, DCQCN and HPCC, for this scenario.
Especially at higher link speeds, neither comes close to delivering the available bandwidth 
to the long flow or maintaining small queues for short flows.
% As link speed increases, both DCQCN and HPCC achieve lower throughput for the long-lived flow relative to the link speed (\Fig{mot:ll:tput}). Small flows also suffer a higher queuing delay at higher link speed (\Fig{mot:ll:delay}). 

\if 0

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images_motivation/mot_buffer.pdf}
    \vspace{-4mm}
    \caption{\small CDF of switch buffer occupancy relative to the capacity. The vertical line at 40~$\boldsymbol{\mu}$s represents Tomahawk3's buffer size. Higher speeds reduce the ability to control buffer occupancy.} % \pg{Should I add the data Tom suggested here? Not sure which you meant?}
    \label{fig:mot_buffer}
    \vspace{-6mm}
 \end{figure}

These issues also occur with incast. 
\Fig{mot_buffer} shows the switch buffer occupancy divided by the switch capacity for DCQCN and HPCC
as we vary the link speed. These simulations use a 2-tier Clos topology with 128 servers and the Facebook workload with an average load of 60\% relative to each link speed, out of which 5\% consists of synchronized flows that create incast (see \S\ref{s:eval} for details). To determine how well these schemes control buffer occupancy, we set the switch buffer sizes to be very large so that there are no packet drops. While one would expect the absolute buffer occupancy to increase with increasing link speed (since the BDP increases), the surprising finding  is that the {\em buffer occupancy relative to the switch capacity} also increases, indicating that the congestion control protocols are less effective at higher link speeds. 
\fi
%\smallskip
%\noindent{\bf An illustrative Example.}
% \subsection{An Illustrative Example} 
 
% \Fig{mot_buffer} shows the switch buffer occupancy divided by the switch capacity for two state-of-the-art congestion control protocols, DCQCN and HPCC, at three different link speeds. These simulations use a 2-tier Clos topology with 128 servers and the Facebook workload with an average load of 60\% relative to each link speed, out of which 5\% consists of synchronized flows that create incast (see \S\ref{s:eval} for details). To determine how well these schemes control buffer occupancy, we set the switch buffer sizes to be very large so that there are no packet drops. While one would expect the absolute buffer occupancy to increase with increasing link speed (since the BDP increases), the surprising finding  is that the {\em buffer occupancy relative to the switch capacity} also increases, indicating that the congestion control protocols are less effective at higher link speeds. 

%To understand the impact on application performance, \Fig{mot_qdelay} shows the queuing delay experienced by single-packet flows in the above experiments. Queuing delay at the tail increases at higher link speeds. Note that this increase in the tail queuing delay (at a port) is larger than the increase in the tail switch buffer occupancy (averaged across ports) from Fig.~\ref{fig:mot_buffer}. 

% There are two reasons for the decline in efficiency at higher link speeds. First, a larger fraction of the traffic completes in the first few RTTs before the congestion control protocol has time to stabilize. Second, the churn in the number of active flows at a link also increases with higher link speed since flows arrive and depart more  quickly. This implies that the correct rate for a flow, i.e., its fair share of the link, varies at a faster rate, making it more difficult to control buffers while utilizing the links completely. 

\cut{
\begin{figure}[t]
\centering
    \includegraphics[width=0.8\columnwidth]{images_motivation/mot_qdelay.pdf}
    \vspace{-4mm}
    \caption{\small CDF of per-packet queuing delay. Increasing switch speed, increases the per-packet latency at the tail.}
    \label{fig:mot_qdelay}
    \vspace{-4.5mm}
 \end{figure}}
 

%\smallskip
%\noindent\textbf{Other schemes:}


\subsection{Existing Solutions are Insufficient}

%Can't we address these challenges by using other existing scheme? Turns out the answer is no. 
There are several existing solutions that go beyond end-to-end congestion control. We briefly discuss the most prominent of these approaches and why they are insufficient to deal with the challenges described above.


\smallskip
\noindent{\bf Priority flow control (PFC).}
One approach to handling increased buffer occupancy would be to use PFC, a hop-by-hop flow control mechanism.\footnote{For simplicity, we focus on the case where there is congestion among the traffic at a particular priority level.} With PFC, if the packets from a particular input port start building up at a congested switch (past a configurable threshold), the switch sends a ``pause'' frame upstream, stopping that input from sending more traffic until the switch has a chance to drain stored packets. This prevents switch buffers from being overrun. Unfortunately, PFC has a side effect: head-of-line (HoL) blocking~\cite{dcqcn}. For example, incast traffic to a single server can cause PFC pause frames to be sent one hop upstream towards the source of the traffic. This stops {\em all} the traffic traversing the paused link, even those flows  that are destined to other uncongested egress ports. These flows will be delayed until the packets at the congested port can be drained. Worse, as packets queue up behind a PFC, additional PFC pause frames can be triggered at upstream hops, widening the scope of HoL-blocking.

%HoL-blocking is particularly problematic for tail-latency performance, as short flows can be queued be-hind much longer flows. Any congestion hurts tail latency, but HoL-blocking delays are often a large multiple of the delays a packet would experience in an idealized non-HoL blocking network at the same load level. 


\smallskip
\noindent{\bf Switch scheduling.}
Several efforts use switch scheduling to overcome the negative side-effects of elephant flows on the latency of short flows. These proposals range from approximations of fair queuing (e.g., Stochastic Fair Queuing~\cite{sfq}, Approximate Fair Queuing~\cite{afq}) to scheduling policies that prioritize short flows (e.g., pFabric~\cite{pfabric}, QJump~\cite{qjump}, Homa~\cite{homa}). 
While such scheduling policies can improve flow completion times, they cannot prevent packet drops or HoL-blocking due to PFC pause frames, given today's buffer-constrained switches (\S\ref{s:eval_performance}). The problem is that scheduling by itself does nothing to reduce buffer occupancy. As link speeds increase, the fair
share rate becomes more variable,
% reducing the ability of end-to-end congestion control to control buffer occupancy while keeping links utilized, 
and performance will suffer with end-to-end congestion control regardless of the scheduling policy. 

\smallskip
\noindent{\bf Receiver-based congestion control.}
Because sender-based congestion control systems generally perform poorly on incast workloads, some researchers have proposed shifting to a scheme where the receiver prevents congestion by explicitly allocating credits to senders for sending traffic.
Three examples are NDP~\cite{ndp}, pHost~\cite{phost} and Homa~\cite{homa}.
However, these schemes can only address congestion that occurs at the last hop, where the receiver has complete visibility. In practice, over-subscription is common, and measurements of production data center networks suggest that congestion can occur throughout the network~\cite{jupiter}.
Other proposals suggest collecting credits from all switches in the path before 
sending~\cite{expresspass, tva,scion}; at high link speeds, there is low auto-correlation 
in the fair share rate over short time scales (\Fig{mot_noincast}), making that problematic.

% I removed the Aeolus reference - as long as we remove the claim about saving the first round
% trip, we're ok.  I don't think Aeolus would work well in practice - it can have high loss rate in
% the first RTT, so to make it practical you'd need to separately reprioritize short flows.  But
% all that is way in the weeds. 

% \pg{Aeolus~\cite{hu2020aeolus} is a recent proposal that can be used as an add-on with such receiver-based schemes. While Aeolus can improve performance of the above schemes, their deployment regime is still restricted.}
% \sout{In other work}~\cite{expresspass, tva,scion}\sout{, routers give 
% credits to the sender via the receiver. This could be used to control congestion but incurs a high overhead for short flows. All flows must wait at least one RTT prior to transmitting, increasing the completion time of flows that fit in the BDP by 2-3$\times$.}  \pg{Aeolus exactly argues why this is not necessary. We don't know the short comings of their system well enough, except that the CC is still end-to-end.}


%Our goal with this work is to design a scheme that can work in modern heterogeneous data center environments, such as asymmetric topologies, and/or topologies with different link speeds and latencies. Moreover, these schemes are still end-to-end in nature, flows start at line rate to reduce FCTs. As a result, in case of an incast, these schemes can build deep packet buffers and also incur drops/PFCs, both of which hurt latency.


\subsection{Revisiting Per-hop, Per-Flow Flow Control}
Our approach is inspired by work in the early 90s on hop-by-hop credit-based flow control for managing
gigabit ATM networks~\cite{anderson1993high, kung1995credit}. Credit-based flow control was also introduced by multiprocessor hardware designs of the same era~\cite{chaos,dash,cm5}. In these systems, each switch methodically tracks its buffer space, granting permission to send at an upstream switch if and only if there is room in its buffer. In ATM, packets of different flows are buffered in separate queues and are scheduled according to the flows' service requirements. The result is a network that has no congestion loss by design. 

An ideal realization of such a per-hop, per-flow flow control scheme has several desirable properties: 

\noindent{\bf (1) Fast reaction:}  When a flow starts experiencing congestion at a switch, the upstream switch can reduce its rate within a 1-hop RTT, instead of the end-to-end RTT that it takes for standard congestion control schemes. Likewise, when capacity becomes available at a switch for a particular flow, the upstream switch can send it packets within a 1-hop RTT (provided the upstream switch has packets from that flow). Assuming a hardware implementation, the 1-hop RTT consists of the propagation latency and the switch pipeline latency\,---\,typically 1-2~$\mu$s.\footnote{For example, a 100~m cable has a propagation latency of 500~ns, and a typical data center switch has a pipeline latency around 500~ns~\cite{broadcom, tofino}.} This is substantially smaller than the typical end-to-end RTT in data centers (e.g., 10-20$\mu$s), which in addition to multiple switch hops includes the 
latency at the endpoints.
% even if the congestion control is implemented in hardware on the NIC

\noindent{\bf (2) Buffer pooling:} During traffic bursts, a per-hop per-flow flow control mechanism throttles traffic upstream from the bottleneck. This enables the bottleneck switch to tap into the buffers of its upstream neighbors, thereby significantly increasing the ability of the network to absorb bursts.

%\sout{For example, consider an incast event where $N$ senders simultaneously start transmitting to a single bottleneck switch at line rate. With end-to-end congestion control, the bottleneck switch would receive and have to buffer one end-to-end BDP of packets \emph{per sender}, even if the senders stop sending immediately after one end-to-end RTT. In contrast, with per-hop per-flow flow control, the bottleneck switch will throttle the traffic from a given upstream switch within a 1-hop RTT, and thus the maximum buffering at the bottleneck switch will be only one 1-hop BDP \emph{per upstream switch}. }
 
\noindent {\bf(3) No HoL-blocking:} Unlike PFC, there is no HoL-blocking or congestion spreading with per-hop per-flow flow control, because switches isolate flows in different queues and perform flow control for each of them separately. 

%. At an egress port each flow is scheduled based on the feedback from the upstream. This was a flow causing congestion at a switch doesn't affect other flows at the switch. Moreover, the backpressure feedback for the flow doesn't affect flows at the upstream either. 

 
\noindent {\bf (4) Simple control actions:} Flow control decisions in a per-hop per-flow flow control system are simpler to design and reason about than end-to-end congestion control algorithms because: {\em (i)} whether to send or pause a flow at a switch depends only on feedback from the immediate next-hop switch (as opposed to multiple potential points of congestion with end-to-end schemes), {\em (ii)} concerns like fairness are dealt with trivially by scheduling flows at each switch, and therefore flow control can focus exclusively on the simpler task of managing buffer occupancy and ensuring high utilization. 

%with flows isolated in separate queues and scheduled at each switch,  and flow control decisions can ignore concerns like fairness. 



%Deadlock can be prevented in a variety of ways, but is typically through per-destination queues. BFC differs from the earlier ATM approaches by using on/off pause frames  rather than numerical credits, and it does not assume per-connection state. As a result, BFC is not lossless.


Despite these compelling properties, per-hop per-flow flow control schemes have not been widely deployed, in part because of their high implementation complexity and resource requirements. As we detail in the next section, traditional ATM schemes require per-connection state and large buffers, and are not feasible to implement in today's data center switches. The principal contribution of our work is a practical design called Backpressure Flow Control (BFC). BFC differs from ATM approaches in several ways: it uses on/off pause frames rather than credits; it operates with a relatively small number (e.g., 10s) of physical queues per port;  it carefully manages buffer space to work within the bounds of current hardware; and, critically, {\em it does not require per-connection state}. BFC can be implemented using only constant-time switch operations on a modern programmable switch. BFC is not perfectly lossless, but it makes losses extremely rare.

\begin{table}
\small
\begin{center}
\begin{tabular}{c|c|c}
 Scheme & Throughput (\%) & 99\% Queuing Delay ($\boldsymbol{\mu}$s)\\ 
 \hline
 \hline
 BFC & 37.3 & 1.2 \\
  \hline
 HPCC & 22.9 & 23.9 \\
  \hline
 DCQCN & 10.0 & 30.4 \\
   \hline
 HPCC + SFQ & 21.9 &  15.9\\
\end{tabular}
\end{center}
\vspace{-5mm}
\caption{\small{For a shared link with a long flow, BFC achieves close to ideal throughput (40\%) for the long flow, with lower tail queuing delay. Same setup as \Fig{mot_noincast} on 100\,Gpbs links.}}
\label{tab:mot_bfc_noincast}
\vspace{2mm}
\end{table}



As an example of BFC's performance benefits, we repeat the experiment in \Fig{mot_noincast} with a single long-lived flow competing against variable cross-traffic with 60\% average load at 100\,Gbps link speed. Additionally, we include HPCC + SFQ (i.e., HPCC with stochastic fair queuing at the switches) in the results. Table~\ref{tab:mot_bfc_noincast} shows that BFC is able to achieve close to the maximum possible throughput for the long-lived flow (40\%), while reducing 99$^{th}$ percentile queuing delay compared to the other schemes.

\cut{
\begin{figure}[t]
\centering
    \begin{subfigure}[tbh]{0.208\textwidth}
        \includegraphics[width=\textwidth]{images_nsdi21/mot_bfc_buffer.pdf}
         \vspace{-7mm}
        \caption{Buffer Occupancy}
        \label{fig:mot_bfc:buffer}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.26\textwidth}
        \includegraphics[width=0.8\textwidth]{images_nsdi21/mot_bfc_fct.pdf}
        \vspace{-3mm}
        \caption{99$^{th}$ percentile FCT slowdown}
        \label{fig:mot_bfc:fct}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Per-hop, per-flow flow control (BFC) reduces buffer occupancy and improves flow completion time (FCT). %Same setup as \Fig{mot_buffer} on 100\,Gbps links, but with a 40\,$\mu$ buffer and PFC enabled.
    }
    \label{fig:mot_bfc}
    \vspace{-6mm}
\end{figure}
We also re-ran the experiment in \Fig{mot_bfc} that uses a 2-tier Clos topology with 128 servers and the Facebook workload with an average load of 60\%, out of which 5\% consists of synchronized flows that create incast. The link speed is 100~Gbps, and the switches have a 40\,$\mu$s shared buffer (relative to the switch capacity) with PFC enabled (see \S\ref{s:eval} for details). \Fig{mot_bfc:buffer} and \Fig{mot_bfc:fct} compare the switch buffer occupancy and 99$^{th}$ percentile flow completion time across different flow sizes for BFC, HPCC, DCQCN and HPCC + SFQ (i.e., HPCC with stochastic fair queuing at the switches). BFC reduces the peak buffer occupancy by nearly \pg{1.65$\times$} and  significantly reduces tail flow completion time (FCT) for both short and large flows. For example, it improves the tail latency by over 3.5$\times$ for both the shortest and the largest flows compared to HPCC + SFQ. 
}
% \pg{Note that PFC is responsible for reducing the buffer occupancy of other schemes compared to the numbers in \Fig{mot_buffer}. Should we say this?}


%These simulations use a 2-tier Clos topology with 128 servers and the Facebook workload with an average load of 60\% relative to each link speed, out of which 5\% consists of synchronized flows that create incast (see \S\ref{s:eval} for details). To determine how well these schemes control buffer occupancy, we set the switch buffer sizes to be very large so that there are no packet drops.







==> related.tex <==
\section{Related Work}
\label{s:related}

\smallskip
\noindent\textbf{ATM era schemes:} Our work was inspired by work in the early 90s on hop-by-hop credit-based 
flow control for managing high speed switches in ATM networks~\cite{anderson1993high, kung1995credit}. 
ATM networks have small fixed-sized cells and per-connection state at every switch.
Credit-based flow control was also introduced by multiprocessor hardware designs of the same era~\cite{chaos,dash,cm5}; 
the technique is still in wide use in that setting. In these systems, each switch methodically tracks its buffer space, 
granting permission to upstream switches to forward traffic if and only if there is room.  The result is
a network that has no congestion loss by design. Deadlock can be prevented in a variety of ways, but is
typically through per-destination queues. BFC differs from the earlier ATM approaches by using on/off pause frames 
rather than numerical credits, and it does not assume per-connection state. As a result, BFC is not lossless.

\smallskip
\noindent\textbf{Sender-based congestion control for RDMA:} Data center network operators have
developed and deployed several end-to-end congestion control protocols for RDMA networks.  These
differ in the feedback information available to the algorithms (TIMELY~\cite{timely} uses
delay variation, DCQCN uses ECN marks ~\cite{zhu2016ecn}, and HPCC uses link load~\cite{hpcc}).
For these systems, congestion information can be out of date by the time it arrives back at the sender,
and so careful control theory design is needed for stability, with multiple parameters that
must be carefully tuned to the workload and physical network. By contrast, because it operates
only over a single hop, BFC's control loop is shorter and simpler to configure, and can therefore
support higher utilization for a given target tail latency.

\cut{
\smallskip
\noindent\textbf{Selective retransmission:} We can remove the need for all-or-nothing PFC pause frames for RDMA by changing
the standard to support selective retransmission in hardware, as suggested by IRN~\cite{irn}. Handling arbitrary out-of-order
packets is non-trivial in hardware, however, and flows can still experience deep packet buffers and packet loss, especially
during incast events.
Recent work has shown that, replacing PFC with IRN helps DCQCN but does not remove the need for
congestion control~\cite{hpcc}. DCTCP~\cite{dctcp} and TCP Bolt~\cite{bolt} are software sender-based 
congestion control schemes. These support selective retransmission but have higher CPU overhead and latency 
than RDMA hardware. They are also vulnerable to incasts~\cite{vasudevan2009safe}. 
Recent work has shown that DCTCP has worse flow completion tail latency than HPCC~\cite{hpcc}. }

\smallskip
\noindent\textbf{Receiver-driven congestion control:} Because sender-based congestion control systems generally perform
poorly on incast workloads, some researchers have proposed shifting to a scheme
where the receiver prevents congestion by explicitly allocating credits to senders for sending traffic.
Three examples are NDP~\cite{ndp}, pHost~\cite{phost} and HOMA~\cite{homa}.
Unlike BFC, these schemes only address congestion that occurs at the last hop, assuming congestion
in the network is negligible.  Measurements of
production data center networks suggest that congestion can occur throughout the network~\cite{jupiter}. 
In earlier work on preventing denial-of-service attacks~\cite{tva,scion}, routers themselves give 
credits to the sender (via the receiver). This could be used to control congestion but faces 
similar control theory challenges to other end to end schemes.

\smallskip
\noindent\textbf{Switch scheduling:} Several efforts have looked at improving switch scheduling
to reduce average flow completion times. Stochastic fair queueing~\cite{sfq} hashes flows to a 
smaller number of FIFO queues to approximate fair queueing; our virtual-to-physical queue 
mapping accomplishes the same goal but avoids head-of-line blocking when the number of active flows is 
less than the number of physical queues. Approximate Fair Queuing (AFQ) \cite{afq} assigns packets 
to priority queues to approximate the order that fair queueing would schedule
packets. We considered using AFQ but could not devise a simple way to pause a flow once its packets had been
assigned to a priority level. pFabric~\cite{pfabric} labels packets at the sender with the amount of 
remaining data in the flow, allowing the switch to assign packets to priority queues to implement 
shortest remaining flow first.  We think of pFabric as complementary; it is future work to study 
how best to integrate BFC with switch scheduling algorithms like pFabric.



==> table.tex <==
\begin{table*}

\begin{center}
\small
 \begin{tabular}{|c |c |c|} 
 \hline
Function & Mechanism &Purpose \\
 \hline
 \hline
  Physical Queue (\S\ref{s:qassignment})& Dynamic assignment to physical queues & Efficient use of scarce physical queues  \\
  \hline
  Flow Table (\S\ref{s:qassignment})& Array indexed by <egress port, Hash(FID)> & Compute-efficient way to store state for flows \\
  \hline
  Upstream Queue (\S\ref{s:backpressure})& Physical queue assignment at the previous hop & Low overhead pausing/resuming of flows \\
  %Pause Frame (\S\ref{s:backpressure})& Bloom filter of Hash$_{BF}$(FID) & Low bandwidth signalling of paused flows \\
  \hline
  Pause Counter (\S\ref{s:backpressure})& Array indexed by <ingress port, upstream queue> & Tracking the upstream queues to be paused\\
  \hline
\end{tabular}
\end{center}
\vspace{-5mm}
\caption{\small{Key design components of \bfc{}.}}
\label{tab:functionality}
\vspace{-6mm}
\end{table*}

==> tofino2.tex <==
\section{SwitchX implementation}
\label{switchx}
We implemented BFC in SwitchX, a to-be-released P4-based programmable switch ASIC with a Reconfigurable Match Table (RMT) architecture~\cite{bosshart2014p4}. A packet in SwitchX first traverses the ingress pipeline, followed by the traffic manager (TM) and finally the egress pipeline. SwitchX has four ingress and four egress RMT pipelines. Each pipeline has multiple stages, each capable of doing stateful packet operations.
Ingress/egress ports are statically assigned to pipelines.
%\pg{All the per-packet operations are implemented entirely in the dataplane, and therefore BFC can run at full switch capacity. (recirculation caveat?)} 

\noindent
\textit{Bookkeeping:} The flow table and pause counter are both maintained in the ingress pipeline. The flow table contains three values for each entry and is thus implemented as three separate register arrays (one for each value), updated one after the other. 

\noindent
\textit{Multiple pipelines:} The flow table is \emph{split} across the four ingress pipelines, and the size of the table in each ingress pipeline is 25 $\times$ the number of queues. During normal operation, packets of an active flow arrive at a single ingress pipeline (same ingress port). Since the state for a flow only needs to be accessed in a single pipeline, we can split the flow table. However, splitting can marginally increase collisions if the incoming flows are distributed unevenly among the ingress pipelines. Similarly, the pause counter is split among the ingress pipelines. An ingress pipeline contains the pause counter entries corresponding to its own ingress ports. 

\noindent
\textit{Gathering queue depth information:} We need queue depth information in the ingress pipeline for pausing and dynamic queue assignment. SwitchX has an inbuilt feature tailored for this task. The TM can communicate the queue depth information for all the queues in the switch to all the ingress pipelines without consuming any additional ingress cycles or bandwidth. The bitmap of empty queues is periodically
updated with this data, with a different rotating starting point per pipeline to avoid new 
flows from being assigned to the same empty queue.
%However, it can take upto a $\mu$s to communicate queue depth to an ingress pipeline. We evaluate the impact of this delay in \pg{forward pointer}. 

\noindent
\textit{Communicating from egress to ingress pipeline:} The enqueue operations described earlier are executed in the ingress pipeline when a packet arrives. Deqeueue operations should happen at the egress but the bookkeeping data structures are at the ingress. To solve this, in the egress pipeline, we mirror packets
as they exit and recirculate the header of the mirrored packet back to the ingress pipeline it came from. The dequeue operations are executed on the recirculated packet header. 

Recirculating packets involves two constraints. First, the switch has dedicated internal links for recirculation, but the recirculation bandwidth is limited to 12\% of the entire switch capacity. 
% To reduce recirculation bandwidth consumption, we only recirculate the header of the packet. 
Second, the recirculated packet consumes an additional ingress cycle. The switch has a cap on the number of packets it can process every second (pps capacity). 

Most workloads have an average packet size greater than 500 bytes~\cite{benson2010understanding}, 
and SwitchX is designed with enough spare capacity in bandwidth and pps to handle header recirculation
for every packet for those workloads (with room to spare). 
% which is well above the average packet size SwitchX can process at full line rate. For these workloads, even at full incoming capacity the switch will have more than 50\% free cycles. 
If the average packet size is much smaller, we can reduce recirculations by sampling packets for recirculation (described in \App{incr_deploy}). 

Recirculation is not fundamental to BFC. For example, SwitchX has native support for PFC bookkeeping
in the TM. Likewise, if BFC bookkeeping was implemented in the TM, it would not need recirculation.
% as the bookkeeping tables can be accessed at both enqueue and dequeue in the TM. This the same reason why PFC is implemented in the TM in SwitchX. Moreover,
Similarly, in switches with a disaggregated RMT architecture~\cite{chole2017drmt} where 
the same memory can be accessed at both the ingress and egress, there is no need for recirculation.




%We believe that BFC should be implemented in the TM eventually, eliminating the need for recirculation. Note that PFC is implemented in the TM in SwitchX for the same reason. Moreover, in reconfigurable switches with disaggregated RMT architecture~\cite{chole2017drmt}, a memory block can be accessed at both the ingress and egress, and therefore there is no need for recirculation.





